Quantitative System-Level Security Verification of the IoV Infrastructure

The Internet of Vehicles (IoV) equips vehicles with connectivity to the Internet and the Internet of Things (IoT) to support modern applications such as autonomous driving. However, the consolidation of complex computing domains of vehicles, the Internet, and the IoT limits the applicability of tailored security solutions. In this paper, we propose a new methodology to quantitatively verify the security of single or system-level assets of the IoV infrastructure. In detail, our methodology decomposes assets of the IoV infrastructure with the help of reference sub-architectures and the 4+1 view model analysis to map identified assets into data, software, networking, and hardware categories. This analysis includes a custom threat modeling concept to perform parameterization of Common Vulnerability Scoring System (CVSS) scores per view model domain. As a result, our methodology is able to allocate assets from attack paths to view model domains. This equips assets of attack paths with our IoV-driven CVSS scores. Our CVSS scores assess the attack likelihood which we use for Markov Chain transition probabilities. This way, we quantitatively verify system-level security among a set of IoV assets. Our results show that our methodology applies to arbitrary IoV attack paths. Based on our parameterization of CVSS scores and our selection of use cases, remote attacks are less likely to compromise location data compared to attacks from close proximity for authorized and unauthorized attackers respectively.

==> sections/1.0_introduction.tex <==
% (autonomous vehicle, IOV)
\section{Introduction}

% \IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
% for IEEE journal papers produced under \LaTeX\ using
% IEEEtran.cls version 1.8b and later.


% paragraph about: like title states, most important idea is multi-layered security assessment/applicability/ 

%\instruction{here is a problem}
\IEEEPARstart{N}{ew} connectivity capabilities in the \ac{iov} provide vehicles with access to the Internet infrastructure and cloud. 
As a result, upcoming services around connected vehicles access new forms of data for enhanced driving experiences, safety, and automation such as autonomous decision making over maneuvers \cite{kaiwartya2016internet}.
Simultaneously, increasing connectivity causes an increase in complexity which opens up a larger surface for attackers. 
Attackers who successfully compromise vulnerabilities of the \ac{iov} infrastructure face new opportunities to remotely interfere with vehicles. 
As a direct consequence, the potential of attacks, that affect vehicle safety by accident or on purpose, increases \cite{sagstetter2013security}.
Attacks, such as remote control of air conditioning, brakes, power supply, steering, user data, and infotainment, count to recent attacks on connected vehicles \cite{wong2017uber} \cite{eiza2017driving}.
\begin{figure}[!ht]
\centering
\begin{tikzpicture}[scale=1]

\node (v1) at (-3,2) [scale=1, rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2.5cm, minimum height=0.5cm, transform shape = true, align=left] {Logical View};
\node (v12) at (-3,1.5) [transform shape = true, align=left, anchor=west] {Data};

\node (v2) at (3,2) [scale=1, rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2.5cm, minimum height=0.5cm, transform shape = true, align=left] {Developer View};
\node (v21) at (5.5,1.5) [transform shape = true, align=left, anchor=east] {Software};

\node (v3) at (-3,-2) [scale=1, rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2.5cm, minimum height=0.5cm, transform shape = true, align=left] {Process View};
\node (v31) at (-3,-1.5) [transform shape = true, align=left, anchor=west] {Communication};
% \node (vuln) at (2,2) [transform shape = true, align=left, anchor=west] {Libraries, Dependency, Variance, Change, Scale};

\node (v4) at (3,-2) [scale=1, rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2.5cm, minimum height=0.5cm, transform shape = true, align=left] {Physical View};
\node (v41) at (5.5,-1.5) [transform shape = true, align=left, anchor=east] {Hardware};


\node (v5) at (-1.1,0) [draw, anchor=west, thick, fill=white!95!blue, align=left, minimum height=2cm, minimum width=4.8cm, transform shape = true] {};
\node (v6) at (0,0) [scale=1, rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2.5cm, minimum height=0.5cm, transform shape = true, align=left] {Scenarios};
\node (v7) at (3.6,0.6) [transform shape = true, align=left, anchor=east] {Infra, Edge};
\node (v8) at (-1,0.6) [transform shape = true, align=left, anchor=west] {Cloud};
\node (v9) at (3.6,-0.6) [transform shape = true, align=left, anchor=east] {Vehicle};
\node (v10) at (-1,-0.6) [transform shape = true, align=left, anchor=west] {Peripherals};

\draw [->] (v1.east) -- ++(1.5,0) -- ++(0,-1.75);
\draw [->] (v2.west) -- ++(-1.5,0) -- ++(0,-1.75);
\draw [->] (v3.east) -- ++(1.5,0) -- ++(0,1.75);
\draw [->] (v4.west) -- ++(-1.5,0) -- ++(0,1.75);

% \node (vuln) at (2,2) [transform shape = true, align=left, anchor=west] {Libraries, Dependency, Variance, Change, Scale};

\end{tikzpicture}
  \caption{The 4+1 View Model in the \ac{iov} Context}
\label{fig:41IoVscenario}
\end{figure}

For the reason that jeopardized safety-critical systems threaten \ac{iov} acceptance, the investigation of holistic \ac{iov} security concepts represents a common interest of \ac{iov} infrastructure stakeholders \cite{rizvi2017threat}.
Even though comprehensive security solutions for the \ac{iov} exist, they remain in an early development stage. 
Reasons for that are the difficulty of progressing with administrative, legal, and technical development next to sophisticated interactions between a variety of components \cite{parkinson2017cyber}. % which introduce new dimensions of complexity
Thus, the applicability of legacy security patterns suffers and the interplay of different technological domains demands tailored, automated, dynamic, and adaptive security solutions.


To address this challenge, we propose a methodology that provides a modular structure to design and evaluate the security of the \ac{iov} architecture. 
For achieving the goal, this work breaks down the complexity of the \ac{iov} infrastructure using the 4+1 architectural view model \cite{kruchten19954+}, which is shown in Figure \ref{fig:41IoVscenario}, and by respecting the \ac{iov} reference architecture of \cite{maple2019connected}. 
%Figure  which is represented in Figure \ref{fig:41IoVscenario} \cite{kruchten19954+}
% MUDASSAR
% \fmma{I would suggest to move this figure to later section i.e. \ref{viewmodels} where you describe 4+1 model. The introduction section could include a graphical abstract kind of figure if any. The first impression of the paper and contributions comes from this first figure}.
To access the relevant system assets which require protection, the decomposition further relies on a definition of a \ac{cav} use case.
%\ac{iov} architecture in a structured way, the infrastructure decomposition requires a definition of a \ac{cav} use case.
%definition as input. 
Here, this work focuses on the scenarios of location services as they represent the enabling services for \ac{cav}s \cite{wan2018robust} \cite{suhr2016sensor}. 
% Figure \ref{fig:41IoVscenario} shows the application of autonomous shuttle busses and infrastructure assets that enable vehicle location estimation. 
The structured decomposition of the \ac{iov} infrastructure, in respect of the scenarios, sets the foundation for the application of threat modeling and risk assessment concepts per view model perspective.



The comprehensive threat modeling in this work follows an agile approach due to the active and frequently changing \ac{iov} architecture development \cite{oyler2016security} \cite{cruzes2018challenges}.
The analysis steps around the comprehensive threat modeling procedure comprise system modeling, threat, vulnerability, and risk analysis, definition of security requirements, and tailored security design solutions. 
Risk assessment in this work is based on the \ac{cvss} scores which, in turn, extracts the quantitative input to Markov Chains for security verification \cite{cheng2012research}.
We utilize Markov Chains to model the transitions of attack vectors and construct attack vectors based on the view model perspectives as well.
Together with the location service scenario, the attack vector propagation uncovers all necessary communication interfaces and, with that, the networking model of the infrastructure.



% allows fine grained extraction of the main system assets. 
% At the same time, this approach marks the basis requirement for threat modeling and risk assessment.
% Our work applies the 4+1 architecture model in the \ac{iov} context for the first time and demonstrates its applicability.

% \todo{rewrite form here til end of intro}

% The resulting assets of the infrastructure decomposition enables us to label assets with regard to attack surface and reference model type. % into abstraction layers of surface and reference model type.
% In alignment with the 4+1 viewpoint types, we define hardware, networking, software, and data as well as cloud, infrastructure and edge, and vehicle with peripherals as our attack surface and reference model types respectively. 
% The separation among surface types enables attack to vulnerability mapping of an asset. 
% As a next step, defence mechanisms map to attacks for the purpose of attack prevention.
% The mappings around an asset mark the input for the risk assessment of assets.

% The abstraction with regard to \ac{iov} reference architecture domains allows fine grained separation in the allocation of security requirements.
% This way, security requirements map to attributes of system assets which, implicitly, applies risk mitigation in the form of avoidance, acceptance, and transfer. 
% The approach further supports flexibility in attack prevention design.
% The security requirements ensure secure and safe state of asset attributes which are of value for attackers. 
% \todo{rewrite from here on}
% Apart from that, the amount of security requirements affects system complexity and, thereby, asset susceptibility which marks one metric of a vulnerability \cite{hughes2013quantitative}. 
% Our work points out the location of vulnerability analysis within the proposed framework and consequently, the evaluation of the framework relies on simplified vulnerability assessment for risk assessment. 

% Next, the processes within scenarios connect all asset and likewise the different layers of abstraction. 
% On one side, these processes indicate where to impose and connect security practices in the defence design.
% On the other hand, the processes illustrate asset connections which enables attack graph construction.
% Based on the location service application, the attack trees uncover all necessary communication interfaces and with that the networking model of the infrastructure.
% Network attack graphs provide Markov Chain characteristics which can be leveraged for security evaluation through risk assessment \cite{cheng2012research}. 
In short, our work aligns with the following procedure to create a security methodology to design and verify protected critical assets of an \ac{iov} architecture:
\begin{enumerate}
    % \item \ac{iov} use case definition
    \item Apply the 4+1 view model analysis of the \ac{iov} architecture
    % \item Asset identification through system decomposition that is based on the 4+1 architectural view model
    \item Threat modeling and risk assessment of \ac{iov} architecture assets in each of the view models
    \item Attack vector construction based on view model types
    \item Modeling of attack vector transitions for security risk assessment and verification using Markov Chains
    % Evaluation of the security framework based on its contribution to the applicability of Markov Chains for security risk assessment and verification
    \item Proposition and evaluation of an extendable security methodology that allows quantitative security design and verification
    %\ac{ttc} verification concepts of security design
\end{enumerate}

Thus, the contributions of the paper are the following:
\begin{itemize}
    \item To the best of our knowledge, this work applies the 4+1 architectural view model in the \ac{iov} security context for the first time
    \item Introduction of a Markov Chain based security verification concept that builds upon attack vectors between view model perspectives.
    %Comprehensive threat modeling and risk assessment of an \ac{iov} architecture on location service scenarios
    \item Proposition of an agile methodology to design and verify security concepts for the \ac{iov} infrastructure.
    
    %holistic, extendable, and verifiable multi-layer security framework
    % \item Extendable Model to Secure CAV Use Case (use case more complex, means build un top of the basic model of this paper)
\end{itemize}

The rest of the paper is organized as follows. 
Section \ref{section2} introduces the context of \ac{iov} architectures and the threat modeling concept whereas section \ref{relatedwork} presents related work. 
Sections \ref{section3} decomposes the \ac{iov} infrastructure based on the 4+1 view model and applies threat modeling and risk assessment on assets of each view model analysis domain. 
Section \ref{section4} constructs attack vectors towards the assets of the view model scenario and introduces \ac{ttc} security verification based on Markov Chains. Section \ref{section5} proposes and evaluates the security methodology before section \ref{section7} concludes. 

%\added{Rest of the paper is organized as follows. In Section \ref{}, a detailed background of .... Section \ref{} provides an overview of asset identification ....}\fmma{The introduction needs revision, e.g. there is no discussion on location services and it comes directly in the contributions. The storyline and the flow is missing. Rewriting in the end will improve it.}

%, \ac{iov} layer separation, and asset attack surface categorization. 
% The \ac{iov} use case of a connected autonomous bus\fmma{use case should be better introduced before referring to it} represents the 4+1 model scenario of this paper.
% The definition of a very basic CAV use case is important for reduction of the \ac{iov} infrastructure design space.
% other model can be used... 
% The structured decomposition of the \ac{iov} infrastructure allows fine grained extraction of the main security assets of the scenario and sets the basis for threat modeling.
% maybe reference multi layer IoV structure

% Input of the view model comes from...
% Next, the \ac{iov} stakeholder requirements analysis identifies most relevant and mandatory system assets and their attributes. 
% The determination of threats to those assets allows security requirement to asset attribute mapping. 
% This approach implicitly applies risk mitigation in the form of avoidance, acceptance, and transfer. 
% Risk reduction will be conducted actively by imposing security practices.

% ----- continue here -------

% It is possible to further categorize/divide mandatory architecture components into in-vehicle, road side infrastructure (smart city), internet infrastructure, and human layers. 
% Last, separation of component and communication assets deliver granular root assets for attack tree construction. 
% As the stakeholder requirement analysis identifies the properties of assets which require protection, attack trees span children and leafs consisting of attacks that eventually propagate to the most valuable assets.
% missing, how do we perform risk assessment DREAD, PASTA;
% Formula: Risk Value = (Damage+Affected users) x (Reproducibility+Exploitability+Discoverability)
% Formula: R = (T*V*P*I)/Countermeasures
% Subsequent risk assessment of \ac{iov} infrastructure assets based on Time to Compromise and Cost to Compromise complete the \ac{iov} threat modeling approach which consists of the following bullet points:
% \begin{enumerate}
%     \item 4+1 Architectural Model View of CAV Scenario Based on \ac{iov} Stakeholder Requirement Analysis
%     \item Security Requirement Analysis and Assessment CAV Use Case Root Assets
%     \item Attack Tree Construction on Communication and Component Assets
%     \item Risk Assessment of Root Assets
% \end{enumerate}

% The layered and granular decomposition of the \ac{iov} architecture with regard to security threats reveals and assesses (based on risk) cyberattack propagation that affect safety critical assets. 
% Furthermore, attacks can be grouped and mapped to multi layer security frameworks. 
% The application of a multi layer security solution provides a verifiable approach of critical \ac{iov} architecture asset protection.

% The main contributions of the paper are:
% \begin{itemize}
%     \item Comprehensive \ac{iov} Threat Modeling With Focus on Location Services
%     \item Multi-layer \ac{iov} Security Solution
%     \item Extendable Model to Secure CAV Use Case (use case more complex, means build un top of the basic model of this paper)
% \end{itemize}

% \added{Rest of the paper is organized as follows. In Section \ref{}, a detailed background of .... Section \ref{} provides an overview of asset identification ....}\fmma{The introduction needs revision, e.g. there is no discussion on location services and it comes directly in the contributions. The storyline and the flow is missing. Rewriting in the end will improve it.}

% This paper gathers all IoV infrastructure assets which attract attackers with an in-depth IoV stakeholder requirement analysis. 

% Insights of security threats and attack/error propagation on infrastructure entities enables verifiable and tailored security design of IoV infrastructures. 



% NO STATEMENT WITHOUT ARGUMENT, NO STATEMENT WITHOUT SAYING WHY !!!


% one contribution
% The security investigations of this work focuses on a running system in maintenance and support phase. Findings and outcomes contribute to all previous IoV development phases of requirement specification and design, feature development, integration and production, operation. (development models, waterfall ex) 




% Then next category is possible if attack breaks entity it has access to, for example access to interfaces, then break communication interface which results in cause, if this cause is of interest then fine, but if nothing is of interest, then requirement to utilize gained access to and analyse it for understanding how possible to attack over next physical attack vector.
% so attack vector is either physical ways to affect transmission of waves, or physical contact to computer hardware.
% this covers attack vector for vehicle and infrastructure




% PARAGRAPH about: existing solution gaps, where state of the art security lacks
% Attack and Error propagation.
% Mapping of attacks which can target multiple components at the same time have to be considered.
% Model and categorization of IoV infrastructure and mapping all attacks that exist down to components.
% Methodology allows to verify every attack and create security profile of categorizations within IoV infrastructure.



% PARAGRAPH about: our contribution
% In the beginning of all problems and to start breaking down all different security solutions, it is required to group all existing threats, and solutions 
% Initially, we define infrastructure security components of state of the art cybersecurity frameworks of IoV infrastructures.
% Stakeholder, safety critical, application, as well as general security requirement analysis make up SOTA IoV security goals. % need reference here. 
% By contrasting literature reviews of IoV security threats and existing IoV security countermeasures, we investigate and identify SOTA cybersecurity attack-to-component and countermeasure-to-attack mappings and security gaps of IoV infrastructures.
% In the end, we propose a verifiable multi-layered cybersecurity framework for SOTA IOV infrastructures. 

% 0. IoV context as grouper (vehicle, infrastructure, human) (important grouping)
% 1. break down hierarchy to attack surfaces (one category to group threats) -> this delivers threat countermeasure importance estimation/assessment in combination with IoV grouping  
% 2. apply security requirements to all attack surfaces (one category, this groups threats)
% 3. tool status of development phase (not to important)
% 4. component requirements (important category)



% I wish you the best of success.
% \hfill mds
% \hfill August 26, 2015
% \subsection{Subsection Heading Here}
% Subsection text here.


==> sections/1.1_background-relatedw.tex <==
\section{Background}
\label{section2}



\subsection{Security Definitions}
\label{secdefs}

% \todo{this section needs definition of risk assessment!}

% \fmma{Figure 2 appears here but but not discussed on this page.}
Computer security evolves around the main definitions of \emph{assets}, \emph{attacks}, and \emph{defence mechanisms}. % can also use \textit{} italic for word emphasis
The fundamental limitation of security solutions between these three definitions is the fact, that attackers with enough resources, such as time, money, etc., eventually succeed to compromise the \emph{defence mechanism} of a targeted \emph{asset} with any possible \emph{attack}.
% MUDASSAR
% \fmma{Suggestion: I would rather like to change the focus of discussion from attack to risk. So we can say "...of a targeted \emph{asset} with any possible \emph{risk} of attack"}
Hence, an acceptable \emph{defence mechanism} must add excessive %(impossible, disproportionate) 
monetary and/or time costs for the attacker \cite{arm2009security}.
There exist multiple models to describe each of the definitions and their characteristics in detail.


Starting with the \emph{asset}, it represents a protected resource of value for an attacker. 
An \emph{asset} provides a functionality, purpose or design which security requirements try to protect.
The dominating characteristic of an \emph{asset}, from the security perspective, is its vulnerability which stems from the way it is implemented.
Figure \ref{fig:mainsecurityblocks} shows the location of the vulnerability and its connections towards \emph{assets}, \emph{attacks}, and \emph{defence mechanisms}.
The vulnerability attribute of an asset represents a metric for exploitability or weakness with regard to a threat actor.
Throughout this work, we consider the terms, threat actor and attacker, the same and refer to them interchangeably.
Measuring a vulnerability determines the likelihood of an successful \emph{attack} on the \emph{asset}.
With that, the identification of flaws, their likelihood, and resulting impact of a vulnerability exploit count as \emph{risk assessment}.
% MUDASSAR
% \fmma{suggested: Risk assessment measures the likelihood of a successful attack due to vulnerabilities in the assets}
Multiple security \emph{risk assessment} models, which we introduce in section \ref{threatmodeling}, rely on vulnerability metrics as well.
Since an \emph{asset} is a protected resource, it should not expose any vulnerability which would enable an attacker to compromise the \emph{asset}.
Hence, vulnerability models have the objective to extract metrics of vulnerabilities with high impact to the risk assessment.
In order to determine the vulnerability risk of an \emph{asset}, Hughes and Cybenko introduce a fundamental model which describes three conditions that enable a successful \emph{attack} \cite{hughes2013quantitative}.
The necessity for an \emph{attack} to happen is the existence of susceptibility and accessibility properties of an \emph{asset} next to a threat capability.
The value of an asset and its vulnerability, logical and physical reachability, and techniques, tools, and resources to attack an \emph{asset} mark examples for the mentioned conditions respectively. 


% maybe cite software vulnerability discovery techniques: a survey (Software Vulnerability Discovery Techniques: A Survey)


% speak of the attacker model !!
Continuing with the \emph{attack}, its purpose is to intentionally acquire, modify, or disrupt an \emph{asset}.
To analyze the \emph{attack}, Hutzelmann et al. \cite{hutzelmann2019comprehensive} provide a fundamental and comprehensiveness attack model which illustrates the dominating characteristics of an \emph{attack}. 
Their structural \ac{uml} attack diagram connects an attacker, capability, exploit, and objective which mark the main components of an \emph{attack}. % by simultaneously respecting cardinalities between components.
The exploit component addresses \emph{assets} and their vulnerabilities and indicates the connection between the \emph{attack} context and the \emph{asset} context.
The capability and objective components depend on and connect to the attacker.
% This connection between attacker connected components and the exploit component shows the comprehensiveness of the \emph{attack} model.
To focus on the attacker more specifically, the work, defined by Monteuuis et al. \cite{monteuuis2018attacker}, introduces a general attacker model in order to identify similar attacks with different goals. 
Thereby, they introduce membership, motivation, scope, method, and goal as the key attributes of the attacker.
The work of \cite{karahasanovic2017adapting} adapts the \ac{tal} to the \ac{iov} domain and defines intent, access, outcome, resource, skills, motivations, visibility, limits, and objective as the key attributes of the attacker. 
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.9]
    
    % boxes and box description
    \node (box4) at (3.7,3.5) [draw, anchor=west, thick, align=left, minimum height=9.5cm, minimum width=4cm, transform shape = true] {};
    \node (vuln) at (-0.5,2) [transform shape = true, align=left, anchor=west, rotate=90] {Vulnerability};
    \node (vuln) at (8,5.5) [transform shape = true, align=left, anchor=west, rotate=-90] {ETSI SIEM Defence Approach};
    \node (vuln) at (-0.1,-1.25) [transform shape = true, align=left, anchor=west] {Attacker Context};
    \node (vuln) at (0,8.25) [transform shape = true, align=left, anchor=west] {Asset Context};
    
    % Asset Context
    \node (abox1) at (-0.25,7) [draw, anchor=west, thick, fill=white!95!blue, align=left, minimum height=2cm, minimum width=3cm, transform shape = true] {};
    \node (a1) at (0,7) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Asset};
    \node (a2) at (0,7.75) [transform shape = true,anchor=west, align=left] {Functionality};
    \node (a3) at (0,6.25) [transform shape = true, align=left, anchor=west] {Design};
    \node (a4) at (1.25,7) [transform shape = true, align=left, anchor=west] {Purpose};
    \node (a5) at (1.5,6.25) [transform shape = true, align=left, anchor=west] {etc.};
    
    % security requirements
    \node (sec1) at (0.5,5) [rectangle, anchor=west, thick, draw=black, fill=white!90!yellow, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Security \\Requirements};
    
    % Vulnerability
    \node (abox2) at (-0.25,3) [draw, thick, align=left, minimum height=2cm, minimum width=3cm, transform shape = true, anchor=west] {};
    
    \node (a1) at (0,3.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.5cm, minimum height=0.5cm, transform shape = true, align=left] {Implementation};
    \node (a2) at (0,2.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.5cm, minimum height=0.5cm, transform shape = true, align=left] {Attack/Exploit};
    
    % Attack Context
    \node (abox0) at (0-.25,0) [draw, anchor=west, thick, fill=white!95!red, align=left, minimum height=2cm, minimum width=3cm, transform shape = true] {};
    \node (abox12) at (0,0) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Attacker};
    \node (abox3) at (0,0.75) [transform shape = true, align=left, anchor=west] {Objective};
    \node (abox4) at (0,-0.75) [transform shape = true, align=left, anchor=west] {Capability};
    \node (abox5) at (1.65,0) [transform shape = true, align=left, anchor=west] {etc.};
    
    % Defence Context
    % \node (d3) at (4,0) [transform shape = true, align=left, anchor=west] {Detected \\ Events};
    % \node (d1) at (4,0) [transform shape = true, align=left, anchor=west] {Real Events};

    \node (d1) at (4,3.5) [rectangle, anchor=west, thick, draw=black, fill=white!90!green, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Security Prevention};
    \node (d2) at (4,5.2) [rectangle, anchor=west, thick, draw=black, fill=white!90!green, minimum width=3.25cm, transform shape = true, align=left] {Event Detection};
    \node (d4) at (4,2.5) [rectangle, anchor=west, thick, draw=black, fill=white!90!green, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Event Reaction};
    
    \node (a10) at (4,6.25) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Risk Assessment};
    \node (a11) at (4,7) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Policy \& Plan};
    \node (a12) at (4,7.75) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Verification};
    
    \node (d10) at (4,1.5) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Identify \& Confirm};
    \node (d11) at (4,0.75) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=3.25cm, minimum height=0.5cm, transform shape=true, align=left] {Neutralize};
    \node (d12) at (4,0) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Damage Assessment};
    \node (d13) at (4,-0.75) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=3.25cm, minimum height=0.5cm, transform shape = true, align=left] {Restore \& Learn};
    
    % lines:
    \draw [-{>[scale=1.5]}] (abox1.south) -- ++(-1,0) -- ++(0,-2.25);
    \draw [-{>[scale=1.5]}] (abox1.south) -- ++(0.35,0) -- ++(0,-0.5);
    \draw [-{>[scale=1.5]}] (sec1.south) -- ++(0,-0.75);
    \draw [-{>[scale=1.5]}] (sec1.east) -- ++(0,0.2) -- (d2.west);
    \draw [-{>[scale=1.5]}] (sec1.east) -- ++(0,-0.2) -- ++(2,0) -- ++(0,-1);
    \draw [-{>[scale=1.5]}] (d1.north) -- ++(0,1.15);
    
    \draw [-{>[scale=1.5]}] (abox2.north) -- ++(0,0.5);
    
    \draw [-{>[scale=1.5]}] (d2.north) -- (a10.south);
    \draw [-{>[scale=1.5]}] (a10.north) -- (a11.south);
    \draw [-{>[scale=1.5]}] (a11.north) -- (a12.south);
    
    \draw [-{>[scale=1.5]}] (d4.south) -- (d10.north);
    \draw [-{>[scale=1.5]}] (d10.south) -- (d11.north);
    \draw [-{>[scale=1.5]}] (d11.south) -- (d12.north);
    \draw [-{>[scale=1.5]}] (d12.south) -- (d13.north);
    
    \draw [-{>[scale=1.5]}] (abox0.north) -- (a2.south);
    \draw [-{>[scale=1.5]}] (a2.east) -- (d4.west);
    \draw [-{>[scale=1.5]}] (a2.north) -- (a1.south);
    \draw [-{>[scale=1.5]}] (d1.west) -- (a1.east);
    
    \draw [-{>[scale=1.5]}] (d2.east) -- ++(0.2,0) -- ++(0,-2.7) -- (d4.east);
    
    % \draw [->] (loca1.east) -- (el2.west);
    % \draw [-] (el2.north) -- ++(0,0.78);
    
    \end{tikzpicture}
  \caption{Interplay of Security Definitions That Contribute to Risk Assessment}
\label{fig:mainsecurityblocks}
\end{figure}
The diversity of attack actor models, vulnerabilities, and the complexity of the attack cost leads to many forms of \emph{attacks} \cite{abomhara2015cyber}. 
Variations of attacker attributes may affect vulnerability metrics such as threat capability or system accessibility which aggravates attack-centric risk assessment.


% Other vulnerability metrics for risk estimation and assessment such as the \ac{cvss} score \cite{schiffman2004common} align with this basic model. 
% Although the formula of the \ac{cvss} model comes with more fine grained metric groups. 
% Their base, temporal, and environmental formula groups the impact of \emph{attacks} on security requirements, the impact on exploitability, remediation, and report, and the impact of damage potential respectively to an overall vulnerability score.
% The \ac{dread} \cite{singhal2013fuzzy} and \ac{stride} \cite{hernan2006threat} models count as traditional risk assessment models. 
% The focus of the \ac{dread} model falls into the threat capability, system susceptibility, and environmental metric domains whereas the \ac{stride} model on threat accessibility and security requirements of the \ac{cvss} base formula focuses.
% The \ac{mttc} risk models, on the other hand, allow flexible application and weighting all risk assessment metrics for the calculation of system wide security verification \cite{nzoukou2013unified}.
% However, the application of \ac{mttc} calculations requires a comprehensive asset, threat, network, and process model of the system. 
% Attack graph models incorporate these requirements which in turn allow \ac{mttc} estimation and verification, typically, through modelling of attack graphs with Markov Chains \cite{mcqueen2006time}.

% Membership refers to the affiliation of the attacker in form of authorized insider or unauthorized outsider. Trusted developers or device owners count as authorized protagonists \cite{arm2009security}.
% Motivation differentiates the motives of maliciously damaging an \emph{asset} or rationally exploit profit.
% The scope attribute describes the share of compromised infrastructure which an extended or local attacker controls.
% Last, the method attribute labels \emph{attacks} as active or passive, whereas the \todo{goal direct versus indirect attackers categorize. 
% Direct attackers reach the intended target.}

% In contrast, the attacker model, defined by Monteuuis et al. \cite{monteuuis2018attacker}, focuses on the attacker explicitly before investigating possible attacks

% The attacker component receives input of the motivation component and connects to the capability and objective component. 
% The attacker aptitude, access, and tools make up the remaining inputs to the capability components which connects to the exploit component.
% The system surface or part and the weakness mark the inputs to the exploit component which connects to the objective component to close the loop between the main \emph{attack} components.
% In system and transcending units branch the input to the objective component.
% All connections


% Here, the 
% Another generic attacker model, defined by Monteuuis et al. \cite{monteuuis2018attacker}, introduces membership, motivation, scope, method, and goal as the key attributes of the attacker. 
% It

% All components around the four 
% Additionally, the work specifies the components that make up each of the core components.
% The first zone around the core components consists of motivation which connects to the attacker, aptitude, access, and tools which connect to the capability, weakness and system part which connect to the exploit, and in and transcending system components which connect to the objective.
% Another generic attacker model, defined by Monteuuis et al. \cite{monteuuis2018attacker}, introduces membership, motivation, scope, method, and goal as the key attributes of the attacker.
% Membership refers to the affiliation of the attacker in form of authorized insider or unauthorized outsider. Trusted developers or device owners count as authorized protagonists \cite{arm2009security}.
% Motivation differentiates the motives of maliciously damaging an asset or rationally exploit profit.
% The scope attribute describes the share of compromised infrastructure which an extended or local attacker controls.
% Last, the method attribute labels \emph{attacks} as active or passive whereas the goal direct versus indirect attackers categorize. 
% Direct attackers reach the intended target.
% Variations of attacker attributes may affect vulnerability metrics such as threat capability or system accessibility which indicates the importance of attacker attributes with regard to risk assessment of \emph{assets}.
% All existing \emph{attacks} that originate of attackers 


% might go into background and this needs rewriting in the the sense that 
% The attacker capability follows the categorization options of beginner, intermediate, and expert \cite{abraham2016estimating}.
% The extend of system information gathering and vulnerability/susceptibility exploitation increases in respect of attacker capability. 
% Concerning threat accessibility, latest attacker models in the \ac{iov} consider different general dimensions that apply to and attribute/categorize an attacker during threat access exploitation \cite{monteuuis2018attacker}.
% The dimensions to describe an attacker are membership, motivation, scope, method, and goal.
% Membership refers to the affiliation of the attacker in form of authorized insider or unauthorized outsider. Trusted developers or device owners count as authorized protagonists \cite{arm2009security}.
% Motivation differentiates the motives of maliciously damaging an asset or rationally exploit profit.
% The scope attribute describes the share of compromised infrastructure which an extended or local attacker controls.
% Last, the method attribute labels attacks as active or passive whereas the goal direct versus indirect attackers categorize. Direct attackers reach the intended target.

% Attributes such as the attacking objective of an attacker determine the value of an \emph{asset} for the attacker.




% \begin{figure}[!ht]
%     \centering
%     \begin{tikzpicture}[scale=0.9]
    
%     % 3 major blocks in center
%     \node (el1) at (0,0) [rectangle, anchor=east, thick, draw=black, fill=yellow, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Security \\Prevention};
%     \node (loca1) at (1.15,0) [transform shape = true, align=left] {Real \\Events};
%     \node (el2) at (4,0) [rectangle, anchor=east, thick, draw=black, fill=yellow, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Event \\Detection};
%     \node (loca2) at (5.275,0) [transform shape = true, align=left] {Detected \\Events};
%     \node (el3) at (8,0) [rectangle, anchor=east, thick, draw=black, fill=yellow, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Event \\Reaction};

%     \draw [->] (el1.east) --  (loca1.west);
%     \draw [->] (loca1.east) -- (el2.west);
%     \draw [->] (el2.east) -- (loca2.west);
%     \draw [->] (loca2.east) -- (el3.west);
%     \draw [-] (el3.south) -- ++(0,-0.69);
%     \draw [-] (el2.north) -- ++(0,0.78);

%     % top blocks for detection block
%     \node (netw1) at (3.25,2) [draw, align=left, minimum height=1.5cm,minimum width=7.75cm, transform shape = true] {};
%     \node (el4) at (1.3,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Risk \\Evaluation};
%     \node (el5) at (3.1,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Security \\Policy};
%     \node (el6) at (4.7,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Master \\Plan};
%     \node (el7) at (7,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Verification};

%     \draw [->] (el4.east) -- (el5.west);
%     \draw [->] (el5.east) -- (el6.west);
%     \draw [->] (el6.east) -- (el7.west);

%     % lower blocks for reaction block
%     \node (netw2) at (3.25,-2) [draw, align=left, minimum height=1.7cm,minimum width=9.5cm, transform shape = true] {};
%     \node (el8) at (0.4,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Identify \& \\Confirm \\Event};
%     \node (el9) at (2.4,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Neutralise \\Attack};
%     \node (el10) at (4.25,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Evaluate \\Damages};
%     \node (el11) at (6.25,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Restore \\Normal \\Operation};
%     \node (el12) at (7.85,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Learn \\Lesson};

%     \draw [->] (el8.east) -- (el9.west);
%     \draw [->] (el9.east) -- (el10.west);
%     \draw [->] (el10.east) -- (el11.west);
%     \draw [->] (el11.east) -- (el12.west);

%     \end{tikzpicture}
%   \caption{ETSI SIEM approach against the 3 main security measures \cite{etsi008gsisi}}
% \label{fig:mainsecurityblocks}
% \end{figure}


% speak of the defence mechanisms !!
Last, a \emph{defence mechanism} is a tailored security design or mechanism to counteract an \emph{attack}.
Information security design divides into three main categories of prevention, detection, and reaction which may interact with each other in comprehensive security frameworks.
The right part of Figure \ref{fig:mainsecurityblocks} illustrates categories of defence mechanisms.
Here, the \ac{siem} approach, specified by the \ac{etsi}, embodies an example where a detection and reaction of an security incident have the potential to handle failing prevention techniques. % , shown in Figure \ref{fig:mainsecurityblocks}, ...
Security prevention mechanisms build upon existing vulnerabilities or implement security requirements.
They count to the most used and initial security considerations when designing \ac{it} systems.
For instance, encryption, hashing, and redundancy protect the traditional \ac{cia} security requirements respectively.
% detection examples and process explanation
The detection of security critical events comprises different procedures. 
Risk evaluation as the initial incident processing step feeds the parameterization of security policies.
Section \ref{threatmodeling} introduces risk assessment and evaluation procedures. 
Security policies apply differently depending on the assessment of security requirements or patch feasibility of assets.
The \ac{asil} represents a metric that describes the patch potential of the system \cite{murashkin2015automated}.
The next part of the event detection process organizes and improves security rules of security models that are used for verification. 
For instance, verification procedures may require network graphs for probabilistic model checking which, in turn,  allows modular and system wide security analysis \cite{mundhenk2015security}. 
An example intrusion detection is the time interval analysis of in-vehicle network messages \cite{song2016intrusion}. % intrusion detection timing analysis of can messages
In comprehensive security frameworks, the detection triggers the reaction process which performs the countermeasure strategy. 
The transition of the driving level into safe mode is a potential neutralization of the attack that precedes the damage evaluation step of the reaction plan \cite{waszecki2017automotive}.
Regarding terminology, neutralization and mitigation strategies of risks through either prevention, detection or reaction defines the broader term of \emph{risk management}. 


% Examples for risk evaluation are vulnerability scores such as the \ac{cvss} score \cite{schiffman2004common}, \ac{dread}, \ac{stride} \cite{cagnazzo2018threat}, or the location of the incident detection along an attack path which aggregates metrics such as the \ac{mttc} \cite{nzoukou2013unified}. % \cite{abraham2016estimating}, PASTA, CIA

% \fmma{Fig 3 has wrong placement, should be on next page where it is referred. Moreover, it will be good to say in figure caption that yellow boxes are our extensions?}. 



% On the other hand and with regard to defence mechanisms, the \ac{asil} metric describes the patch potential of the system \cite{murashkin2015automated}.


% everything after attack prevention: --> SIEM platform
% The prevention techniques mark the first building block of three main security blocks proposed by the \ac{etsi} standardization specification for information security \cite{etsi008gsisi}. % important to follow eu regulations in security design

% % maybe include again!
% Figure \ref{fig:mainsecurityblocks} shows the building blocks together with the \ac{etsi} \ac{siem} approach.
% The \ac{siem} framework allows attack detection, reaction, and adaptation which mitigates the attacker capability condition. 



% The vulnerability attribute of an asset represents a metric to measure the likelihood of an successful attack on the asset. 
% Categories such as logical and physical reachability of the asset, techniques, tools, and resources used to attack an asset, or the value of an asset itself count as factors that make up an vulnerability \cite{hughes2013quantitative}. 
% Vulnerability scoring systems such as the \ac{cvss} score \cite{schiffman2004common} and risk assessment methodologies such as \ac{dread}, \ac{stride} \cite{cagnazzo2018threat}, or the \ac{mttc} metric \cite{nzoukou2013unified} weight vulnerability factors differently depending on the application.
% On the other hand and with regard to defence mechanisms, the \ac{asil} metric describes the patch potential of the system \cite{murashkin2015automated}.


% \todo{
% add info that attack only possible if 3 measures of susceptibility, threat accessibility, and attacker capability hold. then vulnerability exist
% }
% Moreover, the quantative exploitation critaria is also covered in \cite{schiffman2004common} Common Vulnerability Scoring System (ac here), which has 3 parts that take basically same info into account.

% Next regarding defence mechanism, Automotive Safety Integrity Level (ASIL) detemines patch capability of the system 

\subsection{Security Requirements}
\label{riskassessment}

The formulation of security requirements has been of prime importance ever since computing systems existed. Models such as the CIA triad expanding Parkerian Hexad \cite{reid2010using} or Marta and Calderon's security taxonomy \cite{calderon2007taxonomy} categorize ever-increasing security requirements. Marta et al. describe elicitation of security requirements by performing the following approach:
\begin{enumerate}
    \item Identification of functional system requirements
    \item Identification of assets which require protection
    \item Identification of threats to identified assets
    \item Definition of software security requirements on assets based on identified threats
\end{enumerate}
The latest and most comprehensive security requirement taxonomy, presented by Rjaibi et al. \cite{rjaibi2015developing}, covers thirteen top category requirements which group thirty-one security requirements sub-factors. 
Nevertheless, the complexity that comes with the amount of security requirements and the overlapping categorizations encourage to stick to traditional or domain specific security requirements. 
Microsoft's \ac{stride} model \cite{hernan2006threat} builds upon six security requirements of integrity, authenticity, availability, confidentiality, non-repudiation, and authorization and remains in focus of recent research \cite{cruzes2018challenges}.
Regarding the automotive domain, \cite{monteuuis2018attacker} introduces access control, trustworthiness, availability, integrity, accountability, privacy, and adaptability to group the main security requirements.
Additionally, automated modeling tools exist for the well studied security concepts which allow concrete mappings to threats \cite{turpe2017trouble}.
Another implicit characteristic that comes with the application of security requirements is the risk treatment and control through strategies of defence, transfer, mitigation, acceptance, and termination \cite{whitman2011principles}.
The decision to apply a security requirement to an asset involves risk identification, assessment, and a control strategy which, additionally, depends on feasibility studies and cost-benefit analysis.


% This paper applies the presented taxonomy to identify security requirements in \ac{iov} scenarios that are needed to protect all relevant system assets against threats. 
% \todo{decide on which metrics to use, opinion go with traditional stride model}



% take existing part, and reformulate
% Our threat modeling approach, shown in Figure \ref{fig:iovthreatmodel}, extends the mentioned steps by adding an \textit{asset requirement evaluation} step after system model decomposition.
% The \ac{iov} stakeholder asset evaluation implicitly applies an early risk treatment and assessment strategy on application level which later supports risk reduction, transfer, avoidance, or acceptance mitigation decisions.
%\fmma{it is more appealing to justify the reasons to add these steps. So, you could say .... The asset requirement evaluation step is added to implicitly apply an early risk treatment ... }





% OS firmware and Data are part of the software branch
% \begin{figure}[!ht]
%     \centering
%     \begin{tikzpicture}[scale=0.9]
    
%     % hardware level
%     \node (loca) at (0,10) [transform shape = true] {Local Attacker};
%     \node (phya) at (5,10) [transform shape = true] {\textbf{Physical Access Propagation}};
%     \node (hardw1) at (0,9) [draw, transform shape = true] {Hardware};
%     \node (r1) at (5,9) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Interface, Memory, Processor}; % System on Chip 2 System on Chip
%     \node (softw1) at (0,8.25) [draw, transform shape = true] {Software};
%     \node (r2) at (5,8.25) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Driver, Thread, Process, Stack}; % Process 2 Process
%     \node (netw1) at (0,7.25) [draw, transform shape = true] {Communication};
%     \node (r3) at (5,7.25) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Destination Identity, Protocol, \\Transport, Time}; % Routing, Delay, Addressing, Device 2 Device, Hardware 2 Hardware

%     % networking entry
%     \node (rmat) at (0,6) [transform shape = true] {Remote Attacker};
%     \node (neta) at (5,6) [transform shape = true] {\textbf{Communication Access Propagation}};
%     \node (netw2) at (0,5) [draw, transform shape = true] {Communication};
%     \node (r4) at (5,5) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Source Identity, Protocol, \\Transport, Time};
%     \node (softw2) at (0,3.85) [draw, transform shape = true] {Software};
%     \node (r5) at (5,3.85) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Process, Thread, Driver, \\Stack};
%     \node (hardw2) at (0,2.75) [draw, transform shape = true] {Hardware};
%     \node (r6) at (5,2.75) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Processor, Memory, \\Interface};
    
%     \draw [->] (loca.south) -- (hardw1.north);
%     \draw [->] (hardw1.south) -- (softw1.north);
%     \draw [->] (softw1.south) -- (netw1.north);
%     \draw [->] (netw1.south) -- (rmat.north);
    
%     \draw [->] (rmat.south) -- (netw2.north);
%     \draw [->] (netw2.south) -- (softw2.north);
%     \draw [->] (softw2.south) -- (hardw2.north);
%     \draw [->] (hardw2.south) -- ++(0,-0.3) -- ++(-1.75,0) -- ++(0,8.3) -- ++(1.75,0) -- (loca.north);
    
%     \draw [->] (phya.south) -- (r1.north);
%     \draw [->] (r1.south) -- (r2.north);
%     \draw [->] (r2.south) -- (r3.north);
%     \draw [->] (r3.south) -- (neta.north);
    
%     \draw [->] (neta.south) -- (r4.north);
%     \draw [->] (r4.south) -- (r5.north);
%     \draw [->] (r5.south) -- (r6.north);
%     \draw [->] (r6.south) -- ++(0,-0.15) -- ++(3,0) -- ++(0,8.45) -- ++(-3,0) -- (phya.north);
    
%     %\draw [->] (loca) -- (phya);
%     %\draw [->] (8,9) -- (8,7);
%     %\draw [->] (loca.south) -- (rmat.north);
%     %\draw [->] (netw1.west) -- ++(-0.5,0) -- (rmat);
%     %\draw [->] (rmat) -- (neta);
%     % \draw [->] (0,4.5) -- (0,2.5);
%     %\draw [->] (rmat.south) -- ++(0,-3.5);

%     \end{tikzpicture}
%   \caption{High Level Attack Surface Propagation}
% \label{fig:attackSurface}
% \end{figure}

% \subsection{Risk Assessment}
% \label{riskassessment}



\subsection{Threat Modeling}
\label{threatmodeling}

% explain all threat modeling with centrics
% explain risk assessment that is possible with the models such as dread and others: 

% we use agile because !!

% remember, difficult to apply threat modeling in agile approach due to abstraction wihch we heavily address

% \todo{cite thesis}

% go through initial mapping,
To identify the main characteristics among different threat modeling approaches, chapter two of the comprehensive work of Shostack \cite{shostack2014threat} introduces threat modeling strategies which are asset-centric, attack-centric, and software-centric models.
By iterating over the threat modeling methodologies of the survey of Hussain et al. \cite{hussain2014threat}, the \ac{stride} threat model, which identifies spoofing, tampering, repudiation, information disclosure, denial of service, and elevation of priviledge as the main threats, counts as a software-centric threat model. 
Likewise, the \ac{stride} Average Model, Fuzzy Logic model and the Abuser Stories methodology utilize \ac{stride}. % which extends agile software development practices in respect of security flaw detection
Attack trees or similar graphical threat modeling concepts model system assets or attacks at different attack propagation stages depending on the assignment of the security expert.
Hence, it is not possible to allocate attack trees to either of the three threat modeling approaches. 
Nevertheless, graphical concepts provide flexibility and extendibility and fit into iterative threat modeling procedures.
% reaction/adaptation/ examples and explanation
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.9]
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% IMPORTANT: vulnerability analysis means common vulnerability score!!
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% the structure comes from "IoT Security Framework for Smart Cyber Infrastructures"
    %%%%%%%%%%%%%%%%%%%%%%%%%%%% 1) Identify attackers, assets, threats and other components, 2) Rank the threats, 3) Choose mitigation strategies, and 4) Build mitigation solutions based on the strategies.
    
    %%%%%%%%%%%%%%%%%%% and ::::::::::: A. Shostack,Threat modeling: Designing for security
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 1. model system, 2. find threats, 3. address threats, 4. validate
    
    
    % \node (el1) at (0,0) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.75cm, minimum height=1cm, transform shape = true, align=center] {Asset \\Identification};
    % \node (el2) at (3,0) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.5cm, minimum height=1cm, transform shape = true, align=center] {Model \\Decomposition};
    % \node (el3) at (5.75,0) [rectangle, anchor=west, thick, draw=black, fill=yellow, minimum width=3cm, minimum height=1cm, transform shape = true, align=center] {Asset Requirement \\Evaluation};
    % \node (el4) at (5.75,-1.25) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=3cm, minimum height=1cm, transform shape = true, align=center] {Attack Surface \\Analysis};
    % \node (el5) at (3,-1.25) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.5cm, minimum height=1cm, transform shape = true, align=center] {Risk Analysis};
    % \node (el6) at (0,-1.25) [rectangle, anchor=west, thick, draw=black, fill=yellow, minimum width=2.75cm, minimum height=1cm, transform shape = true, align=center] {Tailored Security \\Design};
    
    \node (el1) at (0,0) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.75cm, minimum height=1cm, transform shape = true, align=center] {System \\Modeling};
    \node (el2) at (3,0) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.5cm, minimum height=1cm, transform shape = true, align=center] {Threat Analysis};
    \node (el3) at (5.75,0) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=3cm, minimum height=1cm, transform shape = true, align=center] {Vulnerability \\Analysis};
    \node (el4) at (5.75,-1.25) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=3cm, minimum height=1cm, transform shape = true, align=center] {Risk Analysis};
    \node (el5) at (3,-1.25) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=2.5cm, minimum height=1cm, transform shape = true, align=center] {Security \\Requirements};
    \node (el6) at (0,-1.25) [rectangle, anchor=west, thick, draw=black, fill=yellow, minimum width=2.75cm, minimum height=1cm, transform shape = true, align=center] {Tailored Security \\Design};
    
    \draw [->] (el1) -- (el2);
    \draw [->] (el2) -- (el3);
    \draw [->] (el3.east) -- ++(0.25,0) -- ++(0, -1.25) -- (el4.east);
    \draw [->] (el4) -- (el5);
    \draw [->] (el5) -- (el6);
    \draw [->] (el6.west) -- ++ (-0.25,0) -- ++(0,1.25) -- (el1.west);

    \end{tikzpicture}
  \caption{Agile Threat Modeling Approach in the \ac{iov}, actually threat modeling only until build mitigation, security framework enables verification, but older work names validation}
\label{fig:iovthreatmodel}
\end{figure}
Attack libraries such as the \ac{capec} \cite{barnum2008common} or the Intel \ac{tal} \cite{casey2007threat} address the attacker attributes and represent attacker-centric models. 
The automotive compatible \ac{tara} model marks another attacker-centric model that is based on different threat related libraries \cite{karahasanovic2017adapting}.
To close the scope of approaches, the asset-centric \ac{octave} \cite{albert2001octave} and \ac{tvra} \cite{etsi2010intelligent} models analyze threats, risks, and vulnerabilities together.


The work of \cite{karahasanovic2017adapting} and \cite{macher2016review} address the versatility and applicability of threat modeling approaches where \cite{karahasanovic2017adapting} propose a \ac{iov} tailored threat modeling procedure which adapts the \ac{tara} and \ac{stride} strategy.
Based on their work and due to the fact that multiple threat modeling strategies overlap in most of their consecutive processing steps, our work follows the threat model strategy of Figure \ref{fig:iovthreatmodel}.
This threat model strategy represents an iterative process of system modeling, threat, vulnerability, and risk analysis, security requirement definition, and tailored security design.
% As all threat modeling approaches define slightly differentiating but consecutive processing steps.
% \todo{this needs update!, find processes in comments of figure}
This concept aligns with the proposed threat modeling procedures of \cite{shostack2014threat}, \cite{karahasanovic2017adapting}, and \cite{islam2016risk}.
To clarify the statement, \cite{shostack2014threat} relies on the four step framework of  system modeling, threat analysis, threat mitigation, and validation.
In \cite{karahasanovic2017adapting}, the adapted \ac{tara} model lists threat agent risk analysis, high level risk threat agent evaluation, attack method and exposure analysis, and strategy design to target exposures. 
The adapted \ac{tal}, \ac{mol}, and \ac{cel} libraries drive this approach.
The work of \cite{islam2016risk} introduce a risk assessment framework for the automotive domain. 
The strategy relates to threat modeling approaches and consists of system definition, threat analysis, risk assessment, and definition of security requirements.
Their threat analysis identifies assets before the actual threats.
Moreover, the risk assessment block comprises threat and impact level estimation and security level determination.
Finally, the work Hamad et al. \cite{hamad2016towards} combines all aspects of threat modeling, attack tree construction, and risk assessment in a comprehensive threat modeling approach tailored for vehicles.

% Our work aligns with the sequence of \textit{asset identification}, \textit{system model decomposition}, \textit{attack surface analysis}, \textit{threat identification}, and \textit{risk analysis} for threat modeling. 
% Each of the works \cite{hussain2014threat}, \cite{cruzes2018challenges}, \cite{shostack2014threat}, \cite{karahasanovic2017adapting} applies at least a partial subgroup of the mentioned procedures. 
In contrast to general threat modeling approaches such as fuzzy, probabilistic, tree-based, graphical and legacy threat modeling, our work follows the agile threat modeling approach. 
The iterative nature of agile threat modeling provides the necessary flexibility in security analysis for the constantly evolving \ac{iov} domain. 
With this approach, updates of security goals and requirements remain customizable \cite{cruzes2018challenges}. 
Software security analysts have the possibility to iteratively decrease abstraction levels, or change the quantification of scenarios. 
Moreover, our threat model approach includes a final block of tailored security design. % an early asset requirement identification and a
The reasons for this are the work of Xiong et al. \cite{xiong2019threat}, which state the design of a tailored security concept as future work, and the requirement definition of a mitigation concept in \cite{pacheco2016iot}.
% The reason for this is that the attack surface analysis benefits from the asset prioritization and early system complexity management \cite{jaatun2019threat}.
% Further, the work of Xiong et al. \cite{xiong2019threat} states the design of a tailored security concept as future work whereas the four consecutive threat modeling steps of \cite{pacheco2016iot} a mitigation concept requires.

%%%%%%%%%%% IMPOARTANT>>> The reason for this is that the attack surface analysis benefits from the asset prioritization and early system complexity management \cite{jaatun2019threat}.



Threat modeling does not pre-define which method to use for individual processing steps.
As a result, it is left to the security expert to apply suitable processing methodologies for the respective fields. 
The \ac{dfd}, for instance, represents one way to determine the reference model in graph form during asset identification and model decomposition \cite{karahasanovic2017adapting}.
In order to gain structured access to asset identification, model decomposition, and attack surface analysis, our work relies on a view model approach that is described in section \ref{viewmodels}.
% Furthermore, the section states how the security requirement evaluation finds application in the view context.
% Most of the models define the methodology of risk assessment and analysis.
% Nevertheless, t
After the threat and vulnerability analysis, the application of attack graphs for risk analysis remains desirable, not only in respect of agility requirements.
Even though attack trees require detailed system reference models, they remain recommended for system design security analysis \cite{macher2016review}.  
Moreover, it is possible to apply \ac{mttc} risk models if a comprehensive asset, threat, network, and process model of the system exist.
The \ac{mttc} risk models allow flexible parameterization and weighting of all risk metrics for the calculation of system wide security verification \cite{nzoukou2013unified}. 
Thereby, the modelling of attack graphs with Markov Chains enables the incorporation of risk assessment metrics \cite{mcqueen2006time}.
Other vulnerability metrics for risk estimation and assessment such as the \ac{cvss} score \cite{schiffman2004common} or the \ac{dread} \cite{singhal2013fuzzy} model may support the parameter selection for risk estimation.


% Other vulnerability metrics for risk estimation and assessment such as the \ac{cvss} score \cite{schiffman2004common} align with this basic model. 
% Although the formula of the \ac{cvss} model comes with more fine grained metric groups. 
% Their base, temporal, and environmental formula groups the impact of \emph{attacks} on security requirements, the impact on exploitability, remediation, and report, and the impact of damage potential respectively to an overall vulnerability score.
% The \ac{dread} \cite{singhal2013fuzzy} and \ac{stride} \cite{hernan2006threat} models count as traditional risk assessment models. 
% The focus of the \ac{dread} model falls into the threat capability, system susceptibility, and environmental metric domains whereas the \ac{stride} model on threat accessibility and security requirements of the \ac{cvss} base formula focuses.
% The \ac{mttc} risk models, on the other hand, allow flexible application and weighting all risk assessment metrics for the calculation of system wide security verification \cite{nzoukou2013unified}.
% However, the application of \ac{mttc} calculations requires a comprehensive asset, threat, network, and process model of the system. 
% Attack graph models incorporate these requirements which in turn allow \ac{mttc} estimation and verification, typically, through modelling of attack graphs with Markov Chains \cite{mcqueen2006time}.


% Additionally, the pragmatic approach of agile development emphasizes and breaks down threat modeling to only four main consecutive steps \cite{cruzes2018challenges}; that is,  \textit{a) Asset identification}, \textit{b) system model decomposition}, \textit{c) attack surface analysis}, and \textit{d) threat identification and risk analysis}.


%% name why we need the extended design and speak about possible risk assessment (vulnerability score mention as well) (TTC - TTVD) with these models and name why we take the holistic model also mention related work as example which mentions limitation that missing security needs to be included!

% refer to figure here


% Moreover, we apply and evaluate a holistic and \ac{iov} tailored multi-layer security model in an additional last step which addresses all identified threats and attacks. 
% The security model maps attacks and threats to a tailored framework of interconnected countermeasures which extends the threat model towards the comprehensive conceptual model of Shostack et al. \cite{shostack2014threat}.
% \deleted{Figure \ref{fig:iovthreatmodel} shows our agile-based threat model approach.}


% \todo{complete restructure, paragaph structure influence of centricity categorization, mohammad thesis}

% \todo{cite threat modeling survey (THREAT MODELLING METHODOLOGIES: A SURVEY) and mohammad recommendation (Adapting Threat Modeling Methods for the Automotive Industry)}
% https://s3.amazonaws.com/academia.edu.documents/49665567/Threat_modeling_methodologies_a_survey.pdf?response-content-disposition=inline%3B%20filename%3DTHREAT_MODELLING_METHODOLOGIES_A_SURVEY.pdf&X-Amz-Algorithm=AWS4-HMAC-SHA256&X-Amz-Credential=ASIATUSBJ6BAMX3UWBGM%2F20200422%2Fus-east-1%2Fs3%2Faws4_request&X-Amz-Date=20200422T223237Z&X-Amz-Expires=3600&X-Amz-Security-Token=IQoJb3JpZ2luX2VjECYaCXVzLWVhc3QtMSJIMEYCIQCxIchIMMn1aSrW947ouxYrQL8hX6CRebHrTd%2FsGnnuHwIhAPFxr2pAj6PPUyjmsD5GdC0zwM9we9hHOOipFVKVamHVKrQDCE8QABoMMjUwMzE4ODExMjAwIgwziS5Nt%2B0hAO%2BymaEqkQNInnxXZFl6zwVWtMkOCNkGCosjHhCJn6CsztK%2FLqXVJSQ%2Bi9nTAwNoOkn6utv9DHQ5Mimt6ORAoAB0Q8OvEn9ldAagtNzsxY%2BCITPrbT15105cWlzs2CMPgeXqYBpSG0HrS%2BOSdFMO3iS4gdzZqmY28kIEXbHYX39vePiw82yvK80jLqcfwRpoegyfJxskBI0%2FfufOFCLtjtxRdohb%2BPkaiu2qOf7%2Bh42XiUwA1d0onjy6QuFV6mL9e2dS6N49gHt3hetU6TSrjYh0i9rC1VYhj4LXn98wUSbP%2Fi39KSgmGAwTvaYT9%2FghhDHkx%2Bs2iJbPBK%2BhHXVwZFpdyuuJ8c7PKGVUrHWN6YDYYk7ExDmNqc8lUCWFfxRV%2Bmaa41gy1yaxrjmBZD2wdmFNeQj6DqCIGYgjq%2FutG5afqEL8fcV6sVihQRmrKqQgjGCJOmVHWpWGcyBUNS1YQ5DevrcXI3yf8TAzrFo0J4ue10v3MkoL5%2BrRqvsZ3aUjxjP%2Fsge5DAPrfjbabAGOVzngXsyoiUheEzDw%2FYL1BTrqAVivuGr7LDijTYpvwt%2F6iDpaoxbfHrTspT2rxYhZsqb9IzyXY3LryzB9cWyUg%2BWYQ7N7YkV9JAERDfi1YqnZR0jcg9zj7L9kcq6h8J43nc3kX%2FybCdgu4RXomfoy9SlvBbRQtjf30zQeu%2BwK%2BEZj0Ox3K4hBlGnlM%2F2bthntmVidK%2BNPxReytJ8REQQHTdAitzNKPnozcI6NvCvM1KmqROtlB34aq2pcg7qjIKQB3xbf204iCR5q0wjN5UHFfWgaFnQkn3iNLjsKd1ILX%2BzEB8y3XfgT7R4We4RfJfJXSGDlfCdyDPFGoKOzOg%3D%3D&X-Amz-SignedHeaders=host&X-Amz-Signature=859f11c8c828e9fceced71c314a163d21da9935615fbc5a5356d7a81f9ba7d2f
% 

% \todo{cite coras: cora's threat modelling}
% https://books.google.de/books?hl=en&lr=&id=X4lpi3stRvYC&oi=fnd&pg=PR6&dq=cora%27s+threat+modelling&ots=Sejce15AjI&sig=duFX5zl0qJvDYhPUYLUDGkCHDt0#v=onepage&q=cora's%20threat%20modelling&f=false
% @book{lund2010model,
%   title={Model-driven risk analysis: the CORAS approach},
%   author={Lund, Mass Soldal and Solhaug, Bj{\o}rnar and St{\o}len, Ketil},
%   year={2010},
%   publisher={Springer Science \& Business Media}
% }

% https://cheatsheetseries.owasp.org/cheatsheets/Threat_Modeling_Cheat_Sheet.html


% \begin{figure}[!ht]
% \centering
% \begin{tikzpicture}[scale=0.7]

% \node (r1) at (-2,2.75) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, anchor=west] {Cloud};

% \draw pic[scale=0.3,transform shape = true] (server1) at (-1.75,-0.3) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.3,transform shape = true] (server1) at (-1.25,-0.3) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.3,transform shape = true] (server1) at (-0.75,-0.3) {server={black!30!white}{white!30!blue}{white!60!blue}};
% % \draw pic[scale=0.25,transform shape = true] (server1) at (3,3.5) {server={black!30!white}{white!30!blue}{white!60!blue}};
% % \draw pic[scale=0.25,transform shape = true] (server1) at (3.5,3.5) {server={black!30!white}{white!30!blue}{white!60!blue}};
% % \draw pic[scale=0.25,transform shape = true] (server1) at (4,3.5) {server={black!30!white}{white!30!blue}{white!60!blue}};

% \draw pic[scale=0.4,transform shape = true] (switch1) at (-2,1) {switch={black!10!white}{}};
% \draw pic[scale=0.4,transform shape = true] (switch2) at (-1,1) {switch={black!10!white}{}};
% \draw pic[scale=0.4,transform shape = true] (switch3) at (-1.5,1.5) {switch={black!10!white}{}};
% % \draw (1,4) -- (1.75,4.3);
% % \draw (2.4,4) -- (1.75,4.3);
% % \draw (1.5,3.8) -- (1.75,3.8);

% % \node () at (5,5.4) [transform shape = true, anchor=west] {Communication};
% % \node () at (5,5) [transform shape = true, anchor=west] {Microservices};
% % \node () at (5,4.6) [transform shape = true, anchor=west] {Data Analysis};
% % \node () at (5,4.2) [transform shape = true, anchor=west] {Data Storage};
% % \node () at (5,3.8) [transform shape = true, anchor=west] {Monitoring};

% % \draw pic[scale=1,transform shape = true] (clod) at (1,4) {cloud={cloud}{}};


% %% !!TOD: balken diagram for software services

% % Environment, Infrastructure, and Edge
% \node (r2) at (1,2.75) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, anchor=west] {Infra \& Edge};

% \draw pic[scale=0.15,transform shape = true] () at (0.95,1.25) {satelite={white!30!gray}{}};
% \draw pic[scale=0.3,transform shape = true] () at (1.95,2) {cellularsite};
% \draw pic[scale=0.5,transform shape = true] () at (2.95,1.35) {fuelcharge};
% \draw pic[scale=0.4,transform shape = true] () at (1.1,0) {trffclight={red}{yellow}{green}};
% \draw pic[scale=1.25,transform shape = true] () at (1.95,0) {parking={P}};
% \draw pic[scale=1,transform shape = true] () at (2.925,0) {busstop={B}};

% % \node () at (5,3) [transform shape = true, anchor=west] {Actuators};
% % \node () at (5,2.6) [transform shape = true, anchor=west] {Energy Systems};
% % \node () at (5,2.2) [transform shape = true, anchor=west] {Sensors};
% % \node () at (5,1.8) [transform shape = true, anchor=west] {Physical input/output};
% % \node () at (5,1.4) [transform shape = true, anchor=west] {Communication};
% % \node () at (5,1) [transform shape = true, anchor=west] {Microservices};
% % \node () at (5,0.6) [transform shape = true, anchor=west] {Data Analysis};
% % \node () at (5,0.2) [transform shape = true, anchor=west] {Data Storage};
% % \node () at (5,-0.2) [transform shape = true, anchor=west] {Monitoring};


% % Vehicle
% \node (r3) at (4,2.75) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, anchor=west] {Vehicle};

% \draw pic[scale=0.2,transform shape = true] () at (4.5,-0.25) {vehicle={white!50!gray}{blue!15!white}};
% \draw pic[scale=0.2,transform shape = true] () at (4.65,0.9) {mybus={yellow}{blue!10}{black!60!green}};

% % \node () at (5,-1) [transform shape = true, anchor=west] {Wireless Communications};
% % \node () at (5,-1.4) [transform shape = true, anchor=west] {Data Storage};
% % \node () at (5,-1.8) [transform shape = true, anchor=west] {Vehicle Sensors};
% % \node () at (5,-2.2) [transform shape = true, anchor=west] {Infotainment};
% % \node () at (5,-2.6) [transform shape = true, anchor=west] {HMI};
% % \node () at (5,-3) [transform shape = true, anchor=west] {Physical Input/Output};
% % \node () at (5,-3.4) [transform shape = true, anchor=west] {Monitoring};
% % \node () at (5,-3.8) [transform shape = true, anchor=west] {Data Analysis};
% % \node () at (5,-4.2) [transform shape = true, anchor=west] {Actuators};
% % \node () at (5,-4.6) [transform shape = true, anchor=west] {Energy System};

% % Peripherals
% \node (r4) at (7,2.75) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, anchor=west] {Peripherals};

% \draw pic[scale=0.7,transform shape = true] () at (7.45,1) {person};
% \draw pic[scale=0.3] () at (8.35,1.3) {antenna};
% \draw pic[scale=0.17] () at (7.75,-0.4) {smartphone={}} ;

% % \node () at (5,-5.4) [transform shape = true, anchor=west] {Applications};
% % \node () at (5,-5.8) [transform shape = true, anchor=west] {Sensors};
% % \node () at (5,-6.2) [transform shape = true, anchor=west] {Wireless Communications};
% % \node () at (5,-6.6) [transform shape = true, anchor=west] {Physical Input/Output};
% % \node () at (5,-7) [transform shape = true, anchor=west] {Data Storage};

% \draw [<->] (r1.east) -- (r2.west);
% \draw [<->] (r3.east) -- (r4.west);
% \draw [<->] (r3.north west) -- ++(0,0.5) -- ++ (0.5,0) -- ++(0,-0.5);
% \draw [<->] (r2.north) -- ++(0,0.75) -- ++(5.9,0) -- (r4.north);
% \draw [<->] (r2.east) -- (r3.west);
% \draw [<->] (r2.north west) -- ++(0,0.5) -- ++(0.5,0) -- ++(0,-0.5);

% \end{tikzpicture}
%   \caption{Hardware \& Communication Summary of \ac{cav} Reference Model \cite{maple2019connected}}
% \label{fig:referenceArchitecture}
% \end{figure}


\subsection{View Model Frameworks in the Security Context}
\label{viewmodels}

Before introducing the attack surface of the \ac{iov} which happens in section \ref{attacksurfacecategorization}, we introduce different view models which organize descriptions of software architecture. 
This allows us to inspect the reference models and abstraction concepts of the \ac{iov} infrastructure in respect of structured perspectives.
There are several view angles to analyze an \ac{iov} infrastructure \cite{karkhanis2018defining}. 
Considering functional, communication, implementation, enterprise, usage, information, physical, stakeholder, and user viewpoints all together does not bring benefits with regard to security analysis \cite{maple2019connected}. 
Categories may introduce either to much complexity and inconsistencies or, in essence, do not contribute to security related purposes such as attack analysis. 
Hence, a sufficiently balanced portfolio of viewpoints increases the applicability of appropriate security concepts \cite{hughes2013quantitative}.
It is possible to balance the tradeoff between security concept applicability and reference architecture complexity by utilizing the approach of the 4+1 architecture model \cite{kruchten19954+}.
The view model builds upon five concurrent views.
The logical, developer, process, and physical view help to analyze assets, attacker threat vectors, and defence mechanisms individually. 
The fifth scenario view illustrates the four differentiating descriptions of the software architecture and enables validation.
Figure \ref{fig:41IoVscenario} shows the 4+1 view model in the \ac{iov} context together with common characteristics that apply in each of the views.
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.9]

    %\node (one) at (-0.5,2) [transform shape = true] {(a)};
    \node (el11) at (0,6) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attack Goal};
    \node (el12) at (0,5) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attacker Capability};
    \node (el13) at (0,4) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Information Gathering};
    \node (el14) at (0,3) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {System Hacking/Access};
    \node (el15) at (0,2) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attack on Asset};
    \node (el16) at (0,1) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Backpropagation};
    
    \draw [->] (el11.south) -- (el12.north);
    \draw [->] (el12.south) -- (el13.north);
    % \draw [->] (el13.east) -- ++(1,0) --++(0,-1.25) -- (el14.east);
    \draw [->] (el13.south) -- (el14.north);
    \draw [->] (el14.south) -- (el15.north);
    \draw [->] (el15.south) -- (el16.north);
    
    %\node (one) at (-0.5,-0.5) [transform shape = true] {(b)};
    \node (el21) at (4,6) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attack Goal};
    \node (el22) at (4,5) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attacked Function};
    \node (el23) at (4,4) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attack Surfaces};
    \node (el24) at (4,2) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attack on Asset};
    \node (el25) at (4,1) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=3.75cm, minimum height=0.5cm, transform shape = true, align=left] {Attacker Capability};

    \draw [->] (el21.south) -- (el22.north);
    \draw [->] (el22.south) -- (el23.north);
    % \draw [->] (el23.south) -- ++(0.4,0) -- ++(0,-1.25) -- (el24.north);
    \draw [->] (el23.south) -- (el24.north);
    \draw [->] (el24.south) -- (el25.north);

    \end{tikzpicture}
  \caption{Attacker view (left) extracted from \cite{10.5555/3067087} vs. the attack tree identification process for attack surface analysis (right) of \cite{maple2019connected}}
\label{fig:attackerview}
\end{figure}
The model enables the identification of security relevant system boundaries and information flows in respect of essential and topic relevant views.
Simultaneously, the model respects abstraction levels between different views.
This fact enables cross view/domain security evaluation and contributes to a balanced and system wide security verification. % through  network graph creation and markov chains



%%%%%%% attention: this next paragraph might be part of the use case asset identification section in chapter 3, first part of the approach 
Focusing on each view individually, the logical view decomposes the system by leveraging principles of abstraction, encapsulation, and inheritance to describe end-user functionality and services. 
The process view utilizes requirements such as performance, availability, concurrency, distribution, integrity, fault tolerance to map logical view abstractions into a process model of communicating processes and tasks which reveal computing load.
The development view organizes software modules and their import and export relationships by considering rules such as partitioning, grouping, scope, decoupling, reuse, portability, communication, time dependence and reveals allocations of requirements, costs, and planning.
The physical view model determines the physical components of computer networks, processors and interfaces in consideration of non-functional system requirements such as performance, scalability, reliability, and availability drive configuration, deployment and testing decisions of various nodes.
In essence, these properties drive hardware capacity requirements of the physical architecture.
Last, the scenarios define application procedures, sequences, and interactions, identify validation, verification and illustration concepts, and mark the input to all model views.
In the context of threat modeling, the scenario definition is essential, as it reduces complexity of the attack surface by prioritizing assets and system management requirements \cite{jaatun2019threat}.
Moreover, they enable a target-oriented system modeling and asset analysis which represents the initial step of threat modeling and risk assessment approaches.
% The reason for this is that the attack surface analysis benefits from the asset prioritization and early system complexity management \cite{jaatun2019threat}.
As of today, standardized tool sets and development frameworks facilitate implementations of each view model individually.
%%%%%%%


% \todo{layers together with reference model and attack surface categorization, picture of attacker that can interfere with major communication paths between these components}

% \todo{explain how security requirement evaluation can be applied on views}

% \todo{multiple view models exist with more than just 4 views: \cite{karkhanis2018defining}, also reference model paper has multiple view points...}

% Top sentence explain why we use 4+1 over other possible solutions, cite reference architecture paper with other view examples, reason is complexity reduction, find this reference again, then this part right below
% Architectural view models mark the methodology of grouping essential and topic relevant views for a specific and detailed analysis model. 

% Hence, our work leverages the 4+1 software architecture view model to identify security relevant system boundaries and information flows \cite{kruchten19954+}. 
% Separate views such as the logical, developer, process, and physical view help to analyse individual assets, attacker threat vectors, and defence mechanisms. 
% Figure \ref{fig:41IoVscenario} show the 4+1 view model which applies separate views on the same set of scenarios.

% \begin{figure}[!ht]
%     \centering
%     \begin{tikzpicture}[scale=0.9]

%     \node (el1) at (2,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true] {Logical View};
%     \node (el2) at (4,2) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true] {Development View};
%     \node (el3) at (2,0) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true] {Process View};
%     \node (el4) at (4,0) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true] {Physical View};
%     \node (el5) at (3,1) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true] {Scenarios};

%     \draw [->] (el1.south) -- ++(0,-0.45) -- (el5.north west);
%     \draw [->] (el2.south) -- ++(0,-0.45) -- (el5.north east);
%     \draw [->] (el3.north) -- ++(0,0.47) -- (el5.south west);
%     \draw [->] (el4.north) -- ++(0,0.46) -- (el5.south east);

%     \end{tikzpicture}
%   \caption{4+1 Software Architecture View Model}
% \label{fig:fouroneviewmodel}
% \end{figure}
% 
% \todo{remove 4+1 view figure \ref{fig:fouroneviewmodel}, instead take ioV scenario plus view into introduction}


% this needs correction!! 
% \subsubsection{Attacker \& Defender View}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% \todo{shorten this last paragraph?}
Other view model frameworks in the security context cover the perspectives of the attacker and defender.
The attacker view, shown on the left side of Figure \ref{fig:attackerview}, represents the kill chain attacker view model \cite{al2016cyber} which illustrates the view of an ethical hacker \cite{10.5555/3067087}.
The application of this view model framework identifies the attacking process, task, and communication flows that an attacker need to accomplish in order to compromise a system.
Identified attack vectors with the help of this model contribute to and represent a basis requirement for attack vector construction \cite{al2016cyber}.
On the other hand, the view model analysis of \cite{maple2019connected}, introduced on the right side of Figure \ref{fig:attackerview}, reflects the attacking process, goals, and functions from the defender perspective.
The outcome of this model are defence concepts which prevent an attacker from capturing system assets. 

%%%%%% DESCRIPTION OF FIGURE 4
% Both modeling techniques start with the definition of attack goals.
% After that, the attacker view considers attacker capability in the form of knowledge of system fundamentals and cryptography.
% The attacker capability affects the consecutive step of information gathering which includes system footprinting, scanning, and enumeration.
% The information, collected to this point, influences the system hacking outcomes.
% Moreover, system hacking relies on methodical exploitation approaches and tools such as password cracking, privilege escalation, arbitrary execution, file hiding, track coverage, and evidence concealment. 
% After accessing the system, an attacker makes use of an exploit strategy that may include malware, sniffers, social engineering, \ac{dos}, session hijacking, application hacking, \ac{sql} injection, wireless hacking etc.
% Evasion techniques as well as effective techniques to get information out of a compromised computer network fall into the backpropagation block.
% In contrast to the attacker model, the defence model addresses attack techniques and the attack surface of the system in an early stage. 
% Afterwards, analysis of attacker strategies and capability comes into play. 
% Attacker strategies determine the attacks on the target asset and unveil attack propagation through several attack surfaces. 
% These results permit to conclude on attacker capabilities.


% Attack surface analysis from security perspective, introduced by sub-figrue \ref{fig:attackerview} (b), maps attacker goals to attack functions. 
% Possible attack functions such as internal or external function falsification/interruption or communication compromise lead to different attacks on assets. 
% Attacks on assets in turn depend on attacker capability.
% This approach considers threat vectors which eventually lead to the desired goal. 
% Therefore, threat vectors set the boundaries an attacker must follow.



% The hacker view represents the kill chain attacker view model and the attack surface analysis together with out attack vector identification enable attack tree construction \cite{al2016cyber}.
% versus attack goal analysis during attack surface analysis of \cite{maple2019connected}. 
%% !TODO: subfigures need to be references correctly if they stay

% \subsubsection{Defender view}
% \todo{introduce ASIL}











\subsection{General Attack Surface in the \ac{iov}}
\label{attacksurfacecategorization}

To access the holistic infrastructure of the \ac{iov}, works such as \cite{sun2017attacks} and \cite{butt2018social} first describe the general structure of the \ac{iov} in form of physical components, before categorizing the interaction between software components. 
The first description provides a physical separation which allows to apply more detailed analysis. 
In both descriptions, the works incorporate perspectives on logic as well as process communication to the original physical or developer context.
From the logical and developer perspective, the works \cite{iqbal2018context}, and \cite{zou2017research} further categorize the \ac{iov} software surface towards data and security specific modules.
Subsection \ref{relatedwork-iovsecurityframeworks} discusses and compares our security framework against the works we mention in this section. The comparison criteria of the related work analysis regarding these works focuses on security framework characteristics.
To continue with the \ac{iov} attack surface, the work \cite{maple2019connected} provides a comprehensive \ac{iov} reference architecture which considers a physical \ac{iov} infrastructure consisting of four sub-architectures of \ac{cav}s, devices and peripherals, edge, and cloud. % considers a functional-communication viewpoint
Their reference architecture for attack surface analysis is based on a functional-communication viewpoint which creates feasible complexity and manages incorporation of security relevant details.


Our work takes this attack surface analysis as the initial \ac{iov} reference architecture.
The attacker interference opportunities regarding the four sub-architectures defined by Maple \cite{maple2019connected} can be seen in Figure \ref{fig:referenceArchitecture}.
Facing the initial attack surface, an attacker has multiple options in attacking the cloud, infrastructure and edge, vehicle, and peripherals domains.
The attacker may either compromise hardware components or communication interfaces to gain software access of a sub-architecture.
For instance, telematic illusion and time travelling attacks corrupt peripherals, exfiltration, infiltration, and maliciously authentic data attacks compromise vehicle hardware modules, and fully adversarial networking and medium observer attacks affect communication \cite{petit2014revisiting}.
The attack surface might change at every propagation stage of the attack path.
Thereby, attacking capability and scope of the attacker model remain the dominating properties for determination of the depth of the attack surface \cite{de2014security}. 
To keep the focus on \ac{iov} security and even though humans count as another omnipresent attack surface, we do not consider social hacking attacks in this work as it applies in every system. 
% attack surface new
\begin{figure}[!ht]
\centering

\begin{adjustwidth}{0.5em}{}

    \begin{tikzpicture}[scale=0.9]
    
        \node (attckr) at (-0.25,-0.5) [transform shape = true, anchor=west] {Attacker};
        \Ninja[3];
    
        \node (cl1) at (2,2.75) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {HW: Cloud};
        \node (cl2) at (2,3.25) [rectangle, thick, draw=black, fill=white!90!blue, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {SW: Cloud};
        
        \draw pic[scale=0.2,transform shape = true] (server1) at (6.4,3.1) {server={black!30!white}{white!30!blue}{white!60!blue}};
        \draw pic[scale=0.2,transform shape = true] (server1) at (6.4,2.5) {server={black!30!white}{white!30!blue}{white!60!blue}};
        
        \draw pic[scale=0.2,transform shape = true] (switch1) at (5.7,2.9) {switch={black!10!white}{}};
        \draw pic[scale=0.2,transform shape = true] (switch2) at (5.2,2.9) {switch={black!10!white}{}};
        \draw pic[scale=0.2,transform shape = true] (switch3) at (5.55,3.15) {switch={black!10!white}{}};
    
        \node (ifra1) at (2,0.75) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {HW: Infra \& Edge};
        \node (ifra2) at (2,1.3) [rectangle, thick, draw=black, fill=white!90!blue, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {SW: Infra \& Edge};
        
        \draw pic[scale=0.1,transform shape = true] () at (5.27,1.25) {satelite={white!30!gray}{}};
        \draw pic[scale=0.2,transform shape = true] () at (5.9,2) {cellularsite};
        \draw pic[scale=0.25,transform shape = true] () at (6.5,1.35) {fuelcharge};
        \draw pic[scale=0.25,transform shape = true] () at (6,0.75) {trffclight={red}{yellow}{green}};
        \node (veh1) at (2,-1.25) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {HW: Vehicle};
        \node (veh2) at (2,-0.75) [rectangle, thick, draw=black, fill=white!90!blue, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {SW: Vehicle};
        
        \draw pic[scale=0.17,transform shape = true] () at (5.65,-1.3) {mybus={yellow}{blue!10}{black!60!green}};
        
        \node (per1) at (2,-3.3) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {HW: Peripherals};
        \node (per2) at (2,-2.75) [rectangle, thick, draw=black, fill=white!90!blue, minimum width=3cm, minimum height=0.5cm, transform shape = true, anchor=west] {SW: Peripherals};
        
        \draw pic[scale=0.5,transform shape = true] () at (5.45,-3) {person};
        \draw pic[scale=0.2] () at (6.35,-2.7) {antenna};
        \draw pic[scale=0.14] () at (5.75,-3.4) {smartphone={}} ;
        \draw [-] (cl1.west) --++(-0.25,0) -- ++(0,-2) -- (ifra1.west);
        \draw [-] (veh1.west) --++(-0.25,0) -- ++(0,-2.05) -- (per1.west);
        \path (3.5,0.4) edge [decoration={expanding waves,angle=60,segment length=2mm},decorate,draw,color=black] (3.5,-0.4);
        \path (3.5,-1.6) edge [decoration={expanding waves,angle=60,segment length=2mm},decorate,draw,color=black] (3.5,-2.4);
        \draw [->] (0,0) -- (1.25,0);
        \draw [->] (0.5,1) -- (1.25,1);
        \draw [->] (0.5,-1) -- (1.25,-1);
        \draw [->] (0.5,2) -- (1.25,2);
        \draw [->] (0.5,-2) -- (1.25,-2);
        \draw [->] (0.5,3) -- (1.25,3);
        \draw [->] (0.5,-3) -- (1.25,-3);
        \draw [-] (0.5,3) -- (0.5,-3);
    \end{tikzpicture}
\end{adjustwidth}
\caption{High Level Hardware, Software, and Communication \ac{iov} Reference Model Modified From \cite{maple2019connected}}
\label{fig:referenceArchitecture}
\end{figure}

We further simplify the sub-architecture categorization by considering the peripherals and vehicles category as one domain.
For one part, the reason for it is the wireless connectivity between \ac{v2i} and \ac{p2i} interfaces.
The connectivity requirements, for \ac{cav}s with highly dynamic properties of location and speed, apply to vehicles and peripherals in the same way.
Thus, the attack surface of routing strategies applies to both domains which justifies the grouping \cite{cheng2015routing}.
In more detail, transmission strategy (unicast, multicast/geocast, broadcast), information need (topology, position, map, path), delay sensitivity (delay-sensitive,  delay-tolerant), dimensions of scenarios (routing in 1D, 2D, and 3D), and target networks (homogeneous or heterogeneous network) determine the metrics that apply to \ac{cav}s and its appliances. 
For the other part, the attack surface analysis with the focus on the vehicle itself shows that most of the peripherals have wired connections to the \ac{can} network, and thereby, the vehicle architecture \cite{sharma2019extended}.




% continue with figure and state the dynamics and the wifi connection, then continue and sum up with scenario.
% Holistic from the beginning, therefore layered approaches to facilitate access to the complexity of architecture, then it is possible to look into reference architectures of either whole infra or parts such as in vehicle, the further guide down the amount of asset and make security analysis manageable, we apply a scenario as already indicated by the 4+1 model that helps to decompose systems with regard to their applications and from the details it is possible to build back into more larger systems

% structure like this, the architecture is very broad and that is also why most works need to layer the infrastructure in order to break down complexity. The comprehensive reference architecture of .. is the one we use in our work, we only put together the peripherals and vehicles later as they are typically part of the in vehicle network bus system

% To further reduce the complexity and to make security analysis and threat modeling possible we specify a use case in order to apply threat modeling and come up with a defence mechanism.
% Our approach picks the location services of vehicles as they are the most important ones for CAVs to work, otherwise it is not possible to drive
% explain CAV and then
% add use case section here

% explain characteristics and refer to the graph that summes up the attack surface, then state that we use the 4+1 software architectural view model in order to decompose the system in a structured way in order to be able to apply defence mechanisms at all interfaces that exist.

% the charateristics that dominate are the following, that is why the IoV requires wireless communciation which makes it hard

% \todo{reduce content of this chapter and requires better structure}

% \subsubsection{Location dynamics}
% \todo{bring it together with use case section}

% Location and speed of vehicles heavily influence the characteristics of the \ac{iov}. 
% Therefore, vehicle communication is wireless and requires very reliable, fast, and complex transmission strategies. 
% The routing taxonomy of Cheng et al. groups routing protocols with regard to \ac{iov} specific metrics.
% Transmission strategy (unicast, multicast/geocast, broadcast), information need (topology, position, map, path), delay sensitivity (delay-sensitive, delay-tolerant), dimensions of scenarios (routing in 1D, 2D, and 3D), and target networks (homogeneous or heterogeneous network) belong to the pool of \ac{iov} relevant metrics \cite{cheng2015routing}. 

% \todo{this goes into scenario part to justify its importance}
% Location accuracy determines the \replaced{criticality}{critically} level of a vehicle.
% Little confidence in the vehicle location, which means a high critically level, causes either a human to interfere, or the vehicle to slow down and eventually stop.
% To prevent vehicles from stopping due to location inaccuracy and maintain a low critically level, vehicles rely on redundant location services \cite{kolb2020technische}. 
% Odometry, LIDAR, and \ac{dgps} data establish necessary localization redundancy. 
% Additionally, the comparison of local position calculations of sensor and receiver data with predetermined \ac{slam} trajectories create highly accurate location determination.

% \todo{scenario part as well}
% \subsubsection{SAE levels of driving automation}
% Our work focuses on \ac{cav}s.
% The connectivity characteristics of \ac{cav}s derive from the \ac{iov} which first of all stands for Internet connected vehicles.
% The autonomous part of \ac{cav}s describes vehicles which fall into into one of five \ac{sae} levels of automated driving.
% The five levels of driving automation classify the required interaction of a vehicle driver with the vehicle itself \cite{sae2014automated}. 
% Level zero indicates no automation and full-time interaction between a human driver and the vehicle.
% Driver assistance, partial automation, conditional automation, high automation, and full automation increase the systems automation capabilities respectively.
% Full automation expects automated steering, acceleration, deceleration, monitoring, handling of dynamic tasking, and driving modes of the vehicle system.
% Autonomous shuttles which make up the central component of the our scenarios\fmma{Scenario is still undefined. I think we must introduce it in the introduction briefly with a full scope level figure in the beginning or in the next section} target level four of driving automation.

% this automation part leads to high complexity, then justify layered architecture abstractions

% holistic infrastructure leads to multi layer modeling of the architecture \cite{contreras2017internet}

% \# holistic layers, structure: reference of end chapter ! blue layers with security
% The holistic \replaced{picture}{architecture} of an \ac{iov} infrastructure complicates the view on individual assets, attacks, and defence mechanisms. 
% Hence, \ac{iov} architecture analysis approaches evolved to utilize up to seven layers to break down complexity. 
% Our work builds upon the seven layer architecture proposal of Contreras et al. which consists of a user interface, data acquisition, filtering and preprocessing, communication, control and management, and processing layer \cite{contreras2017internet}.
% Such a layered high level view groups and describes end-user functionality and services. 
% Hence, the layered view derives an analysis model based on the metric of functionality type and connection. 
% Other metrics, such as reliability or performance, might produce a different view of the architecture. 


% \todo{great survey on attack surface: An Extended Survey on Vehicle Security}
% https://arxiv.org/pdf/1910.04150.pdf

% \todo{create new figure, top of this column}
% file:///home/jansen/Downloads/security_IETE_2013_ps.pdf

% Attack surface categorization specifies asset access possibilities based on boundaries which affect the attacker. 
% The initial boundaries on the attacker are \textit{locality} and \textit{affiliation}, and attacking \textit{expertise}.\fmma{These terms must be defined and discussed in the same order as they are introduced.}
% It is possible to exclude expertise due to worst case attacking expectations.
% Affiliation has less priority compared to locality as progressing software solutions support granular system privileges. \fmjl{TODO: reference for this claim, also possible to claim employees find more education in future}
% These boundaries on attackers find different opportunities to interface with the access levels of a system.
% Figure \ref{fig:referenceArchitecture} shows the ability of local attackers to actively interfere with user interfaces or computer hardware to launch attacks.
% Once compromised or by legally using computers, an attacker is able to execute remote attacks that allow attack propagation and malicious interaction with software and hardware.

% this allows the attacker to actively or passively interfere with attack surface
% Passive attacks\fmma{This section could be better organized by connecting the story. e.g. start with Active attacks and then come to this point} compromise assets without directly addressing assets and make up another category to interact with attack surfaces. 
% Monitoring, eavesdropping or capturing of electric currents, magnetic fields, or networking traffic mark example\added{s of} passive attacks.

% With regard to the \ac{iov}, the attack surface evolves around the comprehensive \ac{cav} reference architecture of Maple et al. \cite{maple2019connected}. 
% Here, the consideration of functional and communication viewpoints divides the attack surface into four sub-architectures of \ac{cav}s, devices and peripherals, edge, and cloud.
% Their viewpoint combination creates feasible complexity, manages incorporation of important details and justifies the omission of architectural viewpoints based on implementation, enterprise, usage, information, or physical perspectives as well as risk analysis.
% Figure \ref{fig:referenceArchitecture} \fmma{i suggest to use lucidchart for figures which is much easier to draw figures as you imagine. Just a suggestion which may save your time} summarizes the four attack surface sub-architectures with regard to communication, hardware, and software assets. % !TODO: keep updating this when it comes to use cases and new insights of architecture !!! and Table \ref{tab:referenceArchitecture} also summarizes this
% \fmma{the current write up seems like a casual draft of thoughts. This is difficult to understand at times. I hope you plan to rewrite this with better technical write up? - yes I reqrite it, and change some things of the figure as well}

%% !TODO human layer <--
% \todo{
% -- Human Layer around everything
% }


%% !TODO attack tree, and attack probability modelling/risk evaluation for more detailed attack surface analysis <--
% \todo{
% -- Attack Tree as methodology among other threat/modeling approaches to get more detailed attack surface analysis
% }


%% IDEA: put this figure into scenario use case view



% I guess this table can be removed !? don't like it too much
% \begin{table}[htbp] % [!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Software Summary of \ac{cav} Reference Model \cite{maple2019connected}}
% \label{tab:referenceArchitecture}
% \centering
% \begin{tabular}{|p{2cm}|c|c|c|c|}
% \hline
% \textbf{Software} & \textbf{Cloud} & \textbf{Infra \& Edge} & \textbf{Vehicle} & \textbf{Peripherals} \\
% \hline
% \hline
% Sensors & & x & x & x \\
% \hline
% Infotainment & & & x &  \\
% \hline
% Human Machine Interface (HMI) &  &  & x & \\
% \hline
% Physical Input \& Output &  & x & x & x \\
% \hline
% Actuators &  & x & x & \\
% \hline
% Wired Communications & x & x & & \\
% \hline
% Wireless Communications &  & & x & x \\
% \hline
% Data Storage & x & x & x & x \\
% \hline
% Data Analysis & x & x & x & \\
% \hline
% Applications & & & & x \\
% \hline
% Microservices & x & x & & \\
% \hline
% Monitoring & x & x & x &  \\
% \hline
% Energy System &  & x & x & \\
% \hline
% \end{tabular}
% \end{table}



% car keys, environment and infrastructure devices and peripherals, radio masts, cloud servers, edge devices, third party vehicles, drivers, and passengers make up infrastructure components and stakeholders.

%% older reference ---
% Among smart home, smart industry, and smart health etc., the smart transportation domain which includes the \ac{iov} belongs to the \ac{iot} \cite{kaiwartya2016internet}.
% As a consequence, attack surface surveys of the \ac{iot} provide the high level overview of cybersecurity attack surface.
% The analysis of multiple multi-layer \ac{iot} reference models identifies physical objects, protocols, data, and software as main attack surface categories \cite{abdul2018comprehensive}.  % which can be seen in figure .. where we included the mapping 
% Physical objects differentiate between constrained and unconstrained devices which refers to physical hardware capacity.

% categories, protocols explain my tree draw.io list, refer back to layer chapter, 

% - Nils IoT smart home paper
% - IoT attack surface




% interception (eavesdrop), interruption (dos), modification (), fabrication (impersonation, replay) % A Survey of Man In The Middle Attacks 2016 paper

% \subsection{IoV Characteristics \& \ac{cav}s}
% \subsubsection{Location dynamics}
% \todo{bring it together with use case section}

% Location and speed of vehicles heavily influence the characteristics of the \ac{iov}. 
% Therefore, vehicle communication is wireless and requires very reliable, fast, and complex transmission strategies. 
% The routing taxonomy of Cheng et al. groups routing protocols with regard to \ac{iov} specific metrics.
% Transmission strategy (unicast, multicast/geocast, broadcast), information need (topology, position, map, path), delay sensitivity (delay-sensitive, delay-tolerant), dimensions of scenarios (routing in 1D, 2D, and 3D), and target networks (homogeneous or heterogeneous network) belong to the pool of \ac{iov} relevant metrics \cite{cheng2015routing}. 

% Location accuracy determines the \replaced{criticality}{critically} level of a vehicle.
% Little confidence in the vehicle location, which means a high critically level, causes either a human to interfere, or the vehicle to slow down and eventually stop.
% To prevent vehicles from stopping due to location inaccuracy and maintain a low critically level, vehicles rely on redundant location services \cite{kolb2020technische}. 
% Odometry, LIDAR, and \ac{dgps} data establish necessary localization redundancy. 
% Additionally, the comparison of local position calculations of sensor and receiver data with predetermined \ac{slam} trajectories create highly accurate location determination.


% \subsubsection{SAE levels of driving automation}
% Our work focuses on \ac{cav}s.
% The connectivity characteristics of \ac{cav}s derive from the \ac{iov} which first of all stands for Internet connected vehicles.
% The autonomous part of \ac{cav}s describes vehicles which fall into into one of five \ac{sae} levels of automated driving.
% The five levels of driving automation classify the required interaction of a vehicle driver with the vehicle itself \cite{sae2014automated}. 
% Level zero indicates no automation and full-time interaction between a human driver and the vehicle.
% Driver assistance, partial automation, conditional automation, high automation, and full automation increase the systems automation capabilities respectively.
% Full automation expects automated steering, acceleration, deceleration, monitoring, handling of dynamic tasking, and driving modes of the vehicle system.
% Autonomous shuttles which make up the central component of the our scenarios\fmma{Scenario is still undefined. I think we must introduce it in the introduction briefly with a full scope level figure in the beginning or in the next section} target level four of driving automation.















\section{Related Work}
\label{relatedwork}

% chapter 4 section C into related work,
% Same for 5 b first paragraph


\subsection{Threat Modeling in the \ac{iov}}

% \todo{reference A Review of Threat Analysis and Risk Assessment Methods in the Automotive Context}

The \ac{iov} represents a playground where many threat modeling approaches apply at different development lifecycles.
In order to locate our work, the comparison with the threat modeling concept of Zhendong et al. \cite{ma2016threat} outlines relations in the concept and product development phase.
Their systematic threat modeling overview applies threat modeling on high level system design in the concept phase of the development lifecycle. 
Derived high level security requirements and concepts extend the threat knowledge base and mitigation catalogue.
In the development phase, threat modeling adds technical security requirements, validation, and verification procedures to the mitigation catalogue. 
Here, threat modeling analyzes detailed system design implementation details. 
The structures of the systematic threat modeling approach of \cite{ma2016threat} derive from the prominent \ac{iso26262} \cite{iso201126262} and \ac{saej3061} \cite{vcse2016j3061} standards which define a combination of \ac{tara} and \ac{stride} for risk assessment.
Our work relates in the way, that it analyzes high level as well as in depth implementation details and modules of the \ac{iov} architecture through the 4+1 view model analysis.
Likewise, we identify security requirements of assets and provide a methodology to validate and verify security requirement effectiveness.
In contrast to the work \cite{ma2016threat}, our risk analysis methodology differentiates by considering vulnerability, attacker, and defence mechanism characteristics at different attack propagation stages.


The work of Xiong et al. \cite{xiong2019threat}, as the main related work, enhances threat modeling with probabilistic attack simulations that are based on networking graphs with attack paths. 
Their work builds upon the in-vehicle 2014 Jeep Cherokee \ac{can} network model of \cite{miller2014survey} and utilizes the software tool securiCAD for automated attack modeling and risk assessment.
The attack simulations based on the attack path incorporate attack types, vulnerabilities, and countermeasures at every propagation stage and manage to evaluate \ac{ttc} behavior.
Among others, the findings of this work demand more tailored definitions of meta-models or reference architecture, further investigation of countermeasures, a design of a security architecture, validation of the approach through case studies, and quantitative input to the quantitative and probabilistic security metric of \ac{ttc}.
To address the outcomes of \cite{xiong2019threat}, our work reproduces their enhanced threat modeling concept with the following changes.
Regarding the meta models and reference architecture, we leverage the outcomes of the \ac{iov} reference model architecture analysis of \cite{maple2019connected}. 
Based on the proposed reference model, we apply the 4+1 view model to further break down assets to extract detailed vulnerability properties.
The scenario definition specifies the use case study.
For the security requirement analysis, attacker modeling, and risk assessment, we stick with the most used \ac{stride} model and \ac{cvss} scores.
The last input to our risk assessment, next to the attack propagation state which reveals the asset under attack, is the \ac{siem} security defence concept, which we explain in Section \ref{secdefs}.  
After the risk assessment, we propose a comprehensive and high level security methodology to cover the points of security architecture design and verification.
With the security methodology, it is possible to investigate countermeasures as well. 
Moreover, we are able to deliver quantitative input into our probabilistic security verification model, that strongly aligns with the model of \cite{cheng2012research}, to validate our case study/scenario. 
The scope of our threat modeling approach relates to the ideas of comprehensive threat modeling of \cite{pacheco2016iot}.

% Threat modeling in the IoV without holistic security framework \cite{xiong2019threat}
% this way get complete threat modeling coverage until handling threats as proposed by \cite{pacheco2016iot}
% \# 3 paragraph
% Reference Architecture paper with wifi Tesla exploit and parking valet scenario \cite{maple2019connected}

% With regard to the \ac{iov}, the attack surface evolves around the comprehensive \ac{cav} reference architecture of Maple et al. \cite{maple2019connected}. 
% Here, the consideration of functional and communication viewpoints divides the attack surface into four sub-architectures of \ac{cav}s, devices and peripherals, edge, and cloud.
% Their viewpoint combination creates feasible complexity, manages incorporation of important details and justifies the omission of architectural viewpoints based on implementation, enterprise, usage, information, or physical perspectives as well as risk analysis.

% \subsection{CAV Scenarios \& Attacks}

\subsection{\ac{iov} Security Frameworks and Approaches}
\label{relatedwork-iovsecurityframeworks}

% The section summarizes design decisions of security frameworks for the \ac{iov}. 
The proposed social \ac{iov} architecture of Butt et al. \cite{butt2018social} utilizes a layered approach to outline interdependencies of the architecture. 
Their architecture stacks physical, gateway, fog, and cloud layer on top of each other. 
Next to the high level reference model, social relationship, security and privacy, and trust management connect to all layers of the stack. 
On the other hand, application and user layer extend and affect each stack layers additionally. 
The separation of domains allows the analysis of each domain itself where again layers separate the top layer subsystems. The vehicle layer for instance differentiates between physical, in-vehicle, processing, and application layers in the physical subsystem. The gateway layer specifies integration, middleware, and application layer for its subsystem.
Their framework design allows the application of security concepts to each individual layer of subsystems as well as top level layers of different domains.


The work of Iqbal et al. \cite{iqbal2018context} describes the transition of the traditional \ac{iov} architecture into a data-driven-intelligent framework. 
Again, the traditional architecture consists of an interplay of data source (vehicle, sensors), communication, fog, and cloud layer \cite{sun2017attacks}. 
Their data-driven framework translates the architecture into data collection, preprocessing, data analytics, service, and application layers. 
Security, Privacy, and trust management affect all layers as well.
Last, the approach of Zou et al. \cite{zou2017research} proposes an architecture that keeps a security monitoring system, threat intelligence, and networking security modules at the bottom layer. 
Validation and verification services build on top of the lowest layer. Defence, reinforcement, and response systems complete their so called 360 connected vehicle safety framework.


In contrast to the mentioned approaches and frameworks, the reference model selection and 4+1 architecture view model drives the two main concepts of our security methodology. 
The first abstraction concept specifies the amount of sub-architectures or reference model granularity.
The second concept abstracts hardware, software, networking, and data into layers or perspectives. 
These layers apply to each sub-architecture and enable mappings between \emph{attacks}, \emph{assets}, and \emph{defence mechanisms}.
The differences of our model with regard to the other layered security frameworks is the requirement of a scenario definition. % which connects the \ac{siem} security approach to \ac{iov} operators.
The scenarios guide the security analysis, assessment, and resulting security design towards quantitative verification possibilities.
The extendibility and flexibility feature of our methodology does not apply to the related security frameworks due to their more general abstractions of layers.


% - !! good one:Social Internet of Vehicles: Architecture and enabling technologies::: Proposed SIoV architecture \cite{butt2018social} 

% - good one: contains traditional IoV architecture, proposes data driven intelligent framework and adds holistic view of proposed data driven intelligent framework \cite{iqbal2018context}

% if 2 ones not enough, check iot security infrastructures or smart home, smart city, smart transportation in general

% - not really valuable for now: A holistic cyber security implementation framework (https://www.emerald.com/insight/content/doi/10.1108/IMCS-02-2013-0014/full/html)

% - vehicle information security framework (https://dl.acm.org/doi/abs/10.1145/3058060.3058064)




% The following \ac{iov} properties derive design choices which demand permanent consideration during secure \ac{iov} system design. Most notably, \ac{iov} characteristics drive design choices of security solutions which interact closely with the existing infrastructure. 

% \underline{Dynamics of the situation} % time and location
% \underline{Decentralization} 
% \underline{Security}
% \underline{Privacy preservation}
% \underline{Scalability of the model}
% \underline{Sparsity of entities}
% \underline{A measure of Confidence}
% \underline{Incentive}


% ask sebastian about classical Safety Critical System issues
% \subsection{Computer Security}
% \subsubsection{General Security Requirements}

%  upside down
% - possible damages: 
    % - Victim does not notice attack, nor attacker, no recover - attacker wins
    % - Victim does not notice attack, but later is able to find attacker, but cannot recover - loss of attacker and victim
    % - Victim does not notice attack, nor attacker, can recover - attacker looses and victim wins
    % - Victim does not notice attack, but later finds attacker, can recover - attacker looses and victim wins
    
    % - Victim notices attacker:
    %   - options:
    %       - (active) attack back, block
    %       - (passive) hide, hide assets, isolate, 

    % noticing requires detection:
    % detection types:
    %   - monitoring
    %   - analysis of monitoring data
    %   - 
% Emanuel phases: Requirement Specification and Design, Feature Development, Integration and Production, Operation, Maintenance and Support



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% %%%%%%%%%%%%%%%%%% BACKUP %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{figure}[!ht]
% \centering
% \begin{tikzpicture}[scale=0.625]


% \draw pic[scale=1,transform shape = true] (r1) at (-5,-4) {textrect={Process View}{white!50!gray}};
% \draw pic[scale=1,transform shape = true] (r1) at (5,-4) {textrect={Physical View}{white!50!gray}};
% \draw pic[scale=1,transform shape = true] (r1) at (5,4) {textrect={Development View}{white!50!gray}};
% \draw pic[scale=1,transform shape = true] (r1) at (-5,4) {textrect={Logical View}{white!50!gray}};
% \draw pic[scale=1,transform shape = true] (r1) at (0,-1) {textrect={Scenarios}{white!50!gray}};

% \draw pic[scale=1,transform shape = true] (str) at (0,0) {street};

% \draw pic[scale=0.2,transform shape = true] (sat1) at (-4,2.5) {satelite={white!30!gray}{}};
% \draw pic[scale=0.4,transform shape = true] (cellularsite) at (-2,3.25) {cellularsite};
% \draw pic[scale=0.2,transform shape = true] (vh1) at (-0.5,1.1) {vehicle={white!50!gray}{blue!15!white}};
% \draw pic[scale=0.2,transform shape = true] (bus1) at (2,1.1) {mybus={yellow}{blue!10}{black!60!green}};

% \draw pic[scale=0.3,transform shape = true] (fuel) at (-3.6,0.5) {fuelcharge};
% \draw pic[scale=0.75,transform shape = true] (p1) at (-3.6,-0.25) {parking={P}};

% \draw pic[scale=0.5,transform shape = true] (ps0) at (4.9,2.35) {person};
% \draw pic[scale=0.75,transform shape = true] (s1) at (5.5,2.6) {busstop={B}};

% \draw pic[scale=0.21,transform shape = true] (bus2) at (-1.5,-1.9) {mybus={yellow}{blue!10}{black!60!green}};
% \draw pic[scale=0.75,transform shape = true] (s1) at (-2.5,-1.4) {busstop={B}};
% \draw pic[scale=0.5,transform shape = true] (ps1) at (-3.1,-1.625) {person};
% \draw pic[scale=0.5,transform shape = true] (ps2) at (-3.45,-1.625) {person};

% \draw pic[scale=0.5,transform shape = true] (ps3) at (4.5,-1.625) {person};
% \draw pic[scale=0.65,transform shape = true] (c1) at (5.025,-1.5) {caution={!}};

% \draw pic[scale=0.65,transform shape = true] (c1) at (3.75,0.45) {caution={!}};

% \draw pic[scale=0.25,transform shape = true] (l1) at (4.35,1) {trffclight={red}{yellow}{green}};
% \draw pic[scale=0.25,transform shape = true] (l1) at (-4.35,-2) {trffclight={red}{yellow}{green}};
% \draw pic[scale=0.25,transform shape = true] (l1) at (-4.35,1) {trffclight={red}{yellow}{green}};


% \draw pic[scale=0.25,transform shape = true] (server1) at (3,4.25) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.25,transform shape = true] (server1) at (3.5,4.25) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.25,transform shape = true] (server1) at (4,4.25) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.25,transform shape = true] (server1) at (3,3.5) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.25,transform shape = true] (server1) at (3.5,3.5) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.25,transform shape = true] (server1) at (4,3.5) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \draw pic[scale=0.3,transform shape = true] (sw1) at (0,3.5) {switch={black!10!white}{}};
% \draw pic[scale=0.3,transform shape = true] (sw2) at (1,3.5) {switch={black!10!white}{}};
% \draw pic[scale=0.3,transform shape = true] (sw3) at (0.6,4.4) {switch={black!10!white}{}};
% \draw pic[scale=1.25,transform shape = true] (clod) at (1,4) {cloud};

% % draw legend on the right side
% \draw pic[scale=1,transform shape = true] (clod) at (6.5,-0.5) {box={2.5}{4}};
% \draw pic[scale=0.2,transform shape = true] (fuel) at (7,3.1) {fuelcharge};
% \node [scale=0.75, left,transform shape = true] at (8.8,3.1) {Gas Station};
% \draw pic[scale=0.175,transform shape = true] (l1) at (7,2.61) {trffclight={red}{yellow}{green}};
% \node [scale=0.75, left,transform shape = true] at (8.8,2.6) {Traffic Light};
% \draw pic[scale=0.5,transform shape = true] (p1) at (7,2.15) {parking={P}};
% \node [scale=0.75, left,transform shape = true] at (8.8,2.1) {Parking};
% \draw pic[scale=0.5,transform shape = true] (s1) at (7,1.65) {busstop={B}};
% \node [scale=0.75,left,transform shape = true] at (8.8,1.6) {Bus Stop};
% \draw pic[scale=0.4,transform shape = true] (c1) at (7,1.1) {caution={!}};
% \node [scale=0.75,left,transform shape = true] at (8.8,1.1) {Caution};
% \draw pic[scale=0.25,transform shape = true] (sw3) at (6.7,0.6) {switch={black!10!white}{}};
% \node [scale=0.75,left,transform shape = true] at (8.8,0.6) {Switch};
% \draw pic[scale=0.2,transform shape = true] (server1) at (6.85,-0.1) {server={black!30!white}{white!30!blue}{white!60!blue}};
% \node [scale=0.75,left,transform shape = true] at (8.8,0.1) {Server};

% \end{tikzpicture}
%   \caption{4+1 View Model in IoV}
% \label{fig:41IoVscenario}
% \end{figure}


%\begin{figure}[htbp]
% \begin{figure}[htbp]
%   \includesvg{images/41viewmodel.svg}
%   \caption{"4+1" View Model of Software Architecture}
%   \label{41viewmodel}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% detailed abstract view model descriptions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% categorization of architectural components   From a view model perspective, the layered architecture    the layered view represents 

% View models categorize perspectives and analysis models regarding different metrics.
% We leverage the 4+1 view model for software architecture to break down the complexity of the holistic \ac{iov} infrastructure. Application of view models allows us to set boundaries for individual asset, attacker, and defence mechanism analysis. Figure \ref{} 

% View models thereby categorize different perspectives of the architecture.  around the infrastructure decide upon the criteria or metric of grouping architectural components.

% The physical view enables IoV architecture layers of In-Vehicle, Road Side Infrastructure, and Internet. The human layer is another layer from a security perspective which interacts with all other physical architectural layers.

% The logical view allows different layering opportunities. Common layered IoV architecture models introduce different protocol stacks. Kaiwartya et al. introduce a five layered IoV architecture which consists of perception, coordination, artificial intelligence, application, and business layers \cite{kaiwartya2016internet}.

% \subsection{View Models}

% The 4+1 view model of software architecture separates logical, development, process, and physical views. 
% But all views focus on the same scenarios \cite{kruchten19954+}. 
% Figure \ref{} shows the components of the view model.

% explain each view in more detail, who uses it and which components are used in this view
% The logical view describes end-user functionality and services. 
% It serves for system decomposition by leveraging principles of abstraction, encapsulation, and inheritance.
% The IoV use case and stakeholder requirements mark the input to the logical view.
% Abstraction, for instance, allows to connect high level architecture components such as user interfaces and data processing cloud servers.

% The process architecture utilizes requirements such as performance, availability, concurrency, distribution, integrity, fault tolerance to map logical view abstractions into the process architecture.
% Multiple abstraction layers compose the process architecture.
% The highest level connects independent logical networks of communicating processes.
% Typically, these logical networks run on top of WAN or LAN infrastructures.
% % (level 1 connection of processes from services)
% Processes, as the second level, group and control tasks based on processing load or availability. Control capabilities enable task discovery, distribution, replication, reconfiguration, start, and termination.
% Tasks, as the last level, differentiate in scope. Minor tasks cannot be uniquely identified and addressed and serve for local management requirements such as buffering, time-outs, cyclical activities.
% Major tasks implement asynchronous or synchronous inter task communication related services.
% % remote procedure calls, broadcasting, minor tasks can communicate through shared memory or rendezvous
% This way, the process view reveals messaging and process computing loads.

% Programmers and software management organize software modules of the development view.
% The development view aims to define packaged program libraries and subsystems as well as their import and export relationships.
% Rules such as partitioning, grouping and visibility shape the hierarchical layers of software modules of the development view.
% Hierarchical layers of software development decouple common low level services and supporting mechanisms such as storage, communication, and time critical resource management in a way such that higher level frameworks face simplified dependency management.
% After identification of all software elements, the development view serves as a foundation for requirement, work, cost, evaluation, and planning allocation.
% Main guiding properties of this view are reuse, portability and security.  

% The physical view model determines the physical components of computer networks, processors and interfaces.
% Non-functional system requirements such as performance, scalability, reliability, and availability drive configuration, deployment and testing decisions of various nodes.
% In essence, these properties drive hardware capacity requirements of the physical architecture.

% Finally, the scenarios define application procedures, sequences, and interactions and set the input to all model views.
% Scenarios formulate and discover architectural components and validation, verification, and illustration concepts.
% As of today, standardized tool sets and development frameworks facilitate view model implementations.


% Might be useful: inside out vs outside in (correspondance between views)

% maybe
%This paper describes and builds upon two views of the 4+1 architectural model only. The reason therefore is missing whatever....
%(This paper focuses on higher)

% one final sentence on how our work applies the view model. answer: physical view is used to categorize use case and IoV architectural components, logical view allows layering of infrastructure services, we use this view to specify defence components

% The model separates logical, development, process, and physical views to describe a CAV scenario in an IoV system environment. 




==> sections/1.2_methodology0.tex <==
% \section{Approach}

% Approach sections:


% \section{Asset Identification}
\section{4+1 View Model Analysis and Agile Threat Modeling in the \ac{iov}} % 4+1 View Model in the Threat Modeling Context
\label{section3}


To recap, this section introduces the application scenario of location services of \ac{cav}s for the 4+1 view model analysis. 
Next, it applies the agile threat model approach of Figure \ref{fig:iovthreatmodel} in each of the view model domains for analysis purposes.
Finally, subsection \ref{analysisdigest} evaluates the identified assets together with relevant threat, vulnerability, and defence requirements for an overall risk assessment per view model domain.

\subsection{\ac{iov} Scenario: Location Service of \ac{cav}s} % or Autonomous Shuttle Bus

As already stated, all views of the 4+1 view model refer to a set of scenarios.
Thus, the scenario definitions represent the first requirement in order to apply the 4+1 view model in the \ac{iov} context.
In the context of threat modeling, the scenario definitions are essential and reduce the complexity of the broad \ac{iov} infrastructure to a selection of enabling assets.
In this work, we choose the location service application of \ac{cav}s as the main scenario due to the following reasons.
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.9]

    % bottom
    \draw [<->] (1.65,-0.5) -- ++ (0,-0.2) -- ++(2.5,0) -- ++(0,0.2);
    \draw [<->] (1.35,-0.5) -- ++ (0,-0.2) -- ++(-2.5,0) -- ++(0,0.2);
    % top
    \draw [<->] (1.65,3) -- ++ (0,0.2) -- ++(2.5,0) -- ++(0,-0.2);
    \draw [<->] (1.35,3) -- ++ (0,0.2) -- ++(-2.5,0) -- ++(0,-0.2);
    % sides
    \draw [<->] (5.35,0.25) -- ++ (0.2,0) -- ++(0,1.75) -- ++(-0.2,0);
    \draw [<->] (-2.8,0.25) -- ++ (-0.2,0) -- ++(0,1.75) -- ++(0.2,0);
    % satelite car
    \draw [<->] (1.5,-0.5) -- ++(0,-0.4) -- ++(-4.7,0) -- ++(0,3.1) -- ++(0.4,0);

    \draw pic[scale=0.2,transform shape = true] () at (1,0) {mybus={yellow}{blue!10}{black!60!green}};
    \draw pic[scale=0.2] () at (1,1) {antenna};
    \path (0.55,0.4) edge [decoration={expanding waves,angle=60,segment length=2mm},decorate,draw,color=black] (-0.2,0.4);
    \path (2.25,0.4) edge [decoration={expanding waves,angle=60,segment length=2mm},decorate,draw,color=black] (3,0.4);

    \draw pic[scale=0.75] () at (0,1.5) {basestation};
    \node[text width=2cm] at (2,2) 
    {Stationary GPS Receivers};
    % \draw pic[scale=0.75] () at (3.75,-0.2) {basestation};
    % \draw pic[scale=0.5,transform shape = true] () at (-1.25,-1.25) {cloud={Cloud}{}};
    % \draw pic[scale=0.3,transform shape = true] (server1) at (-1.5,0) {server={black!30!white}{white!30!blue}{white!60!blue}};
    \draw pic[scale=0.3,transform shape = true] (server1) at (3.35,1.6) {server={black!30!white}{white!30!blue}{white!60!blue}};
    \node[text width=2cm] at (5.2,2) 
    {A-GPS Server};
    
    \draw pic[scale=0.3,transform shape = true] () at (-2.25,1) {cellularsite};
    \node[text width=2cm] at (-0.75,0.35) 
    {Stationary DGPS};
    
    % \draw pic[scale=0.3,transform shape = true] () at (0.5,-0.5) {cellularsite};
    \draw pic[scale=0.3,transform shape = true] () at (3.6,1) {cellularsite};
    \node[text width=1cm] at (4.7,0.35) 
    {Base Station};
    
    \draw pic[scale=0.15,transform shape = true] () at (-2.4,2) {satelite={white!30!gray}{}};
    % \draw pic[scale=0.15,transform shape = true] () at (4,2) {satelite={white!30!gray}{}};
    \node[text width=2cm] at (-0.75,2) 
    {Satellite};

    \end{tikzpicture}
  \caption{Physical View of \ac{cav} Location Service Scenario (A-GPS \cite{rubino2009gps}, DGPS \cite{pepe2018cors}, Cellular Internet \cite{lee2014design})}
\label{fig:physicallocation}
\end{figure}
Location accuracy contributes to the safety criticality level of a vehicle which, in turn, determines the level of driving automation of \ac{cav}s \cite{bolle2017early}.
Autonomous mini-bus shuttles of \ac{oem}s such as EasyMile, LocalMotors and Navya or trucks aim towards running on \ac{sae} driving automation level four \cite{stocker2018shared}.
Driving automation level four expects automated steering, acceleration, deceleration, monitoring, handling of dynamic tasking, and driving modes of the vehicle system.
All these services of the vehicle system heavily depend on location services.
If there is no provision of accurate location services, the safety critically level of the shuttle increases which requires interference of shuttle operators or stopping of \ac{cav}s.
As a result, without a reliable location service, the application of \ac{cav}s fails as the vehicle cannot drive safely. 


To prevent vehicles from stopping due to location inaccuracy and maintain a low safety criticality level, vehicles rely on redundant location services \cite{kolb2020technische}. 
Several processing services of odometry, \ac{lidar}, and \ac{dgps} data, as shown in Figure \ref{fig:physicallocation}, establish necessary localization redundancy. 
Additionally, the comparison of local position calculations of sensor and receiver data with predetermined \ac{slam} trajectories enhances location estimation.
All in all, the services of vehicle \ac{dgps} communication, sensor (odometry, \ac{lidar}, camera) data processing and communication, \ac{slam} trajectory comparison, and \ac{v2c} communication make up the foundation of the following view model analysis.

% \todo{this sentence to other chapter}
% All in all, we apply threat modeling, derive and evaluate our multi-layer security solution based on the following \ac{iov} relevant scenarios of location services which include services such as vehicle \ac{dgps} communication, sensor (odometry, \ac{lidar}, camera) data processing and communication, \ac{slam} trajectory comparison, and \ac{v2c} communication.

% Theoretically, \ac{cav}s do not require a driver and have the capability to detect and avoid obstacles.
% But regulatory law compliance requires vehicle guidance through attendance of an operator who is able to control the vehicle at all times \cite{pwtdc2015uk}.
% Germany's allegedly most advanced and latest road traffic law \cite{kessel2018germany}, paraphrased and formalised traffic rules from the Vienna Convention on Road Traffic which apply for the reduced environment of highway only \cite{rizaldi2015formalising}. 
% Additionally, European research projects and initiatives of other countries \cite{pwtdc2015uk} legislate pilot zones and autonomous shuttle bus projects. 
% This brings us back to today's CAV projects which run in restricted environments with lower technical challenges \cite{bolle2017early}.


% For the security analysis and derivation of a security framework, we take the location services of \ac{cav}s of the \ac{iov} as the 4+1 view model scenarios.
% In other words, we apply threat modeling, propose and evaluate our multi-layer security solution based on the following \ac{iov} relevant scenarios of location services which include services such as vehicle \ac{dgps} communication, sensor (odometry, \ac{lidar}, camera) data processing and communication, \ac{slam} trajectory comparison, and \ac{v2c} communication.



% \begin{itemize}
%     \item Vehicle DGPS communication
%     \item Sensor (Odometry, LIDAR, Cameras) data processing and communication % odometry is IMU and wheels encoder
%     \item SLAM trajectory comparison % Verifiable 
%     \item Vehicle to cloud communication
% \end{itemize}

% This initial core service is the most important service to become automated in a secure and reliable way. 
%  Moreover localization is the enabler for further automation development of reliable and secure traffic light detection and other remaining services.

% Localization is the enabler for further automation development of reliable and secure traffic light detection and other remaining services.
% Location accuracy contributes to the safety criticality level of a vehicle which in turn determines the level of driving automation of \ac{cav}s. % and little confidence in the vehicle location causes the safety criticality level to increase. 
% Next, five levels of driving automation of \ac{cav}s depend on the safety criticality level. 
% The five levels of driving automation classify the required interaction between a vehicle operator and the vehicle itself \cite{sae2014automated}. 
% A low safety criticality level lowers the driving automation level and requires either the vehicle operator or the vehicle itself to slow down or even stop.
% As a consequence and without a working location service, the application of \ac{cav}s fails. % vehicles cannot ensure a low safety criticality level which would ensure user safety.

% The remaining technical challenges for an autonomous shuttle bus are localization, traffic light/obstacle detection, legal conformance, and course determination with decreasing priority respectively from a security and safety perspective \cite{bolle2017early} \cite{kolb2020technische}. 
% Without continuous retention of the location, the safety critically level of the vehicle increases which in turn requires stopping of the vehicle. 

% To prevent vehicles from stopping due to location inaccuracy and maintain a low criticality level, vehicles rely on redundant location services \cite{kolb2020technische}. 
% Several processing services of odometry, \ac{lidar}, and \ac{dgps} data establish necessary localization redundancy. 
% Additionally, the comparison of local position calculations of sensor and receiver data with predetermined \ac{slam} trajectories create highly accurate location determination.
% Only with 
% From the security and safety perspective, technical challenges for \ac{cav}s such as an autonomous shuttle bus are localization, traffic light/obstacle detection, legal conformance, and course determination with decreasing priority \cite{bolle2017early}.
% Hence, no provision of accurate location services increases the safety critically level which requires \ac{cav}s to stop and fail.


% \todo{scenario part as well}
% \subsubsection{SAE levels of driving automation}
% Our work focuses on \ac{cav}s.
% The connectivity characteristics of \ac{cav}s derive from the \ac{iov} which first of all stands for Internet connected vehicles.
% The autonomous part of \ac{cav}s describes vehicles which fall into into one of five \ac{sae} levels of automated driving.
% The five levels of driving automation classify the required interaction of a vehicle driver with the vehicle itself \cite{sae2014automated}. 
% Level zero indicates no automation and full-time interaction between a human driver and the vehicle.
% Driver assistance, partial automation, conditional automation, high automation, and full automation increase the systems automation capabilities respectively.
% Full automation expects automated steering, acceleration, deceleration, monitoring, handling of dynamic tasking, and driving modes of the vehicle system.
% Autonomous shuttles which make up the central component of the our scenarios\fmma{Scenario is still undefined. I think we must introduce it in the introduction briefly with a full scope level figure in the beginning or in the next section} target level four of driving automation.

% Localization use cases:
% 1. communication of cameras with ECU and odometry, IMU
%     -> local vehicle location determination
% 2. GPS GNSS
% 3. Cellular communication with the internet

% \subsection{4+1 View Model of Scenarios}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Logical View::::


\subsection{Logical View Analysis}

\subsubsection{System Modeling}

The works \cite{10.1007/978-3-030-45096-0_18} and \cite{suhr2016sensor} provide a general overview of the logical software design. 
% The logical view of the location service scenario showcase the processing logic for location determination. 
Figure \ref{fig:logviewlocation} combines three detailed logical views where the top part consist of a \ac{gps} receiver tracking and vision-based object detection system. 
Thereby, vision-based tracking utilizes a 3D proposal network to feed a region based fully connected \ac{ml} fusion network which pools input based on \ac{roi}.
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.7]

    % object detection
    \node (ref1) at (0,6) [align=left, transform shape = true] {Video \\Image};
    \node (ref2) at (2.25,6) [align=left, transform shape = true] {LIDAR \\Front View};
    \node (ref3) at (4.5,6) [align=left, transform shape = true] {LIDAR \\Bird View};


    \node (netw1) at (2.25,3.1) [draw, align=left, minimum height=3cm,minimum width=7cm, transform shape = true] {\\ \\ \\ \\ \\ \\ 3D Proposal Network};

    \node (ac1) at (0,4) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Con/Deconv \\ Layer};
    \node (ac2) at (2.25,4) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Con/Deconv \\ Layer};
    \node (ac3) at (4.5,4) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Con/Deconv \\ Layer};
    
    \node (pool1) at (0,0.5) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {ROI Pooling};
    \node (pool2) at (2.25,0.5) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {ROI Pooling};
    
    \node (mid1) at (3.5,2.75) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Detection \& 3D Proposals};
    \node (pool3) at (4.5,0.5) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {ROI Pooling};
    
    \node (ac) at (2.25,-0.5) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=6.5cm, minimum height=0.5cm, transform shape = true, align=left] {Fully Connected Layer};
    
    \node (netw1) at (2.25,-0.25) [draw, align=left, minimum height=2.5cm,minimum width=7cm, transform shape = true] {\\ \\ \\ \\ \\ Region Based Fusion Network};
    
    \node (ref5) at (4.5,-2.25) [draw, thick, align=left, transform shape = true] {Object Detection};
    \node (ref6) at (0,-2.25) [align=left, transform shape = true] {Odometry};

    \draw [-] (ref1.south) -- (ac1.north);
    \draw [-] (ref2.south) -- (ac2.north);
    \draw [-] (ref3.south) -- (ac3.north);

    \draw [-] (ac1.south) -- (pool1.north);
    \draw [-] (ac2.south) -- ++(0, -0.175) -- ++(-1.75,0) -- ++(0,-2) --++(1.75,0) -- (pool2.north);
    \draw [-] (ac3.south) -- ++(0,-0.4);
    \draw [-] (pool1.north) -- ++(-0.25,0) -- ++(0,1.85) -- ++(1.75,0);
    \draw [-] (pool2.north) -- ++(0.25,0) -- ++(0,0.435) -- ++(1.75,0) -- ++(0,1.05);
    \draw [-] (pool3.north) -- ++(0,1.5);

    \draw [-] (pool1.south) -- ++(0,-0.36);
    \draw [-] (pool2.south) -- ++(0,-0.36);
    \draw [-] (pool3.south) -- ++(0,-0.36);
    
    \draw [-] (ref5.north) -- ++(0.25, 0) -- ++(0,1.2);


    \node (netw4) at (9.2,2.54) [draw, align=left, minimum height=4cm,minimum width=4.75cm, transform shape = true] {\\ \\ \\ \\ \\ \\ \\ \\ \\ GPS Receiver Tracking};
    
    \node (visio) at (4.2,-3.5) [draw, align=left, transform shape = true] {Vision-based Tracking};
    \node (intev) at (10.25,-2.25) [align=left, transform shape = true] {Inter Vehicles \\Communication \\Link};
    \node (dgps) at (10.25,-3.5) [draw, align=left, transform shape = true] {DGPS};
    \node (seudo) at (8.5,-0.5) [draw, thick, align=left, transform shape = true] {Pseudo-Range \&  \\Navigation Data};

    % inteer vehicle based teracking lines 
    \draw [-] (intev.south) -- (dgps.north);
    \draw [-] (intev.west) -- ++(-0.325,0) -- ++(0,-1.24) -- (visio.east);
    \draw [-] (pool3.south) -- ++(0,-0.36);
    
    \draw [-] (ref5.south) -- ++(0,-0.4) -- ++(-0.3,0) -- (visio.north);

    % gps receiver system
    \node (ant) at (8,6) [align=left, transform shape = true] {Antenna};
    \node (refoz) at (10.5,6) [align=left, transform shape = true] {Reference\\Oscillator};
    
    \node (ac7) at (8,4) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Amplifier \& \\ Converter};
    \node (ac8) at (10.5,4) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Frequency \\ Synthesizer};
    
    \node (catc) at (8,2) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Code \\ Tracking \\ Channel};
    \node (cotc) at (10.5,2) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Carrier \\ Tracking \\ Channel};
    
    \draw [-] (ant.south) -- (ac7.north);
    \draw [-] (refoz.south) -- (ac8.north);
    
    \draw [-] (ac7.east) -- (ac8.west);
    
    \draw [-] (ac7.south) -- (catc.north);
    \draw [-] (ac7.south)  -- ++(0,-0.25) -- ++(2.25,0) -- ++(0,-0.6);
    \draw [-] (ac8.south)  -- ++(0,-0.1) -- ++(-2.25,0) -- ++(0,-0.75);
    \draw [-] (ac8.south) -- (cotc.north);
    
    \draw [-] (cotc.west) -- (catc.east);
    \draw [-] (cotc.west) -- ++(0,-0.25) -- ++(-1,0);
    
    
    \draw [-] (seudo.south) -- ++(0,-2.35) -- ++(-2.55,0);
    \draw [-] (seudo.south) -- ++(-0.175,0) -- ++(0,-2.64) -- ++(1.35,0);
    \draw [-] (catc.south) -- ++(-0.65,0) -- ++(0,-1.15) -- ++(1,0) -- ++(0,-0.2);
    \draw [-] (cotc.south) -- ++(0.55,0) -- ++(0,-1.15) -- ++(-2,0) -- ++(0,-0.2);
    
    % to multi fusion sensor
    \node (msf) at (5,-5) [draw, thick, align=left, transform shape = true, fill=white!70!gray, minimum height=1cm] {Multi Sensor Fusion};
    \draw [->] (msf.south west) -- ++(0,-1) node [midway, transform shape = true, right=0.025cm] (txt20) {Altitude};
    \draw [->] (msf.south east) -- ++(0,-1) node [midway, transform shape = true, right=0.025cm] (txt21) {Velocity}; % above, sloped
    \draw [->] (msf.south) -- ++(0,-1) node [midway, transform shape = true, right=0.025cm] (txt22) {Position};
    
    \draw [-] (dgps.south) -- ++(0,-1.25) -- (msf.east);
    \draw [-] (ref6.south) -- ++(0,-2.47) -- (msf.west);
    \draw [-] (visio.south) -- ++(0,-0.35) -- ++(0.8,0) -- (msf.north);

    \end{tikzpicture}
  \caption{Logical View of GPS Receiver Tracking System \cite{navstar1996user}, Sensor Data Processing \cite{chen2017multi}, and Vehicle Localization Components \cite{vetrella2016differential}.}
\label{fig:logviewlocation}
\end{figure}
\ac{lidar} front and bird view data as well as video images pass convolution, deconvolution, and initial object detection and 3D proposal layers to feed \ac{roi} pooling modules of region based fusion processing part.


The \ac{gps} receiver tracking system amplifies and converts \ac{gps} signals and relays them to the code tracking and carrier tracking channels. 
To determine the travel time of the signal, the receiver compares pseudo random codes. 
The code tracking channel compares the internally generated CA/code from the reference oscillator with the exact same code that is inside the satellite signal.
High correlation through code synchronization techniques cannot ensure high precision travel time estimation due to the fact that pseudo random codes have cycle widths of up to a millisecond. 
The speed of light passes up to 300 meters in one millisecond.
To enhance code phase signal travel time estimation, the thousand time faster carrier phase comparison improves precision. 
Here, the code phase correlation result marks the starting point for the carrier phase to count carrier cycles. The remaining carrier phase ambiguity requires investigation to detect the carrier cycle that represents the edge of the timing pulse.
In cases of unreliable \ac{gps} signal reception, location services need to rely on predictive \ac{dgps} carrier phase corrections \cite{indriyatmoko2008artificial}.


% how is SLAM data used and where does it enter the logical model?


The lower part of the logical view indicates a multi sensor fusion system which processes the results of vision-based tracking, \ac{gps} tracking, \ac{dgps} correction, and odometry data to determine high precision altitude, position, and velocity values.
The combination of \ac{lidar} point cloud and odometry data allow Kalman filter estimation of particle motion between \ac{lidar} scans. 
Next, it is possible to decide on different cost functions for point cloud matching between the estimated live \ac{lidar} scans and the \ac{slam} predefined point cloud map \cite{xu20173d}. 
The widely used \ac{ndt} matching approach applies a gaussian probability density function to every point of the \ac{slam} point cloud map and constructs a 3D grid coordinate. 
% maybe functions here
The result of a transformation parameter applied to the point cloud of \ac{lidar} 3D data marks the input to the state density function.
The next step is to solve the maximum likelihood of the state density function by applying an optimization algorithm that adapts the transformation parameter. 
The resulting transformation parameter does not directly represent the distance between map and scan points. It represents the distance between the best possible surface matches which achieves high precision localization offset \cite{qingqing2019multi}.
Point cloud matching moreover allows detection of anomalies which can trigger corrupted map reconstruction or improvement procedures of lacking map data.



\subsubsection{Threat \& Vulnerability Analysis}
\label{datathreatvulnerability}

To be able to calculate the common vulnerability score for the logical view software layer, we first gather the threats that threaten the identified \emph{assets} of the logical view. 
Logical software design, which describes the basic structure of data relationships and, thereby, application logic, represents a part of software system design \cite{teorey2011database}.
Out of the vulnerabilities taxonomies collection of \cite{igure2008taxonomies}, the \ac{risos} \cite{abbott1976security} and \ac{pa} project \cite{bisbey1978protection}, which describe software operating system flaws, apply to any other system design challenges as well. 
The reason for this is that operating systems require and depend on holistic system design modeling.
All possible software data flaws of the referenced collection affect the identified \emph{assets} of Figure \ref{fig:logviewlocation}.
For instance, incomplete or inconsistent parameter validation, privileges, identification, authentication, authorization, serialization, or exploitable logic errors mark vulnerabilities of the logical view domain.
By violating the software data vulnerabilities, an attacker may perform one or multiple \ac{crud} operations on the data.
Data manipulation represents the ultimate target of an attacker to compromise the location services of a vehicle.


%% VULNERABILITY TAXONOMIES
% The closest taxonomy which reveals system de of \cite{igure2008taxonomies}


\subsubsection{Risk Analysis \& Security Requirements}

To perform risk analysis in the software data layer and since the \ac{stride} security requirements are part of the \ac{cvss} base metric, we first check to what extend the \ac{stride} security requirements apply.
With the help of the threat and vulnerability analysis of the previous Section \ref{datathreatvulnerability} and the logical view analysis, we determine the \ac{cvss} metric using Table \ref{tab:cvssscores}.
This table indicates our decisions on \ac{cvss} parameters that we prove in Section \ref{analysisdigest}.
The outcome of the final \ac{cvss} score is $21.1$.
Further security requirements next to the \ac{stride} software metrics are the application of security by design best practices into the logical design and the incorporation of incident detection procedures. 
Incident detection and reaction evaluation is out of scope of this work and remains future work. 
Nevertheless, our final framework provides the possibility to include defence mechanism probabilities.


\subsubsection{Security Considerations}

Based on the outcomes of the logical view analysis, a tailored security design from the logical perspective first of all needs to minimize the number of components and functionality requirements which belong to security by design concepts \cite{bishop1995taxonomy}. 
Other preventive measures such as error handling, of consistency of data over time, authentication, validation, modularity, exposure etc. require consideration and need incorporation into the logical design of the application scenario \cite{igure2008taxonomies}.
For detective and reactive measures, the logical design must detect logic bomb injections which would intentionally hide, delete, or start processes that affect application logic.




% • Violable prohibition or limiting and exploitable logic
% error
% The ten classes from the PA project were:
% • Consistency of data over time
% • Validation of operands, residuals, naming, domain
% • Serialization
% • Interrupted atomic operations
% • Exposed misrepresentations
% • Queue management dependencies
% • Critical operator selection error mark vulnerabilities of the logical view domain.

% \todo{prevention, detection, and reaction per view model context}




%%%%%


% % base metric
% Access Vector = Remote,  exploitable remotely (and possibly locally as well)
% Access Complexity = High, protected with software library, security by design, authentication, detection, timing detection of sensor input etc...
% Authentication = Required, assume communication in vehicle use pki 
% Confidentiality Impact = Partial, video data of street
% Integrity Impact = Partial, difficult to ensure integrity of sensors values, as camera is source of trust.... if this is compromised, nothing you can do except to check value boundaries... 
% Availability Impact = Partial, if compromised module, this can be taken down, but gps might continue to work...
% Impact Bias = integrity
% in infotainment for ex, this parameter would rather be normal! cause it needs to protect all three requirements
% % temporal
% exploitability = Proof of Concept (paper about sensor confusion, have one, or gps jamming, 3G jamming), not functional cause gps jamming and hacking appears to be difficult
% Remediation Level = Temporary Fix, possible to detect and temporal fix
% report confidence = Uncorroborated:  Multiple non-official sources; possibly including
% independent security companies or research organizations
% % environment
% Collateral Damage
% Potential = high, location data wrong and wrong maneuvre might damages operator
% Target Distribution = medium, as location service is part of infra and vehicel and little cloud (not really dangerous for operator anymore)


% BaseScore = round to 1 digit of 10
% * ( 1.0 )
% * ( 0.8 )
% * ( 0.6 )
% * ( (0.7 * 0.25 ) + ( 0.7 * 0.5 ) + ( 0.7 * 0.25 ) )

% total base score = 3,3

% TemporalScore = round to 1 digit of BaseScore
%  * ( 0.9 )
%  * ( 0.90 )
%  * ( 0.95 )
 
% temporal score = 2,5

% EnvironmentalScore = round to 1 digit of (TemporalScore + (10 -
% TemporalScore)
% * (0.5))
% * (0.75)

% environmental score = 5,3

% BS = 10*1*1*1*(0.7*0.25+1*0.5+0.7*0.25) = 8.5
% TMP = BS*0.9*0.9*0.95 = 6.5
% ENV = (tmp + (10-tmp)*0.5)*0.75 = 6.1


% BaseScore = round to 1 digit of 10
% * (case AccessVector of local: 0.7 remote: 1.0)
% * (case AccessComplexity of high: 0.8 low: 1.0)
% * (case Authentication of required: 0.6 not-required: 1.0)
% * ((case ConfidentialityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.5 INTGRTY:
% 0.25 AVLBLTY: 0.25)
% + (case IntegrityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.5 AVLBLTY : 0.25)
% + (case AvailabilityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.25 AVLBLTY : 0.5))


% TemporalScore = round to 1 digit of BaseScore
%  * (case Exploitability of unproven: 0.85 proof-of-concept: 0.9
% functional: 0.95 high: 1.00)
%  * (case RemediationLevel of official-fix: 0.87 temporary-fix: 0.90
% workaround: 0.95 unavail: 1.00)
%  * (case ReportConfidence of unconfirmed: 0.90 uncorroborated: 0.95 confirmed:
% 1.00)

% EnvironmentalScore = round to 1 digit of (TemporalScore + (10 -
% TemporalScore)
% * (case CollateralDamagePotential of none: 0 low: 0.1 medium: 0.3 high:
% 0.5))
% * (case TargetDistribution of none: 0 low: 0.25 medium: 0.75 high:
% 1.00)




% the maximum likelihood of the transformation parameter produces the optimal transformation vector which moves 
% With the grid state density function of every map point, it is possible to input \ac{lidar} 3D point cloud data to the density function and calculate the maximum likelihood with regard to a transformation parameter.
% With the maximum likelihood transformation function for \ac{lidar} 3D point cloud data and the transformation parameter  

% of estimation values derived from live sensor data with data of the \ac{slam} predefined map   \cite{xu20173d}
% The matching of real-time and live sensor data with data of the \ac{slam} predefined map evaluates cost functions  to update cost function weight parameters for particle evaluation. Particle Motion and maneuver prediction in particle filters moreover depends on odometry data \cite{xu20173d}.     of cost functions which updates cost functions which contribute to  3D \ac{lidar} point cloud data with \ac{slam} point cloud data plays another important role to improve localization precision \cite{qingqing2019multi}.
% https://opus.bibliothek.uni-wuerzburg.de/opus4-wuerzburg/frontdoor/deliver/index/docId/14449/file/Houshiar_Thesis_WFRT12.pdf
% localization chapter to explain where SLAM is used

% idea, sum up logical views into one large logical view.... 3 pictures together

% carrier phase processing, .

% In cases of unreliable \ac{gps} signal reception, location services need to rely on predictive \ac{dgps} carrier phase corrections \cite{indriyatmoko2008artificial}. 
% Next, odometry sensor data and trajectory calculation allow for location determination... or sensor information that deliver odometry data for trajectory maintenance .

% (a) for dgps
% (b) for sensor
% (c) SLAM data trajectories =? how does the collection and comparison work

% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5191143/

% sensor analysis on data camera, radar, LIDAR, GPS, Ultrasonic, object detection architecture, thats part of adaptive autosar applications



\subsection{Developer View Analysis}

% malware
% https://ieeexplore-ieee-org.eaccess.ub.tum.de/stamp/stamp.jsp?tp=&arnumber=8746516

\subsubsection{System Modeling}

%% IN VEHICLE ::::::::::::
% software developer view important, because it gives attacker hints on what software and which version is currently installed, zero days. 
The software implementation of location services builds upon the software architecture stack of the \ac{autosar} Classic Platform and the \ac{autosar} Adaptive Platofrm which structure software libraries, dependencies and interactions \cite{furst2016autosar}. 
The classic version of \ac{autosar} applies to deeply embedded systems that focus on safety, real-time capability and process determinism whereas the adaptive platform high-end computing in form of customer applications targets. 


% describe both architectures
The classic \ac{autosar} software architecture divides into four main layers. 
On top of the microcontroller layer, which groups \ac{ecu} hardware, the basic software layer as well as the \ac{autosar} runtime environment abstract hardware functionality through software modules. The top level application layer utilizes the runtime environment for software and application module communication \cite{warschofsky2009autosar}. 
Equal to the classic \ac{autosar} architecture, the adaptive \ac{autosar} software architecture builds the adaptive \ac{autosar} foundation of on top of a virtual machine/hardware layer.
The adaptive \ac{autosar} foundation consists of several \ac{api}s and services for \ac{os}, time, execution, communication, configuration, security, and monitoring management.
This layer enables the \ac{ara} to expose these \ac{api}s to applications that run on top of \ac{ara} \cite{furst2016autosar}.


Regarding the software architecture of the cloud, infrastructure and edge reference architecture, the works \cite{bertaux2015software} and \cite{zhang2017carstream} introduce recent software networking stacks and cloud software architecture stacks respectively. 
Even though these software assets provide potential entry points for an attacker to attack the location services of vehicles, we leave this analysis as future work due to prioritization decisions.

% Question? graph necessary here???
% \todo{CLOUD SOFTWARE STACK :::  maybe not to important for location scenario use case, but for attacking important as attacker can attack from both sides \cite{}
% }
% \todo{SATELLITE NETWORKING SOFTWARE STACK :: Software Defined Networking and
% Virtualization for
% Broadband Satellite Networks 
% } \cite{bodas2011cosp}, \cite{bertaux2015software}

\subsubsection{Threat \& Vulnerability Analysis}

Since the developer view is part of the software context, it is possible to consider the traditional software threats of the \ac{stride} model.
Additionally, the software vulnerability taxonomy of \cite{tsipenyuk2005seven} lists input validation and representation, \ac{api} abuse security features time and state, errors, code quality, encapsulation, and environment as flaws.
These software flaws clearly focus on implementation and software library modules and do not consider weak spots of data and system design.
All the stated flaws apply to the software architecture module analysis identified by the developer view in the previous section.

\subsubsection{Risk Analysis \& Security Requirements}

Again and with the help of the asset analysis of the developer view and the software vulnerability taxonomy, we determine the \ac{cvss} parameters of the software implementation layer in Table \ref{tab:cvssscores}. 
The risk analysis with the \ac{cvss} score gives a final score of $8.1$ for the software layer analysis for the location service scenario.


\subsubsection{Security Considerations}

Tailored security design in the software domain of the developer view analysis concerns safe development, implementation, verification, testing, deployment, and maintenance of services such as interoperability, dynamic and automated risk assessment, attack prediction and attribution, threat predictive analytics, monitoring, and detection intelligence, encrypted traffic analysis, forensic readiness, intrusion detection and prevention, and penetration testing \cite{rao2017probabilistic} \cite{cheng2018encrypted} \cite{haas2017intrusion}.
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.9]

    \node (el11) at (0,2) [rectangle, anchor=center, thick, draw=black, fill=white!90!gray, minimum width=6cm, minimum height=0.5cm, transform shape = true] {GNSS Data Reception (A-GPS, DGPS)};
    \node (el12) at (0,1) [rectangle, anchor=center, thick, draw=black, fill=white!90!gray, minimum width=6cm, minimum height=0.5cm, transform shape = true] {Vision-based Tracking};
    \node (el13) at (0,0) [rectangle, anchor=center, thick, draw=black, fill=white!90!gray, minimum width=6cm, minimum height=0.5cm, transform shape = true] {Odometry(IMU) Trajectory Estimation};
    \node (el14) at (0,-1) [rectangle, anchor=center, thick, draw=black, fill=white!90!gray, minimum width=6cm, minimum height=0.5cm, transform shape = true] {Visual Scan and SLAM Map Matching};
    \node (el15) at (0,-2) [rectangle, anchor=center, thick, draw=black, fill=white!90!gray, minimum width=6cm, minimum height=0.5cm, transform shape = true] {Location Data Communication};
    
    \draw [->] (el11.south) -- (el12.north);
    \draw [->] (el12.south) -- (el13.north);
    \draw [->] (el13.south) -- (el14.north);
    \draw [->] (el14.south) -- (el15.north);

    \end{tikzpicture}
  \caption{Process View of High Level Location Determination}
\label{fig:locationdetprocess}
\end{figure}
% link explaining carrier phase estimation https://www.trimble.com/gps_tutorial/sub_phases.aspx
It is necessary to apply all stated security concepts for location service networking, sensor fusion algorithms, and operating system software modules and dependencies. 



% interoperability \cite{eu2018road}, \ac{gdpr} \cite{sfakianakis2019enisa}, dynamic and automated risk assessment \cite{rao2017probabilistic}, attack prediction and attribution \cite{patel2013classification}, threat predictive analytics, monitoring, and detection intelligence \cite{nec18itaru}, encrypted traffic analysis \cite{cheng2018encrypted} \cite{anderson2017machine}, forensic readiness \cite{valjarevic2013harmonized}, intrusion detection \cite{haas2017intrusion} \cite{alheeti2016hybrid}, intrusion prevention \cite{anwar2017intrusion} \cite{anuar2009response}, penetration testing \cite{scarfone2008technical}, and honeypots \cite{wahlisch2013design}.

% requires module verification, unit and system testing, monitoring, logging, etc. to cover the stated software vulnerabilities which apply to sensor fusion, networking, and operating system software.

% \todo{prevention, detection, and reaction per view model context}



% BS = 10*1*0.8*0.6*(1*0.25+1*0.25+1*0.5) = 4
% TMP = BS*0.85*0.87*0.9 = 4*0.85*0.87*0.9 = 2.6
% ENV = (TMP + (10-TMP)*0.5)*0.25 = 1.5

% BaseScore = round to 1 digit of 10
% * (case AccessVector of local: 0.7 remote: 1.0)
% * (case AccessComplexity of high: 0.8 low: 1.0)
% * (case Authentication of required: 0.6 not-required: 1.0)
% * ((case ConfidentialityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.5 INTGRTY:
% 0.25 AVLBLTY: 0.25)
% + (case IntegrityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.5 AVLBLTY : 0.25)
% + (case AvailabilityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.25 AVLBLTY : 0.5))


% TemporalScore = round to 1 digit of BaseScore
%  * (case Exploitability of unproven: 0.85 proof-of-concept: 0.9
% functional: 0.95 high: 1.00)
%  * (case RemediationLevel of official-fix: 0.87 temporary-fix: 0.90
% workaround: 0.95 unavail: 1.00)
%  * (case ReportConfidence of unconfirmed: 0.90 uncorroborated: 0.95 confirmed:
% 1.00)

% EnvironmentalScore = round to 1 digit of (TemporalScore + (10 -
% TemporalScore)
% * (case CollateralDamagePotential of none: 0 low: 0.1 medium: 0.3 high:
% 0.5))
% * (case TargetDistribution of none: 0 low: 0.25 medium: 0.75 high:
% 1.00)

% explain adaptive autosar in 2 sentence, with communication middleware that is used to communicate among different devices

% explain autosar classic layered architecture and runtime environment that binds all modules together... access to this component is most desirable

% where is data stored, and where do adaptive autosar application store keys and where to enter software interfaces

% HEAT project Hamburg and Stimulate Berlin autonomous buses circular courses with 26 stops max speed of 20km/h on board vehicle operator
% \cite{kolb2020technische}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PROCESS VIEW


\subsection{Process View Analysis}

\subsubsection{System Modeling}


The process view indicates the interplay of logical components for location determination in a sequential order.  Figure \ref{fig:locationdetprocess} represents the order which starts with \ac{agps} utilization for faster satellite localization. Reception of \ac{gps} data from satellites and subsequent merging of \ac{dgps} correction data determines the initial position estimation of the vehicle. 
At the same time, \ac{imu} data of vehicle movement passes the Kalman filter to feed the estimation between vision-based tracking scans. 
When it comes to the matching of scan and map data, the initial \ac{gps} position narrows the area of map matching  which further optimizes and stabilizes the position estimation \cite{qingqing2019multi}. 
The last part of the process view is the transmission of vehicle location data to the cloud services for vehicle tracking. Services of \ac{adas} modules such as maneuver estimation services \cite{alhajyaseen2012estimation} and lane hypothesis estimation benefit from the \ac{slam} map matching as well \cite{rabe2019lane}.

\subsubsection{Threat \& Vulnerability Analysis}
All communication protocols of the mentioned services outside of the vehicle make up a direct attack surface for the attacker. 
Even though communication protocols differ, common attacks such as jamming, spoofing, timing, capturing, modification, removal, payload, etc. apply to all communication protocols independent of the software \ac{osi} reference layers \cite{cui2019review}. 
The collection of \cite{igure2008taxonomies} provides several network vulnerability taxonomies which vary the following way. 
The \ac{ncva} taxonomy of \cite{marlin1988methodology} classifies networks on transfer strategy, control method, link structure, link access method or protocol, and system topology.
This high level assessment identifies susceptibilities and overlaps with the system design vulnerability assessment of the logical view due to the fact that topology design is driven by system design.
The taxonomies of \cite{jayaram1997network} and \cite{welch2003wireless} highlight threats over the actual vulnerabilities in form of assets. 
To name threats that complement the initially introduces threats on communication protocols, malign problems, traffic analysis, passive eavesdropping, active eavesdropping, session highjacking and replay attacks belong to the taxonomies.
The last network vulnerability taxonomy overlaps with the developer view threats but focuses on communication software.
Explicitly, the work of \cite{pothamsetty2004vulnerability} lists clear text communication, message parsing, state handling, packet rates, reuse, field authentication, entropy problems
as vulnerabilities of communication protocols.


\subsubsection{Risk Analysis \& Security Requirements}

The risk analysis with the identified assets, threats and vulnerabilities of the networking category allows us to determine the \ac{cvss} score of $15$. 
Table \ref{tab:cvssscores} illustrates our selection of labels. 
Due to the exposure of communication messages and interfaces, we emphasize on the reaction patterns of security requirements for the networking domain.
The large scale communication attack mitigation analysis of \cite{kholidy2016risk} identifies sixteen reactive defence mechanism and provides pros and cons of each mitigation strategy. 
To provide an initial taste, packet dropping, replica, isolation, disconnection, termination, restart, redirection, inspection, filtering, etc. belong to this collection of concepts. 
The defence mechanisms thereby counteract the malicious communicator and sensor disrupter attacker types of the \ac{iov} specific attacker model of \cite{monteuuis2018attacker}.



\subsubsection{Security Considerations}

Security considerations for the networking domain affect safe and reliable connectivity of \ac{v2i} and \ac{p2i}.
Since \ac{mitm} and other networking attacks are difficult to prevent, the focus in this domain lies on detection and especially reaction concepts \cite{khader2015preventing}.
Another reason for this fact is the necessary exposure of networking interfaces which enable the localization services in the first place. 
Hence, safe routing, redirect adaptivity, redundant connectivity, etc. point out the direction of tailored communication security for the location services of \ac{cav}s.



% \todo{prevention, detection, and reaction per view model context}


% BS = 10*1*1*0.6*(0.7*0.25+1*0.5+0.7*0.25) = 5.1
% TMP = BS*0.95*0.9*0.95* = 4.1
% ENV = (TMP+(10-TMP)*0.3)*1 = 5.87


% BaseScore = round to 1 digit of 10
% * (case AccessVector of local: 0.7 remote: 1.0)
% * (case AccessComplexity of high: 0.8 low: 1.0)
% * (case Authentication of required: 0.6 not-required: 1.0)
% * ((case ConfidentialityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.5 INTGRTY:
% 0.25 AVLBLTY: 0.25)
% + (case IntegrityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.5 AVLBLTY : 0.25)
% + (case AvailabilityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.25 AVLBLTY : 0.5))


% TemporalScore = round to 1 digit of BaseScore
%  * (case Exploitability of unproven: 0.85 proof-of-concept: 0.9
% functional: 0.95 high: 1.00)
%  * (case RemediationLevel of official-fix: 0.87 temporary-fix: 0.90
% workaround: 0.95 unavail: 1.00)
%  * (case ReportConfidence of unconfirmed: 0.90 uncorroborated: 0.95 confirmed:
% 1.00)

% EnvironmentalScore = round to 1 digit of (TemporalScore + (10 -
% TemporalScore)
% * (case CollateralDamagePotential of none: 0 low: 0.1 medium: 0.3 high:
% 0.5))
% * (case TargetDistribution of none: 0 low: 0.25 medium: 0.75 high:
% 1.00)



\subsection{Physical View Analysis}



\subsubsection{System Modeling}

Due to the large infrastructure of the \ac{iov} autonomous shuttle scenario, the physical view remains at a rather high level and outlines physical connections of infrastructure components.
Figure \ref{fig:physicallocation} shows the physical view of the vehicle, \ac{dgps}, and cloud components and their connections. Even though the cloud has no icon in the figure, it is connected over the cellular base station. 
We neglect to show the physical view of the infrastructure for creating \ac{slam} maps due to the fact, that \ac{slam} data as well as trajectory calculations happen before autonomous vehicle deployment \cite{li2016road}. 
Nevertheless, securing the process of creating unbiased and high quality \ac{slam} trajectories of deployment environments is important and remains as another security research focus. 


% section explain process of localization service of physical view
The simplest form of a \ac{gps} infrastructure consists three segments called control, space, and user segment \cite{navstar1996user}. 
The control segment of stationary \ac{gps} base stations with fixed locations monitor as well as update satellite navigation data messages.
The arrangement of twenty four satellites in six orbital planes define the space segment and broadcast position, velocity, and time information. 
Receivers of the user segment calculate the position and time of each satellite based on transmission times of \ac{gps} signals which allow range determination of satellites. 
The minimum of four satellite positions enables receivers to determine their own position. 



% second in vehicle logical view here....
%\todo{rework}
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.9]

    % \draw [<->] (0,0) -- ++ (1,1);

    % \node (rmat) at (0,1) [transform shape = true] {Remote Attacker};
    % \node (hardw1) at (1,2) [transform shape = true, anchor=west] {Hardware};
    
    \node (g1) at (0,4) [rectangle, thick, draw=black, fill=white!80!gray, minimum width=1cm, minimum height=0.75cm, transform shape = true, align=left] {Gateway};
    
    \node (dc1) at (0.1,3) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=west, align=left] {Domain \\Controller};
    \node (dc2) at (-0.1,3) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=east, align=left] {Domain \\Controller};
    
    \node (points) at (-3,3) [transform shape = true, anchor=west] {.....};
    \node (points) at (4.2,3) [transform shape = true, anchor=west] {.....};
    % \node (dc3) at (-2,3) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=east, align=left] {Domain \\Controller};
    \node (dc4) at (3.7,3) [rectangle, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=east, align=left] {Domain \\Controller};
    
    \node (ec1) at (1.5,2) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=west] {Sensing \& Diagnostics};
    \node (ec2) at (1.5,1) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=west, align=left] {Adaptive Cruise \\Control Module};
    % \node (ec3) at (-2.35,2) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=east] {ECU};
    \node (ec4) at (-1.6,1) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=east, align=left] {Telematics \\Module};
    
    % \node (sa1) at (2.8,2) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=west] {Sensor};
    %\node (sa2) at (3,0) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=west] {Actuator};
    %\node (sa3) at (-3.25,2) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=east, align=left] {Optional \\Sensor};
    %\node (sa4) at (-2,-0.25) [rectangle, thick, draw=black, fill=white!90!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, anchor=west, align=left] {Sub-bus \\Component};
    
    \draw [-, thick] (g1.west) -- ++(-0.2,0) -- (dc2.north);
    % \draw [-, thick] (g1.west) -- ++(-2.1,0) -- (dc3.north);
    \draw [-, thick] (g1.east) -- ++(0.2,0) -- (dc1.north);
    \draw [-, thick] (g1.east) -- ++(2.1,0) -- (dc4.north);
    
    %\draw [-] (ec3.west) -- (sa3.east);
    %\draw [-] (ec4.south) -- ++(0,-.785) -- (sa4.west);
    
    % \draw [-, thick] (dc1.south) -- ++(0,-0.535) -- (ec1.west);
    \draw [-, thick] (dc1.south) -- ++(0,-1.535) -- (ec2.west);
    \draw [-, thick] (dc4.south) -- ++(0,-0.25);
    % \draw [-, thick] (dc3.south) -- (ec3.north);
    \draw [-, thick] (dc2.south) -- ++(0,-1.535) -- (ec4.east);
    
    % \draw [-] (ec1.east) -- (sa1.west);
    %\draw [-] (ec2.south) -- ++(0,-0.535) -- (sa2.west);

    \end{tikzpicture}
  \caption{Physical View of Simplified In-Vehicle E/E-Architecture}
\label{fig:physicalautomotivearch}
\end{figure}
Next to vehicle communication links for location determination, on-board vehicle sensors as well as the \ac{eea} constitute the next resources for localization data collection and processing. 
Figure \ref{fig:physicalautomotivearch} presents a simplified physical view of the in-vehicle architecture. 
There exist different architecture designs such as zone, domain, or central gateway based architectures \cite{brunner2017automotive}. 
The reference architecture shown in Figure \ref{fig:physicalautomotivearch} follows the domain based architectural design. 
The reason for it is that the modern automotive Ethernet anatomy has computational powerful domain controllers which group \ac{adas}, drive-train, infotainment, \ac{hmi}, etc network segments \cite{sharma2019extended}. % ethernet2014overview
The design enables isolation, criticality and bandwidth respecting separations and unloads the gateway component \cite{shreejith2017vega}. 
\ac{lidar}, camera, odometry (\ac{imu} and wheel encoder), and \ac{gnss} \ac{rtk} sensors, actuators, and antennas gather location relevant visual, odometry/motion, and communication data and send receptions to \ac{ecu}s \cite{brunner2017automotive}. 
The automotive \ac{eea} attaches sensors and actuators to \ac{ecu}s which in turn connect to domain controllers or directly connect to the central gateway component depending on safety critical functionality \cite{shreejith2017vega}. 
With the transmission of location data to the cloud, the gateway enables cloud services to publish vehicle information to smartphone applications \cite{lee2014design}.


\subsubsection{Threat \& Vulnerability Analysis}

It is unlikely for an attacker to gain access to physical infrastructure units in the cloud, networking, or satellite domain. 
For this reason, we focus on the vehicle architecture threats and vulnerabilities in the physical domain.
The general attack taxonomy of physical attack on \ac{iot} devices of \cite{abdul2018comprehensive} counts twelve hardware threat types.
They moreover map threats and attacks to affected security requirements and countermeasures. 
Object tampering, outage, object replication, camouflage, side-channel, hardware trojans, physical damage etc. attacks are among the threats of this work.
Highlighting in-vehicle architecture attacks specifically, the work of \cite{sharma2019extended} provides a detailed attack surface.
Here, non-\ac{can} attacks, in form of \ac{tpms} and KeeLoq Cipher, and \ac{can} attacks, in form of media player, \ac{obd}, bluetooth module, and \ac{tcm} attacks, exploit attack surface spots of the listed devices.
The vulnerability assessment of \cite{salfer2015attack} further identifies boot memory, debug interfaces, inter-chip communication channels, and side-channel attacks among others as susceptible hardware units.


% Attack Surface and Vulnerability Assessment of Automotive Electronic Control Units -- GREAT !!!
% Connected Vehicles

\subsubsection{Risk Analysis \& Security Requirements}

Again, with the attacks surface and the threat modeling and vulnerability analysis, it is possible to calculate the \ac{cvss} score in Table \ref{tab:cvssscores}.
The vulnerability score of physical \ac{iov} infrastructure components reaches a total value of $7$.
Regarding security requirements and complementing the classical taxonomies, \cite{sharma2019extended} intrusion detection next to the classic authentication requirement as the most important defence mechanisms.
To cover hardware vulnerabilities such as for instance memory, \cite{salfer2015attack} and \cite{oyler2016security} emphasize on stack canaries, no execute bit, address space layout randomization, protection units, management units, privilege separation, and \ac{hsm} mitigation concepts. 



\subsubsection{Security Considerations}

In the opposite way to networking components, access to physical components remains a challenging task due to location and speed dynamics of vehicles and the distance to cloud or infrastructure assets. 
Thus, tailored security for physical components of the \ac{iov} location service focuses on insider attacks \cite{dietzel2015context}.
This means physical attack surfaces such as \ac{obd} assets require misbehavior detection frameworks and secure aggregation mechanisms.

% \todo{prevention, detection, and reaction per view model context}


% stride for in vehicle devices
% https://onlinelibrary.wiley.com/doi/epdf/10.1002/sec.1610


% \cite{abdul2018comprehensive} covers the rows of physical protection, freshness, secure information flow, and attack detection. 


% BS = 10*1*0.8*0.6*(0.7*0.333+0.7*0.333+0.7*0.333) = 3.5
% TMP = BS*0.9*0.87*0.9 = 2.4
% ENV = (tmp + (10-tmp)*0.3)*0.25 = 1.1


% BaseScore = round to 1 digit of 10
% * (case AccessVector of local: 0.7 remote: 1.0)
% * (case AccessComplexity of high: 0.8 low: 1.0)
% * (case Authentication of required: 0.6 not-required: 1.0)
% * ((case ConfidentialityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.5 INTGRTY:
% 0.25 AVLBLTY: 0.25)
% + (case IntegrityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.5 AVLBLTY : 0.25)
% + (case AvailabilityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.25 AVLBLTY : 0.5))


% TemporalScore = round to 1 digit of BaseScore
%  * (case Exploitability of unproven: 0.85 proof-of-concept: 0.9
% functional: 0.95 high: 1.00)
%  * (case RemediationLevel of official-fix: 0.87 temporary-fix: 0.90
% workaround: 0.95 unavail: 1.00)
%  * (case ReportConfidence of unconfirmed: 0.90 uncorroborated: 0.95 confirmed:
% 1.00)

% EnvironmentalScore = round to 1 digit of (TemporalScore + (10 -
% TemporalScore)
% * (case CollateralDamagePotential of none: 0 low: 0.1 medium: 0.3 high:
% 0.5))
% * (case TargetDistribution of none: 0 low: 0.25 medium: 0.75 high:
% 1.00)





\subsection{Analysis Digest}
\label{analysisdigest}

To prevent addressing of similar vulnerability metrics in different domains, this section walks through each vulnerability metric of the \ac{cvss} score and applies it in respect of multiple view model layers.
The formulas \ref{cvssf1}, \ref{cvssf2}, and \ref{cvssf3} calculate the \ac{cvss} base, temporal, and environmental score respectively and can be found in \cite{schiffman2004common}.
Additionally, this work explains all definitions of the scoring parameters.
The parameters within each of the formula originate of the \emph{Short} column on Table \ref{tab:labelsandscores}.
Every parameter of Table \ref{tab:labelsandscores} requires a label which determines its value except the \emph{CIB}, \emph{IIB}, \emph{AIB} scores which depend on the setting of the \emph{Impact Bias}.
The following paragraphs explain our choice of labeling which Table \ref{tab:cvssscores} summarizes.
\begin{equation}
\label{cvssf1}
\resizebox{.91\hsize}{!}{$
Base Score = 10*AV*AC*A*((CI*CIB)+(II*IIB)+(AI*AIB))
$}
\end{equation}
\begin{equation}
\label{cvssf2}
\resizebox{.6\hsize}{!}{$
Temporal Score = Base Score*E*RL*RC
$}
\end{equation}
\begin{equation}
\label{cvssf3}
\resizebox{.91\hsize}{!}{$
Environmental Score = (Temporal Score+(10-Temporal Score)*CDP)*TD
$}
\end{equation}
The connectivity of the \ac{iov} architecture components enables the label remote for the access vector in every category. % to remote (R).
The access complexity has a similar distribution where every category except networking fulfills the label high. 
Reasons for this choice is the safety critical application of \ac{cav} which requires highest access control standards at every stage.
% Furthermore, the strong interest of the industry does not pose monetary limits on paying security experts for high quality security solutions.
Networking access complexity remains low in the location service scenario due to the fact, that attackers face direct access to networking applications of redundant location services.
\begin{table}[htbp] % [!t]
\renewcommand{\arraystretch}{1.3}
\caption{Default \ac{cvss} Labels and Scores}
\label{tab:labelsandscores}
\centering
\begin{tabular}{|p{2.25cm}|p{0.6cm}|p{4.75cm}|}
\hline
\textbf{Parameters} & \textbf{Short} & \textbf{Possible Labels and Score} \\ 
\hline
\hline
Access Vector  & AV  & Local (L) 0.7; Remote (R) 1.0 \\ 
\hline
Access Complexity & AC & High (H) 0.8; Low (L) 1.0  \\ % camera networking/communication or apis need medium/Low access complexity in oder for user phones to connect and fetch service 
\hline
Authentication & A  & Required (R) 0.6; Not-Required (N) 1.0 \\ 
\hline
Confidentiality Impact & CI & None (N) 0; Partial (P) 0.7; Complete (C) 1.0  \\
\hline
Confidentiality Impact Bias & CIB & case IB==N 0.333; case IB==C 0.5; case IB==I 0.25; case IB==A 0.25  \\
\hline
Integrity Impact & II & None (N) 0; Partial (P) 0.7; Complete (C) 1.0 \\ 
\hline
Integrity Impact Bias & IIB & case IB==N 0.333; case IB==C 0.25; case IB==I 0.5; case IB==A 0.25  \\ 
\hline
Availability Impact & AI & None (N) 0; Partial (P) 0.7; Complete (C) 1.0 \\ 
\hline
Availability Impact Bias & AIB & case IB==N 0.333; case IB==C 0.25; case IB==I 0.25; case IB==A 0.5  \\ 
\hline
Impact Bias & IB & Normal (N); Confidentiality (C); Integrity (I); Availability (A)  \\ 
\hline
\hline
Exploitability & E & Unproven (U) 0.85; Proof of Concept (PoC) 0.9; Functional (F) 0.95; High (H) 1.0 \\ % this needs references 
\hline
Remediation Level & RL & Official fix (OF) 0.87; Temporal fix (TF) 0.9; Walkaround (W) 0.95; Unavailable (U) 1.0 \\ 
\hline
Report Confidence & RC & Unconfirmed (UCF) 0.9; Uncorroborated (UCB) 0.95; Confirmed (C) 1.0 \\ 
\hline
\hline
Collateral Damage Potential & CDP & None (N) 0; Low (L) 0.1; Medium (M) 0.3; High (H) 0.5 \\ 
\hline
Target Distribution & TD & None (N) 0; Low (L) 0.25; Medium (M) 0.75; High (H) 1.0 \\ 
\hline
\end{tabular}
\end{table}
% Regarding authentication, software provides data access and authentication privileges per default. 
% To access the \ac{iov} cloud and vehicle environment requires (R) authentication but infrastructure services such as \ac{gps} data reception does not need authentication.
Every category requires authentication concepts except the data domain. 
Regular \ac{gps} receivers do not necessarily authenticate satellites. 
But software behind signal reception interfaces authenticates correct signals.
%
% where it is possible for any device to receive \ac{gps} data. % question, doesnt it require device authentication only? or does gps really authenticate data? it just uses correlation which implcitly detects wrong signals...
Compromising software has the potential to cause complete confidentiality, integrity, and availability loss in the whole system.
Equally, successful data and networking integrity manipulation could allow data or network participants to propagate through the system if not correctly detected in initial checks. 
Otherwise, impact on the \ac{cia} requirements remains partial.
For the impact bias and with regard to the location service scenario, data and networking components obviously weight integrity over other requirements as incorrect location data or communication entities potentially destroy the service.
Since there is a centralized sensor fusion software module, the impact bias of software applies greater weighting to availability.
With respect to the hardware category, exploiting any of the listed security requirements leads to comparable normal impact of the attack on the system. 

% We consider the impact on integrity and availability as partial due to redundant location data sources.
% Confidentiality exploitation impacts the data of the scenario only in the case of video data which contains privacy relevant data. 
% Integrity must be ensured in for location service data at any time which sets the impact bias to integrity (I).

Regarding data attacks, existing research on \ac{gps} spoofing provide a \ac{poc} to manipulate location data \cite{larcom2013modeling}. 
This fact can be used to assume the existence of additional uncorroborated sources.
At the same time temporal fix solutions exist for detection and prevention of such attacks. 
The networking category behaves similar except that it is possible to access functional networking exploit code by using hacking operating systems.
With software, we assume non-disclosed solutions of sensor fusion and localization algorithms of vehicle manufacturers.
This fact sets the exploitability of location service \ac{ecu} software to unproven.
Due to the criticality of location service correctness, one must expect official fixes of newly confirmed vulnerabilities.


\begin{table}[htbp] % [!t]
\renewcommand{\arraystretch}{1.3}
\caption{\ac{cvss} Scores per View Model Layer}
\label{tab:cvssscores}
\centering
\begin{tabular}{|p{2.25cm}|p{0.75cm}|p{1cm}|p{1.5cm}|p{1.25cm}|}
\hline
\textbf{Parameters} & \textbf{Data} & \textbf{Software} & \textbf{Networking} & \textbf{Hardware} \\ 
\hline
\hline
Access Vector  & R  & R  & R  & R \\ 
\hline
Access Complexity & H  & H  & L & H \\ % camera networking/communication or apis need medium/Low access complexity in oder for user phones to connect and fetch service 
\hline
Authentication & N  & R  & R  &  R \\ 
\hline
Confidentiality Impact & P  & C & P & P \\  % in the software module, exploit reveals total confidentiality
\hline
Integrity Impact & C & C & C & P \\ 
\hline
Availability Impact & P & C & P & P \\ 
\hline
Impact Bias & I & A & I & N \\ 
\hline
\textbf{Base Score} & \textbf{8.5}  & \textbf{4}  & \textbf{5.1}  & \textbf{3.5} \\ 
\hline
Exploitability & PoC & U & F & PoC \\ % this needs references 
\hline
Remediation Level & TF & OF & TF & OF \\  % hardware and software vendors need to publish updates, dod and data manipulation at input cannot be prevented, software Dos needs vendor solution
\hline
Report Confidence & UCB & UCF & UCB & UCF \\ 
\hline
\textbf{Temporal Score} & \textbf{6.5}  & \textbf{2.6}  & \textbf{4.1}  & \textbf{2.4} \\ 
\hline
Collateral Damage Potential & H & H & M & M \\ 
\hline
Target Distribution & M & L & H & L \\ 
\hline
\textbf{Environmental Score} & \textbf{6.1} &  \textbf{1.5} & \textbf{5.8}  & \textbf{1.1} \\ 
\hline
\textbf{Total} & \textbf{21.1} &  \textbf{8.1} & \textbf{15}  & \textbf{7} \\ 
\hline
\end{tabular}
\end{table}
The collateral damage potential of data and software is high as it directly affects safety of the vehicle system.
Redundancy and robustness of location services enables temporal autonomy of a vehicle and reduces the damage potential of networking and hardware attacks to medium \cite{miucic2018connected}.
Regarding target distribution, the multi sensor fusion software as well as the physically reachable hardware deserve a low distribution value. 
Communication and location data propagate from infrastructure nodes through the vehicle to the cloud and require a high distribution value. 
However, compromised location data of cloud services do not affect the location service functionality of the vehicle itself anymore. 
Only the redistribution of malicious vehicle location data from cloud services to other vehicles causes problems. For this reason we evaluate the distribution of highly critical location data as medium. 


The \ac{cvss} scoring of this work groups abstract categories which provides quantitative risk assessment measures.
As a consequence, the resulting security verification, applied in section \ref{section6}, of this work remains quantitative as well.
It is moreover necessary to state that the \ac{cvss} scoring is an old risk assessment system which is not tailored to \ac{iov} specific vulnerabilities. 
The application of \ac{iov} specific risk assessment scoring methodologies remains future work.
For this work, the simple and straight forward \ac{cvss} scoring system demonstrates an initial risk assessment.
But it would be possible to further set up vulnerability scores for each of the reference model domains. 
This would improve the overall risk assessment per view model domain. 
Nevertheless, the introduction of more detailed parameters of the vulnerability scoring model requires adaptation and normalization regarding the remaining values.

% \todo{need a comment here on the values?}

% \todo{better writing, the disclaimer}
% Disclaimer, this scoring groups all software components but there exist multiple software modules in each reference model sub-architecture. this needs more detailed analysis and more fine grained attack paths for explicit attacks.
% but it is a first general evaluation that suffices for a quantitative security verification.

% Even though the state of practice of defence mechanisms covers a very wide range of attacks, shortcomings remain. % \cite{parkinson2017cyber}. 
% It is therefore important to pay special attention to the following categories of security gaps of the works \cite{sun2017attacks},  \cite{barnard2014threat}, and \cite{parkinson2017cyber}.
% \begin{itemize}
%     \item Reduction of effects of existing systems
%     \item External effects
%     \item Long term studies of fast evolving security techniques
%     \item Knowledge Gaps and their potential impact
%     \item Human error and criminology
%     \item Impact of law, policy, and liability
% \end{itemize}

% difficult attack prediction and attribution \cite{patel2013classification}, requires detection, risk analysis and simulation to attribute attacks 







% TOTAL BS = 10*1*1*1*(1*0.5+1*0.5+1*0.5) = 15
% TOTAL TEMP = BS * 1*1*1 = 15
% TOTAL ENV = (TMP+(10-TMP)*0.5)*1 = 12,5

% TOTAL = 42.5


% BaseScore = round to 1 digit of 10
% * (case AccessVector of local: 0.7 remote: 1.0)
% * (case AccessComplexity of high: 0.8 low: 1.0)
% * (case Authentication of required: 0.6 not-required: 1.0)
% * ((case ConfidentialityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.5 INTGRTY:
% 0.25 AVLBLTY: 0.25)
% + (case IntegrityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.5 AVLBLTY : 0.25)
% + (case AvailabilityImpact of none: 0 partial: 0.7
% complete: 1.0)
% * (case ImpactBias of normal: 0.333 CNFDNTLTY: 0.25 INTGRTY
% : 0.25 AVLBLTY : 0.5))


% TemporalScore = round to 1 digit of BaseScore
%  * (case Exploitability of unproven: 0.85 proof-of-concept: 0.9
% functional: 0.95 high: 1.00)
%  * (case RemediationLevel of official-fix: 0.87 temporary-fix: 0.90
% workaround: 0.95 unavail: 1.00)
%  * (case ReportConfidence of unconfirmed: 0.90 uncorroborated: 0.95 confirmed:
% 1.00)

% EnvironmentalScore = round to 1 digit of (TemporalScore + (10 -
% TemporalScore)
% * (case CollateralDamagePotential of none: 0 low: 0.1 medium: 0.3 high:
% 0.5))
% * (case TargetDistribution of none: 0 low: 0.25 medium: 0.75 high:
% 1.00)



% \subsection{Attack Surface Investigation and Evaluation based on Security Requirements}

% table structure explanation
% The application of the attack surface categorization of section \ref{attacksurfacecategorization} allocates the reference model sub-architectures to the attack surface types of hardware, communication, and software. 
% Subsequently, it is possible to map assets, that have been identified by the physical view, to the four reference sub-architectures of the type of hardware attack surface.
% Similarly, assets identified by the logical view map to the reference models grouped under the type of communication attack surface.
% And last but not least, assets identified by the developer view map to the reference models that belong to the type of software attack surface.
% The three left most columns of Table \ref{tab:attacksurfevaluation} show these mappings.
% The reason for considering the peripherals and vehicle models as one single category for the asset mapping is to reduce the reference architecture to the most essential characteristics. A wide range of viewpoints and differentiating between similar sub-architectures hampers the security analysis \cite{karkhanis2018defining}. 


% %%
% Before the application of security requirements on identified assets, there are two things to reconsider.
% First, attackers need to compromise the surface type of either hardware or communication to attack the software type of attack surface.
% Second, the process view indicates the attack surface of the localization service for attacks which successfully breach first level defence mechanisms.
% To protect the predefined scenarios for localization determination, Table \ref{tab:attacksurfevaluation} shows the selection of security requirements that apply to hardware, software, and communication assets of different categories of the reference model.
% The security requirement of conformance is not listed in the requirements column due to the fact that it applies to all assets.


% % this is in the wrong place here, but leaving it for now, this last paragraph of this section should explain why certain requirements are mapped to assets and why some others are left away
% % the paragraph written here might go into the defence mechanism chapter
% In order to design and evaluate mitigation strategies for the identified assets, the security requirements reveal design choices of risk treatment strategies with regard to reduction, transfer, avoidance, and acceptance of possible risks. 
% This way, potential threats can be identified, mitigated, and addressed during the software development life cycle of the multi-layer security framework \cite{zahid2019security}. 
% Simultaneously, risk mitigation contributes to the defence model design and helps to complete the threat modeling procedure of respective risk identification and assessment through asset and attack analysis \cite{pacheco2016iot}.
% Another point is the design of the trade-off of different requirements per asset. 
% Assets with many security requirements face higher attack susceptibility due to an increase of validation, configuration, and implementation requirements. 
% Next to threat vector accessibility and attacker capability, system susceptibility represents the third ingredient for a vulnerability to exist \cite{hughes2013quantitative}. 


% The \ac{iov} characteristics that affect autonomous vehicles require high precision and real-time location services with continuous connectivity.
% As a consequence, vehicle location services depend on advanced \ac{gps} services such as \ac{agps}, \ac{dgps}, off-centered \ac{gps} \cite{choi2019leveraging}. 
% With \ac{agps}, receivers have the possibility to leverage location data of \ac{ssid}s or download almanac collection data (information of satellite constellation) which drastically reduces the receiver \ac{ttff} \cite{rubino2009gps}.
% Here, vehicle \ac{gsm} modules and cellular network infrastructure establish the connectivity to the Internet \cite{lee2014design}.

% The underlying assumption of \ac{dgps} is that \ac{gps} receivers of closer proximity experience similar location determination errors. 
% In designated locations, stationary \ac{dgps} base stations are capable of calculating correction data. Transmitted to the user segment receiver, correction data enhances precision of pseudo-range measurements of user segment receivers \cite{pepe2018cors}.
% Figure \ref{fig:logviewlocation} provides details of pseudo-range measurement determinations of user segment receivers.


%% picture here as second phyysical view


% The physical view of vehicle sensors for obstacle detection and localization consists of \ac{lidar}, camera, odometry (\ac{imu} and wheel encoder), and \ac{gnss} \ac{rtk} sensors \cite{}. % reference navya arma 
% The automotive \ac{eea} attaches sensors and actuators to \ac{ecu}s \cite{brunner2017automotive}. \ac{ecu}s connect to the the central gateway component which in turn has the capability to connect to cellular base stations and with that to the cloud. Figure \ref{fig:physicalautomotivearch} illustrates the vehicle physical view.

% The logical view shows base stations which know their location and determine the location of satelites which travel around the globe. Satelites keep the information of the base station calculation in a data table called ephemeris which they send down to fixed position DGPS stations that in turn communicate with vehicles. Next satelites have another data table called almanach which contains information about other satelite locations. 

% satelite data pakets: Apart from these data fields, satelite messages have the following fileds: TLM telemetry incl präambel, HOW handover words incl time of week, clock correction/Uhrenkorrektur then TLM+HOW then Bahndaten/orbit trace data, TLM+HOW, Bahndaten TLM+HOW, Almanach refraktionsmodel, TLM+HOW, almanach

% satelite data transmission: C/A codes, correlation measurements for time correction, signal BPSK, goals to reduce: 1.geometric range, 2.receiver bias clock, 3. satelite clock bias, 4. ionosphere (most critical), 5.troposphere, 6. multipath+receiver noise+other errors, - disturbing all these data properties is attack goal
% -- all these points can be corrected by using :1. bahndaten, 2. berechnungstrick, 3. correction, 4. correction+calculation model 5. antenna+filter 6. estimation+kalman filter

% improving gps:
% SBAS satelite based augmentation system(WAAS,EGNOS,MSAS): 
%     - Ionosphärenmessung mit bodenstation
%     - senden von korrekturdaten mit erhöhter datenrate

% A-GPS (over GSM/cellular network):
%     - almanach data over 2nd channel with higher data rate (internet)
%     - receiver clock correction
%     - grob lokalisierung with other sources(WLAN SSIDs)

% more accurate:
% - P(Y) code: longer code 720 Gbit long (1 week), 10 Mbit/s, better correlation+better resolution (military use and encrypted)
% - L2 channel: 1227 MHz frequency, only P(Y) code, frequency dependency allows correction of ionosphere time distortion by receiving both signals
% - L2C channel: testing since 2015,  longer CM/CL codes on L2 frequency

% --> differential GPS:
% - base station with known fixed location for second receiver
% - creates correction data for second receiver (itself is first) -- sending correction data to vehicle
% - higher relative accuracy cause ionosphere distortion eliminated
% --> carrier phase:
% - delay correction directly with carrier frequency instead of C/A code 
% - 1500 times more accurate
% - integer ambiguity every 18 periods , this requires to count every schwimung, cannot have schlechter epfang sonst weis man nicht wieviele schwinungen dazukommen  (short replication of code, every 18 cm there ist gültige lösung for positionsberechnung, kann auch normale C/A code correlation, dann umshalten auf carrier phase combination)

% %%% NAVYA technology:
% A GPS antenna is a device designed to receive and amplify the radio signals transmitted on specific frequencies by GPS satellites and convert then to an electronic signal for use by a GPS receiver. The output of the GPS antenna is fed into a GPS receiver which can compute the position.

% What’s the difference between GPS and GNSS?
% GPS is the USA’s global positioning system and GNSS stands for Global
% Navigation Satellite System. GNSS covers all the difference systems in
% use worldwide, such as GPS, GLONASS, Galileo, Beidou etc.
% A GNSS antenna needs a slightly wider bandwidth as the GLONASS
% system operates on slightly different frequencies to GPS.
% So while a GPS antenna may pick up GLONASS signals, it isn’t
% recommended.

% Real-time kinematic (RTK) positioning is a satellite navigation technique used to enhance the precision of position data derived from satellite-based positioning systems (global navigation satellite systems, GNSS) such as GPS, GLONASS, Galileo, NavIC and BeiDou. It uses measurements of the phase of the signal's carrier wave in addition to the information content of the signal and relies on a single reference station or interpolated virtual station to provide real-time corrections, providing up to centimetre-level accuracy.[1] With reference to GPS in particular, the system is commonly referred to as carrier-phase enhancement, or CPGPS.[2] It has applications in land survey, hydrographic survey, and in unmanned aerial vehicle navigation.
% [1]  Wanninger, Lambert. "Introduction to Network RTK". www.wasoft.de. IAG Working Group 4.5.1. Retrieved 14 February 2018.
% [2] Mannings, Robin (2008). Ubiquitous Positioning. Artech House. p. 102. ISBN 978-1596931046.

%% ADDITIONAL INFO
% The ephemeris contains Keplerian orbital elements wich allow satelite calculation at a specific point in time. These elements are Epoch Time - the time at which the other seven values are defined, i - Inclination (degrees) - the angle between the equator and the orbit plane, e – Eccentricity - a constant defining the shape of the orbit (0=circular, <1=elliptical), a - Semi-major Axis (meters) - a constant defining the size of the orbit, ν - True Anomaly (degrees) - the angle between perigee and the vehicle (in the orbit plane), Ω - Right Ascension of the Ascending Node (degrees) - the angle between vernal equinox and the point where the orbit crosses the equatorial plane (going north), ω - Argument of Perigee (degrees) - the angle between the ascending node and the orbit's point of closest approach to the earth (perigee)



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% physical sensor surface







% \subsection{Attack Surface Investigation and Evaluation based on Security Requirements}


% % table to summarise attack surface:
% \begin{table*}[t]
% \caption{Attack Surface Evaluation}
% \label{tab:attacksurfevaluation}
%   \centering
%   \begin{tabular}{|p{6em}|p{6em}|p{24em}|p{24em}|}
%     \hline
%     \textbf{Surface Type} & \textbf{Model Type} & \textbf{Asset} & \textbf{Requirement} \\
%     \hline
%     \hline
%     Hardware & Cloud & Gateway, Server, Router, Ethernet & Physical Protection, Access Control  \\
%     \hline
%     Hardware & Infra \& Edge & DGPS and Cellular Base Station, Cables, Traffic Lights & Physical Protection, Access Control  \\
%     \hline
%     Hardware & Vehicle \& \ \ Peripherals & ECU, Gateway, Sensor, Actuator, Ethernet/CAN & Physical Protection, Access Control, Privacy \\
%     \hline

%     Communication & Cloud & Vehicle to Cloud & Integrity, Freshness, Manageability, Usability, Privacy, Attack Detection, Non-repudiation, Access Control  \\
%     \hline
%     Communication & Infra \& Edge & Vehicle to Vehicle/Road Side Units/Smartphone, Satellite to Vehicle/Base Station, Base Station (DGPS, Cellular) to Vehicle & Integrity, Freshness, Manageability, Privacy  \\ % Vehicle is considered a Infrastructure component
%     \hline
%     Communication & Vehicle \& \ \ Peripherals  & ECU to Gateway/ECU/Sensor/Actuator/Key & Integrity, Secure Information Flow, Usability, Privacy  \\
%     \hline

%     Software & Cloud & Web API, Web Protocols, Source \& Destination, Time, Database, Session Management, Queues, Events & Usability, Integrity, Access Control, Manageability, Privacy, Attack Detection  \\
%     \hline
%     Software & Infra \& Edge & Networking Stack & Usability, Integrity \\
%     \hline
%     Software & Vehicle \& \ \ Peripherals & APIs, Services, Queues, Events, Time & Usability, Integrity, Manageability, Privacy, Attack Detection, Non-repudiation, Access Control, Freshness, Secure Information Flow, Fair Exchange \\ % Fair exchange with regard to over the air software updates !!!, this means that receiver is able to prove that exchange was completely supplied, and allows to reclaim something is something did not work out
%     \hline
%   \end{tabular}
% \end{table*}


% % table structure explanation
% The application of the attack surface categorization of section \ref{attacksurfacecategorization} allocates the reference model sub-architectures to the attack surface types of hardware, communication, and software. 
% Subsequently, it is possible to map assets, that have been identified by the physical view, to the four reference sub-architectures of the type of hardware attack surface.
% Similarly, assets identified by the logical view map to the reference models grouped under the type of communication attack surface.
% And last but not least, assets identified by the developer view map to the reference models that belong to the type of software attack surface.
% The three left most columns of Table \ref{tab:attacksurfevaluation} show these mappings.
% The reason for considering the peripherals and vehicle models as one single category for the asset mapping is to reduce the reference architecture to the most essential characteristics. A wide range of viewpoints and differentiating between similar sub-architectures hampers the security analysis \cite{karkhanis2018defining}. 


% %%
% Before the application of security requirements on identified assets, there are two things to reconsider.
% First, attackers need to compromise the surface type of either hardware or communication to attack the software type of attack surface.
% Second, the process view indicates the attack surface of the localization service for attacks which successfully breach first level defence mechanisms.
% To protect the predefined scenarios for localization determination, Table \ref{tab:attacksurfevaluation} shows the selection of security requirements that apply to hardware, software, and communication assets of different categories of the reference model.
% The security requirement of conformance is not listed in the requirements column due to the fact that it applies to all assets.


% % this is in the wrong place here, but leaving it for now, this last paragraph of this section should explain why certain requirements are mapped to assets and why some others are left away
% % the paragraph written here might go into the defence mechanism chapter
% In order to design and evaluate mitigation strategies for the identified assets, the security requirements reveal design choices of risk treatment strategies with regard to reduction, transfer, avoidance, and acceptance of possible risks. 
% This way, potential threats can be identified, mitigated, and addressed during the software development life cycle of the multi-layer security framework \cite{zahid2019security}. 
% Simultaneously, risk mitigation contributes to the defence model design and helps to complete the threat modeling procedure of respective risk identification and assessment through asset and attack analysis \cite{pacheco2016iot}.
% Another point is the design of the trade-off of different requirements per asset. 
% Assets with many security requirements face higher attack susceptibility due to an increase of validation, configuration, and implementation requirements. 
% Next to threat vector accessibility and attacker capability, system susceptibility represents the third ingredient for a vulnerability to exist \cite{hughes2013quantitative}. 



% \todo{
% This sections needs comparison to related work ASAP
% its the definition of risk with regard to the time to compromise
% }


% the reason why we do the security requirement mapping: enhance Time To Compromise + we need to secure all the requirements with our defence framework within the specified regions, thus this evaluation points out where in our defence framework we need strong guarantees towards what assets!! , these requirements justify our defence design and must therefore at the same time increase the Time To Compromise 

%Assuming one defence mechanism per security requirement and equally complex defence mechanisms, assets with more security requirements need more complex defence mechanisms.
%Furthermore, it can be assumed that the attack surface of a defence mechanisms increases with increasing complexity. Thus, a larger attack surface of the defence mechanism has a higher risk to be successfully attacked. 
%Assets with higher risk can be compromised faster. 
%We want to increase the time to compromise in the end, so we need to lower the risk per asset which in turn means to lower attack surface of defence mechanism and thereby lower the need of security requirements per asset.

% this part also needs: 
% \\
% \textbf{Build your risk treatment strategy}

% \textbf{Reduce}: %building controls if the form of code upgrades, confirming a specific design for the application or building a specific configuration during the deployment phase to make sure that application risk is reduced.

% \textbf{Transfer}: %For a specific component in the application the risk can be transferred to an outsourced third party to develop that component and making sure that the third party is doing the right testing for the component; or during the deployment phase, outsourcing a third party to do the deployment and transferring that risk to that third party.

% \textbf{Avoid}: %an example of avoiding the risk is disabling a specific function in the application that is the source for that risk.

% \textbf{Accept}: %if the risk is within acceptable criteria set earlier, in that case, the designer risk owner can accept that risk


% thats the reason we apply security requirements




% The physical view model of the location service scenario exposes four categories 
% Software attack surface can only be reached if first layer is breached
% Interplay between surface types is analysed by process view !! this allows to create attack propagation flows
%Regarding requirements: Conformance not considered as it applies to all components in the safety critical infrastructure of \ac{iov}, missing functionality and conformance increases the critically level of the vehicle
% Justify why peripherals not really considered for now !? --> due to missing importance to location services, not true as sensors and actuators count as peripherals !!





% zooming in on identified assets










==> sections/1.2_methodology1.tex <==

\section{Attack Tree Construction and Security Verification based on 4+1 View Model Analysis}
% \section{Multi-Layer Security Framework based on Threat Modeling Analysis using 4+1 View Model}
% \section{Attack Identification}
\label{section4}


This section constructs attack vectors which model every attack propagation step with one of the abstract categories of the 4+1 analysis. Afterwards, Markov Chains can be used to model the consecutive attacking stages with the help of 4+1 view model domains. The threat modeling and risk assessment parameters per category can be used to determine detailed state transition probabilities and with that quantitative system security verification based on \ac{ttc} metrics.




% \subsection{Attack Surface Investigation and Evaluation based on Security Requirements}


% table to summarise attack surface:
% \begin{table*}[t]
% \caption{Attack Surface Evaluation}
% \label{tab:attacksurfevaluation}
%   \centering
%   \begin{tabular}{|p{6em}|p{6em}|p{24em}|p{24em}|}
%     \hline
%     \textbf{Surface Type} & \textbf{Model Type} & \textbf{Asset} & \textbf{Requirement} \\
%     \hline
%     \hline
%     Hardware & Cloud & Gateway, Server, Router, Ethernet & Physical Protection, Access Control  \\
%     \hline
%     Hardware & Infra \& Edge & DGPS and Cellular Base Station, Cables, Traffic Lights & Physical Protection, Access Control  \\
%     \hline
%     Hardware & Vehicle \& \ \ Peripherals & ECU, Gateway, Sensor, Actuator, Ethernet/CAN & Physical Protection, Access Control, Privacy \\
%     \hline

%     Communication & Cloud & Vehicle to Cloud & Integrity, Freshness, Manageability, Usability, Privacy, Attack Detection, Non-repudiation, Access Control  \\
%     \hline
%     Communication & Infra \& Edge & Vehicle to Vehicle/Road Side Units/Smartphone, Satellite to Vehicle/Base Station, Base Station (DGPS, Cellular) to Vehicle & Integrity, Freshness, Manageability, Privacy  \\ % Vehicle is considered a Infrastructure component
%     \hline
%     Communication & Vehicle \& \ \ Peripherals  & ECU to Gateway/ECU/Sensor/Actuator/Key & Integrity, Secure Information Flow, Usability, Privacy  \\
%     \hline

%     Software & Cloud & Web API, Web Protocols, Source \& Destination, Time, Database, Session Management, Queues, Events & Usability, Integrity, Access Control, Manageability, Privacy, Attack Detection  \\
%     \hline
%     Software & Infra \& Edge & Networking Stack & Usability, Integrity \\
%     \hline
%     Software & Vehicle \& \ \ Peripherals & APIs, Services, Queues, Events, Time & Usability, Integrity, Manageability, Privacy, Attack Detection, Non-repudiation, Access Control, Freshness, Secure Information Flow, Fair Exchange \\ % Fair exchange with regard to over the air software updates !!!, this means that receiver is able to prove that exchange was completely supplied, and allows to reclaim something is something did not work out
%     \hline
%   \end{tabular}
% \end{table*}





% we dont expect attackers to go to internet base stations and attack physically, physical attacks only on vehicle, but not in cloud or infrastructure and edge
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\caption{IoV Cyber Attack Vector Propagation}
\label{tab:attackpropagation}
\centering
\begin{tabular}{|p{6em}|p{6em}|p{48em}|}
%\begin{tabular}{|p{1.6cm}|p{1.5cm}|p{3.75cm}|}
\hline
\textbf{Attacker Type} & \textbf{Model Type} & \textbf{Attack Vector Propagation}  \\
\hline
\hline
Authorized & Cloud & \textbf{Cloud Access (SW)} $\Rightarrow$  \textbf{Vehicle \& Peripherals (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (SW)} $\Rightarrow$ \textbf{Target \ac{ecu} (DATA)} \\
\hline
Authorized & Infra \& Edge & \textbf{Infra \& Edge Access (SW or COM)} $\Rightarrow$ \textbf{Vehicle \& Peripherals (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (SW)} $\Rightarrow$ \textbf{Target \ac{ecu} (DATA)} \\
\hline
Authorized & Vehicle \& \ \ Peripherals & \textbf{Vehicle \& Peripherals Access (HW)} $\Rightarrow$ \textbf{Target \ac{ecu} (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (SW)} $\Rightarrow$ \textbf{Target \ac{ecu} (DATA)} \\
\hline
%Authorized & In-Vehicle & \textbf{HW Access}: vehicle \& peripherals $\Rightarrow$ \textbf{COM Attack}: vehicle \& peripherals to target \ac{ecu} $\Rightarrow$ \textbf{SW Attack}: target \ac{ecu} \\
%\hline
Unauthorized & Cloud & \textbf{Cloud (COM)} $\Rightarrow$ \textbf{Vehicle \& Peripherals (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (SW)} $\Rightarrow$ \textbf{Target \ac{ecu} (DATA)} \\ % maybe requires $\Rightarrow$ \textbf{Cloud Attack (SW)} at step 2 !!
\hline
Unauthorized & Infra \& Edge & \textbf{Infra \& Edge (COM)} $\Rightarrow$  \textbf{Vehicle \& Peripherals (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (SW)} $\Rightarrow$ \textbf{Target \ac{ecu} (DATA)} \\
\hline
Unauthorized &  Vehicle \& \ \ Peripherals &   \textbf{Vehicle \& Peripherals (HW or COM)}  $\Rightarrow$ \textbf{Target \ac{ecu} (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} (SW)} $\Rightarrow$ \textbf{Target \ac{ecu} (DATA)} \\
\hline

% Authorized & Cloud & \textbf{Cloud Access (SW)} $\Rightarrow$  \textbf{Vehicle \& Peripherals Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (SW)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (DATA)} \\
% \hline
% Authorized & Infra \& Edge & \textbf{Infra \& Edge Access (SW or COM)} $\Rightarrow$ \textbf{Vehicle \& Peripherals Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (SW)} \\
% \hline
% Authorized & Vehicle \& \ \ Peripherals & \textbf{Vehicle \& Peripherals Access (HW)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (SW)} \\
% \hline
% %Authorized & In-Vehicle & \textbf{HW Access}: vehicle \& peripherals $\Rightarrow$ \textbf{COM Attack}: vehicle \& peripherals to target \ac{ecu} $\Rightarrow$ \textbf{SW Attack}: target \ac{ecu} \\
% %\hline
% Unauthorized & Cloud & \textbf{Cloud Attack (COM)} $\Rightarrow$ \textbf{Vehicle \& Peripherals Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (SW)} \\ % maybe requires $\Rightarrow$ \textbf{Cloud Attack (SW)} at step 2 !!
% \hline
% Unauthorized & Infra \& Edge & \textbf{Infra \& Edge Attack (COM)} $\Rightarrow$  \textbf{Vehicle \& Peripherals Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (SW)}\\
% \hline
% Unauthorized &  Vehicle \& \ \ Peripherals &   \textbf{Vehicle \& Peripherals Attack (HW or COM)}  $\Rightarrow$ \textbf{Target \ac{ecu} Attack (COM)} $\Rightarrow$ \textbf{Target \ac{ecu} Attack (SW)} \\
% \hline
%Unauthorized & In-Vehicle &  \textbf{HW or COM attack}  \\
%\hline
%\end{tabular}
%\end{table}

  \end{tabular}
\end{table*}


% \subsection{Scenario Specific Attacker Analysis}


%% old state
% attacker goals, data of locaton services is ultimate goal and attacker has to specify different attack goals between softwafe, hardware, or communication surface to attack data
% To figure out the roots as well as the leaves of an attack vector, it is necessary to apply the attacker view analysis of \cite{10.5555/3067087} and \cite{maple2019connected}. 
% With the ultimate goal to compromise data that serves for position estimation, an attacker has the possibility to target the attack surfaces of communication or hardware in order to propagate to the \ac{ecu} that runs the software for location data processing \cite{karlsson2017future}.
% Before reaching the software component of the location service, any disturbance during data acquisition, processing, storage, and the phenotype of data can cause the location service to fail. 
% Therefore, attacking communication, processing, storage, and the phenotype of data represent the other main goals in the attacker model of connected and automated vehicles \cite{monteuuis2018attacker}. 
% The attack goals urge the attacker to decide upon an attack surface vulnerability to exploit. 
% This choice depends on the capability of the attacker, the information gathering that the attacker performs in order to identify system susceptibility, and threat accessibility.


%% very old state, do not copy in
% % might go into background and this needs rewriting in the the sense that 
% The attacker capability follows the categorization options of beginner, intermediate, and expert \cite{abraham2016estimating}.
% The extend of system information gathering and vulnerability/susceptibility exploitation increases in respect of attacker capability. 
% Concerning threat accessibility, latest attacker models in the \ac{iov} consider different general dimensions that apply to and attribute/categorize an attacker during threat access exploitation \cite{monteuuis2018attacker}.
% The dimensions to describe an attacker are membership, motivation, scope, method, and goal.
% Membership refers to the affiliation of the attacker in form of authorized insider or unauthorized outsider. Trusted developers or device owners count as authorized protagonists \cite{arm2009security}.
% Motivation differentiates the motives of maliciously damaging an asset or rationally exploit profit.
% The scope attribute describes the share of compromised infrastructure which an extended or local attacker controls.
% Last, the method attribute labels attacks as active or passive whereas the goal direct versus indirect attackers categorize. Direct attackers reach the intended target.

%% old state
% Endowed by the general dimensions of \cite{hutzelmann2019comprehensive} and following the attack model frameworks \cite{monteuuis2018attacker}, an attacker can gain accessibility to the \ac{iov} system by disrupting sensors, maliciously mechanic hardware from inside or outside of the vehicle \cite{petit2014revisiting}, attack communication, or persuade fusion. 
% Again, fusion persuading aims to trick data processing algorithms.
% Details about which type of asset to attack in each category can be seen in the evaluation Table \ref{tab:attackpropagation}.
% The starting point of the attack vector can be mapped to one of the \ac{iov} reference model categories. 
% The threat modeling analysis which determines the scores of Table \ref{tab:cvssscores} outlines attack and defence mechanisms for an assets per reference model category.
% The scope, goal, and motivation of the attacker determine whether the attack propagates to the final state to attack data.


\subsection{Attack Vector Construction}

Together with the attacker analysis and the 4+1 view model attack surface evaluation, it is possible to construct attack vector propagation towards the ultimate goal of interfering with location service data within \ac{ecu} software. 
Attack vectors target the identified assets in the different categories of cloud, infrastructure and edge, and vehicle and peripherals.
Thereby, attacks face an attack surface of view model determined hardware, networking, software, or data domains. 
By inspecting all different dimensions of an attack, the attacker has different initial positions to access the system. 
An authorized attacker has access to the cloud infrastructure by using credentials. % needs reference 
Logged into a platform, such an attacker initially starts to attack the system software to gain further access. 
A trusted developer as the most advantageous attacker potentially leverages security keys to start from an even deeper level of cloud software access. 
On the contrary, unauthorized attackers need to attack the cloud infrastructure with communication attacks.
Communication attacks such as session hijacking lead to platform access whereas unprotected \ac{api}s to full privilege software access leads. % reference here
In the reference model category of infrastructure and edge, unauthorized attackers can only attack communication vulnerabilities. 
In the authorized case, attackers have further opportunities to leverage the software of accessible edge devices as attack vectors to target vehicle and peripheral assets.
In the vehicle and peripheral domain, authorized staff such as in-vehicle operators find themselves in a situation with direct access to assets. 
After all, the barrier of attacking hardware remains as operators require access to covered hardware interfaces such as \ac{obu}s \cite{song2016intrusion}.
Unauthorized vehicle and peripheral attackers delude vehicle \ac{obu}s through communication as well as hardware attacks. 


% section about propagation
From the initial attacking positions, attacks propagate with different distances and attack types towards in-vehicle \ac{ecu}s.
Travel distance especially depends on factors such as attacker scope, motivation, and method.
Cloud attacks travel from cloud assets over vehicle gateways to target \ac{ecu}s. 
Infrastructure and edge attacks influence \ac{gps} infrastructure or vehicle \ac{obu} sensing. 
Affected data propagates into multi sensor fusion algorithms and mutates the results of position estimation.
The same data propagation distance holds for attacks on vehicle peripherals. 
Vehicle and in-vehicle attacks face the shortest propagation distance towards the electronic vehicle architecture.
Table \ref{tab:attackpropagation} summarizes the attack vector propagation of different attacker categories that attack from different initial positions. 
The attack vector propagation highlights attacks of different types at different stages.
The reason for grouping the propagation stages with regard to hardware, communication, and software attacks serves for attack to asset mapping facilitation and follows the 4+1 view model structures.  
The categorization allows to build defence mechanisms per category per attack stage.
This modular separation is a prerequisite for mapping attack and defence components for detailed risk assessment. 
% in a multi-layer defence framework.
%%%%%%%%%%%%% IMPORTANT reference this in intoduction




% this descriptive part maybe put it into more organisational part somewhere, if there will be a more suitable location in future
% The following section \ref{soaattackanalysis} identifies system hacking attacks which can be used to attack the different stages of the attack vector propagation. 
% Implicitly, the analysis of attacks on assets is the basis of backpropagation concepts and completes the attacker analysis. 
%The three left most columns of the resulting Table \ref{tab:attackanalysis} show the mapping of attacker capability to threat accessibility. 



\subsection{Quantitative Security Verification Model}
\label{evalmodel}


We choose a slightly simplified version of the attack realization metric and algorithm of \cite{cheng2012research} to demonstrate the applicability of Markov Chain models on attack propagation graphs that follow categorization structures of the 4+1 view model analysis.
% simultaneously evaluate and demonstrate the applicability of the proposed framework. 
The security evaluation of this approach utilizes the simulation model of an extended Markov Chain. % applied to an attack graph. 
The reason to rely on the basic extended Markov Chain and not on non-homogenous continues-time Markov models as in \cite{abraham2016estimating} is the fact that the extended Markov Chain suffices in modeling the high level attack graph of our scenario. % ,as introduced in \ref{evalmodel},
Moreover, the application is able to showcase the behavior of the proposed security framework in section \ref{section6}.
All five hypothesis of the assumptions of \cite{cheng2012research} equally apply to the \ac{iov} assets.


% general question, would it be possible to say the set of actions contains defence mechanisms and attack mechanisms??? 

% I need a nicer way to indicate the attack surface type, and the reference model type(depends on the state)

The discrete-time finite state Markov Chain models a time and state discrete stochastic process where the future state at time $t_{i+1}$ depends on the current state at time $t_{i}$ only and does not rely on past states at time $t_{-1}$.
Per definition, the Markov Chain $MC(I, P, A)$ is a 3-tuple consisting of system state space $I$, transition probability matrix $P$, and a set of possible atomic actions $A$. 
Additionally, the following characteristics count for state, transition, action, and state to target probability of attack realization respectively.
\begin{enumerate}
    \item $S_{i} \in I$, where $S_i$ is either of HW, SW, COM asset/attack surface type and is part of either one of the reference model types. Moreover, a concrete number of security requirements apply to the asset $S_i$.
    \item $\forall i=1,2,\dots$;  $\sum_{j=1}^{\infty} p_{ij} = 1$; %$p_{ij} \in \{1-a_{j}, a_{j}, a_{j}(1-d_{j}), a_{j}d_{j}+(1-a_{j})(1-d_{j}), 1-d_{j}, d_{j}, d_{j}(1-a_{j}) \} $; $ a $ probability of successful attack; $ d $ probability of successful defence mechanism.
    \item $a_{i}, d_{i} \in A$ probabilities of successful attack and defence mechanism in respect of asset/attack surface, reference model type, and security requirement
    \item $W^{n}(S_{i=1})= \sum_{S_i \in SUBSEQ(S_1)} \sum_{a_i,d_i \in RULES(S_1 \rightarrow S_i)}$ $ p_{ij}*E(a_i,d_i)*W^{n-1}(S_i)$, where $E(a_i,d_i)$ represents the attack/defence realization. $SUBSEQ$ returns the set of remaining states $S_i$ and $RULES$ marks the set of possible attack and defence actions. 
\end{enumerate}

Due to the high level attack vectors of Table \ref{tab:attackpropagation} and due to the evaluation purpose of the framework, we can assume that there is no empty action that affects the realization metric $E$. Hence, we can set it equal to one. 
To further simplify, we can remove both sums of the state to target probability as we are only interested in the worst case attack with maximum effect due its high significance.
This direction keeps transitions between states that connect starting and target states without detours.
The weight of multiple probabilities of attacks and response actions reduces to the state transition probabilities that are depicted in Figure \ref{fig:transitionprobgraph}. 



% The transition probabilities for the initial, consecutive, and final transitions are the following respectively.
% \begin{itemize}
%     \item $p_{0j}=(1-a_j) + a_j = 1$
%     \item $\sum_{j=1}^{\infty} p_{ij}= a_{j}d_{j} + (1-a_{j})(1-d_{j}) + a_{j}(1-d_{j}) + d_{j}(1-a_{j}) = 1$
%     \item $p_{nj}=(1-d_j) + d_j = 1$
% \end{itemize}
% Figure \ref{fig:transitionprobgraph} shows the transition probability graph.

Regarding the state transition probabilities of attack and defence reaction actions, the initial state only starts with either an successful attack or remains in the set of initial states. 
Similarly, the last state only changes through an effective response action against the attacker.
In the intermediate steps, states remain the same if either no action occurs ((1-a)(1-d)) or an successful attack faces immediate countermeasures (ad). 
If an attack action succeeds and no defence reaction occurs, the attacker moves to the next state.
Vice versa, failing attacks and successful reactions may transition the attacker backwards.
Section \ref{evalassumptions} outlines our approach to determine the probabilities which suffice the purpose of a quantitative evaluation of our proposed security framework.
% maybe rename d to c for countermeasure, because it is a system reaction!! 
Other characteristics of the model are the sum of outgoing weights of each state which sum up to the value one. 



When it comes to parameter modeling of the attack and defence probabilities, we take the vulnerabilities assessment, that is faced in the respective the attack surface stage, as the attacking probability $a$.
% Next, the probabilities of attack actions depend on the vulnerabilities assessment faced in the respective the attack surface stage.
Thereby, the stage of the attacker depends on the surface type of hardware, networking, software, and data as well as the reference model type of the asset under attack. 
Since the \ac{cvss} score has a maximum possible value of $42.5$, we normalize each vulnerability score with respect to this value.
In the end, this gives the attack probability formula of \ref{formula0} where $i$ refers to the attacking stage in the attack tree which determines what reference model type and, thereby, vulnerability type to choose.
For instance, the formula $f_{cvss} (2)$ of the second attack path of Table \ref{tab:attackpropagation} returns a vulnerability score of type networking.
\begin{figure}[!ht]
    \centering
    % \begin{tikzpicture}[scale=0.9]
    
    % \end{tikzpicture}
    \begin{tikzpicture}[scale=0.9, ->, >=stealth', auto, semithick, node distance=1.8cm]
        \tikzstyle{every state}=[fill=white,draw=black,thick,text=black,scale=1]
            \node[state]    (A)                     {$i=1$};
            \node[state]    (B)[right of=A]   {$\dots$};
            \node[state]    (C)[right of=B]   {$i$};
            \node[state]    (D)[right of=C]   {$\dots$};
            \node[state]    (E)[right of=D]   {$i=n$};
            \path
            (A) edge[loop above]     node{$1-a$}         (A)
                edge[bend left]     node{$a$}     (B)
                %edge[bend left,below]      node{$p(1-p)$}      (D)
                %edge[bend right]    node{$p(1-p)$}      (C)
            (B) edge[bend left]    node{}           (C)
                edge[bend left, below]    node{}           (A)
            (C) edge[bend left]    node{$a(1-d)$}   (D)
                edge[loop above]     node{$ad+(1-a)(1-d)$}   (C)
                edge[bend left, below]     node{$d(1-a)$}   (B)
            (D) edge[bend left]     node{}     (E)
                edge[bend left, below]    node{}    (C)
            (E) edge[loop above]    node{$1-d$}     (E)
                edge[bend left,below]    node{$d$}      (D);
                %edge[bend left]     node{}      (C)
                %edge[bend left,above]     node{}         (B);
            %\node[above=0.5cm] (A){Patch G};
            
            % red circle
            % \draw[red] (0.4,1) ellipse (1cm and 1cm)node[yshift=1.2cm]{$\sum = 1$};
        \end{tikzpicture}
    
  \caption{Markov Chain Transition Probability Graph of Attack and Reaction Transition Probabilities}
\label{fig:transitionprobgraph}
\end{figure}
It is moreover possible to extend the model of the attack probability $a$ per stage $i$ by introducing another Formula \ref{formula02} which describes the increase of the attacking likelihood for increasing stages $i$.
The underlying assumption for the necessity of such a value is the fact that a single successful attack opens up opportunities to compromise more vulnerabilities or combinations of vulnerabilities which increases the likelihood of an successful attack.
The resulting function for such an enhanced attack probability would follow a negative exponential function with negative exponent, as shown in equation.
\begin{equation}
\label{formula0}
a_i = \frac{f_{cvss} (i)}{42.5}; \hspace{5mm} i \in \mathbb{N}.
\end{equation}
\begin{equation}
\label{formula02}
a_i = 1-e^{-i*\frac{f_{cvss} (i)}{42.5}}; \hspace{5mm} i \in \mathbb{N}.
\end{equation}


% The amount of security requirements influence the attack probability of an asset under attack due to the increasing system complexity with affects system susceptibility and makes successful attacks more probable. 
The defence mechanism probabilities $d$ depend on actual attack actions. 
Nevertheless, we model successful countermeasure probabilities independently of the causing attack due to missing attack attribution formulas which would enable attack identification, assessment, and reaction actions for all attacking stages.
This measure also simplifies the quantitative calculations within the Markov Model for now but requires further investigation in the future. 
The framework evaluation in section \ref{section6} applies the security verification model in order to evaluate out proposed security methodology. 

% if they cause detection, we model them independently. 
% Again, the reason for it is the focus on the evaluation of the proposed security framework.

% \todo{indiccate tuning idea, with propagation with dependency to stage index which increases attack probability, also state the attacker to target distance which we know as system designers}


%The probability distributions among the transition actions require tuning.












































%continue here and describe trees, asset identification and goal description is enough for it, then inspect attacks in more detail !!! better flow this way

%just describe table 3


%By considering the attacker goal, capabilities, and view as well as the identified state-of-the-art threats, it is possible to construct attack trees. Similar to the attack surface asset evaluation, the attack tree construction groups all abstract attack classes per attack surface asset. From there and with the help of the asset identification, it is possible to create several attack graphs which are shown in Figure \ref{}.

%defender view on the system and together with the process view for attack propagation possibilities that occur from entering the attack surface, we identifies the following attack trees to for each attacker category 

%the attack goal in our scenario is the location service !!



%where is automation of attack trees possible, why using attack trees and not probabilistic models ? reason is agile threat modeling, read up again on other methodologies and when to use them

% access level of mechanism
%      - network-level:  between devices
%      - device-level:   between processors of one device
%      - program-level:  between software classes of the same program
%      - hardware-level: physical matter

% \todo{
% state again that identified assets are the attack surface that is first connected, and these assets make up the attack starting point of table 3 
% }
% \todo{
% either figure of attack propagation or table, table for now
% }

%With the attribution of the dimensions, an attackers threat access depends on the locality and physical access to the system. ...

%Second, an attacker gains accessibility to a system by disrupting sensors, maliciously mechanic from inside or outside of the vehicle, attack communication, 
%Details about which assets to attack in each category can be seen in the evaluation Table \ref{tab:attacksurfevaluation} 

%The threat accessibility, in the form of logical and physical reachability of an attack surface to the attacker, is modelled in different dimensions. 

%The attacker model of smart vehicles specifies sensor confusion, evil mechanic, and communication attacks \cite{petit2014revisiting}

%The following section \ref{soaattackanalysis} identifies system hacking attacks that enable attacks on assets and complete the attacker analysis. 
%The three left most columns of the resulting Table \ref{tab:attackanalysis} show the mapping of attacker capability to threat accessibility. 

%The attacker goal to our predefined localization scenarios it to compromise either all, a combination, or one of the scenarios.
%By following the attacker model for connected and automated vehicles of \cite{monteuuis2018attacker}, attackers compromise the scenario by either attacking  if the 
%For compromization, 

%Following the categorization of \cite{arm2009security}, attackers are either remote, specialists, trusted developers, or device owners. 
%Each of the attacker role  These different roles of attackers 
%From the location perspective in the infrastructure and attacker can have the following possibilities to interact with the hardware components: \cite{monteuuis2018attacker}


% \subsection{State-of-the-Art IoV Threats and Defence Mechanisms}
% \label{soaattackanalysis}
% %% this chapter is the threat modelling
% \todo{remove this section and include into threat and defence mechanism threat modeling per view, also add where possible to attack tree construction}

% At the different stages of the attack propagation, attackers rely on a variety of attacks. 
% Table \ref{tab:attackanalysis} summarizes the attack repertoire and groups attacks in respect of the type of the attack surface.
% The collection of attacks originates from the following \ac{iov} attack reviews and surveys.
% The work, presented by Cui et al. \cite{cui2019review}, dominates the attack findings of the first four rows and the last row of Table \ref{tab:attackanalysis}.
% The work of Abdul-Ghani et al. \cite{abdul2018comprehensive} covers the rows of physical protection, freshness, secure information flow, and attack detection. 
% % The study of Abdulghani et al. \cite{abdulghani2019study} contributes to the rows of fare exchange and non repudiation. Here, the security requirement of trustworthiness expresses the intention of the term  fare exchange with different wording. 
% % The listed attacks on manageability derive from the ranking of Kettani et al. \cite{kettani2019top}.
% All reviewed surveys propose countermeasures that are incorporated as much as possible in our multi-layer security solution of section \ref{proposedsolution}.


% \subsection{\ac{iov} Cyber Defence State of Practice} % (existing technologies)
% \label{countermeasuresiov}
% \subsubsection{Mitigation \& Countermeasures}

% \todo{heavily reduce references!}
% The overview of defence mechanisms groups all potential countermeasures with regard to security requirements and attack surface types. Table \ref{tab:defenceanalysis} shows the summary of all collected defence concepts of the following surveys.
% The works \cite{cui2019review}, \cite{abdulghani2019study} bring together and categorize countermeasures against attacks that target \ac{iov} specific hardware, software, and communication, data at rest, \ac{iot} software, communication protocols, network communication, connectivity, and physical hardware.
% Next, the following works highlight the importance of the selected concepts of interoperability \cite{eu2018road}, \ac{gdpr} \cite{sfakianakis2019enisa}, dynamic and automated risk assessment \cite{rao2017probabilistic}, attack prediction and attribution \cite{patel2013classification}, threat predictive analytics, monitoring, and detection intelligence \cite{nec18itaru}, encrypted traffic analysis \cite{cheng2018encrypted}, forensic readiness \cite{valjarevic2013harmonized}, intrusion detection and intrusion prevention \cite{anwar2017intrusion}, penetration testing \cite{scarfone2008technical}, and honeypots \cite{wahlisch2013design}. 
% The collection of countermeasures serves for orientation about which countermeasure to apply in what layer of the proposed multi-layer security concept.
% Even though the state of practice of defence mechanisms covers a very wide range of attacks, shortcomings remain \cite{parkinson2017cyber}.


%%% include gaps !!
% Even though the state of practice of defence mechanisms covers a very wide range of attacks, shortcomings remain. Problematic is the adaptation of security frameworks to latest security standards \cite{rasmussen2018gap}. It is therefore important to pay special attention to the following categories of security gaps of the works \cite{sun2017attacks},  \cite{barnard2014threat}, and \cite{parkinson2017cyber}.
% \begin{itemize}
%     \item Reduction of effects of existing systems
%     \item External effects
%     \item Long term studies of fast evolving security techniques
%     \item Knowledge Gaps and their potential impact
%     \item Human error and criminology
%     \item Impact of law, policy, and liability
% \end{itemize}



% The overview of defence mechanisms groups all potential countermeasures with regard to security requirements and attack surface types. Table \ref{tab:defenceanalysis} shows the summary of all collected defence concepts of the following surveys.
% The works \cite{cui2019review}, \cite{jang2014survey}, \cite{abdulghani2019study}, and \cite{abdul2018comprehensive} bring together and categorize countermeasures against attacks that target \ac{iov} specific hardware, software, and communication, data at rest, \ac{iot} software, communication protocols, network communication, connectivity, and physical hardware.
% Next, the following works highlight the importance of the selected concepts of interoperability \cite{eu2018road}, \ac{gdpr} \cite{sfakianakis2019enisa}, dynamic and automated risk assessment \cite{rao2017probabilistic}, attack prediction and attribution \cite{patel2013classification}, threat predictive analytics, monitoring, and detection intelligence \cite{nec18itaru}, encrypted traffic analysis \cite{cheng2018encrypted} \cite{anderson2017machine}, forensic readiness \cite{valjarevic2013harmonized}, intrusion detection \cite{haas2017intrusion} \cite{alheeti2016hybrid}, intrusion prevention \cite{anwar2017intrusion} \cite{anuar2009response}, penetration testing \cite{scarfone2008technical}, and honeypots \cite{wahlisch2013design}. 
% The collection of countermeasures serves for orientation about which countermeasure to apply in what layer of the proposed multi-layer security concept.

% \begin{table}[htbp] % [!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{IoV Cyber Attack Evaluation}
% \label{tab:attackanalysis}
% \centering
% \begin{tabular}{|p{1.25cm}|p{5.5cm}|p{0.8cm}|} % p{1cm}|
% \hline
% \textbf{Affected Requirements} & \textbf{Attack} & \textbf{Surface Type} \\  % & \textbf{Category}   \\
% \hline
% \hline
% Access control & Sybil, Falsified entities, Replication, \ac{gnss} spoofing and injection, Timing & All \\ %%  & Create, Modify  \\
% \hline
% Usability & Jamming, Flooding, Malware, Spamming, \ac{dos}, Wormhole & All \\ % & Create, Modify, Read, Remove  \\
% \hline
% Integrity & Masquerading, Replay, Alteration, Tampering, Map database poisoning  & COM, SW    \\ % & Create, Modify \\
% \hline
% Privacy & Eavesdropping, Interception & All  \\ % & Read, \ \ \ \ Interrupt, Modify \\
% \hline
% Non-repudiation & Remnant usage, Manipulation, Insider & SW, COM  \\ % & Modify, Remove \\
% \hline
% Manage- ability & Spam, Ransomware & SW  \\ % & Interrupt \\
% \hline
% Physical Protection & Outage, Physical damage, Node replication, Side-channel attack, Tampering, Jamming, Camouflage, Cloning, Hardware Trojans, Tag interference, Injection  & HW   \\ %  & Interrupt, Modify  \\
% \hline
% Attack \ \ Detection & Backdoor, Unknown, Trojans, Misconfiguration  & SW     \\ %   & Create, Read \\
% \hline
% Fare Exchange & Remnants usage, Insider, Spoofing, Hijacking &  SW, HW  \\ %  & \\
% \hline
% Freshness & Leakage, Hash collision, Manipulation, Exposure, Loss & SW    \\ % & Modify, Remove, Read, Create \\
% \hline
% Secure Information Flow & Time, Stripping, Flooding, Fragmentation, Hijacking, Sniffing, Overflow, Forward, Wormhole, Sybil, Black hole, Version  & COM, SW    \\ % & Read, Create, Interrupt, Remove \\
% \hline
% Confor-mance & Malware  & SW   \\ % & x \\
% \hline
% \end{tabular}
% \end{table}

%%%% Ask mudassar on every table and every column:
% in this table case, why not remove category column on the right, remove if not used in defence framework simplification !!





















% Categorization of communication attacks:
% \begin{itemize}
%     \item Regular communication (not interception) (affects no one, remove, just here for comparison
%     \item Read (eavesdrop) (affects sender, sender required)
%     \item Modify (affects message of sender, sender required)
%     \item Create (affects only receiver, no sender required)
%     \item Interrupt (disturb or interfere message, sender required)
%     \item Remove (catch message and drop, sender required)
% \end{itemize}

% We have the following attack goals
% \begin{itemize}
%     \item point cloud map of SLAM
%     \begin{itemize}
%         \item Modify, Remove, gain access an read
%     \end{itemize}
%     \item vehicle to cloud communication catch position of vehicle
%     \begin{itemize}
%         \item modify data, affects only cloud service but not vehicle safety - vehicle people stay safe
%     \end{itemize}
%     \item vehicle DGPS communication 
%     \begin{itemize}
%         \item affects real position data outcome and thereby safety of vehicle
%     \end{itemize}
%     \item Sensor data processing attack
%     \item internet communication attack agps
%     \begin{itemize}
%         \item affects safety as well
%     \end{itemize}
% \end{itemize}

% FIGURE OF FOUR ATTACK VECTOR GRAPHS AND PROPAGATIONS TO GOAL
%- this follows the approach that is referenced in background


%We assume that the attacker tries to attack our predefined scenarios of localization determination. 




%%%% MORE DETAILED MOTIVATION EXAMPLE
%This means, the goal of the attack is to either modify (total modification is remove/delete), prevent, or passively gain read access to location data of the vehicle. (whats the benefit of read access to the data: allows attacker to create map of all compromised vehicles which violates privacy laws ..cite here..) 





% \begin{enumerate}
%     %\item position data needs to be protected -- done
%     %\item final position data determined in software -- done
%     %\item attacker needs to compromise software -- done
%     %\item before that attacker needs to compromise either communication or gain hardware access to be able to get access to software -- done
%     %\item attacker can have the following locations to attack hardware: in vehicle, outside of vehicle, in vehicle as expert, in vehicle as fake/malicious employee (insider attack), identify: ATTACKER ROLES and ATTACKER SURFACE INTERACTION  -- done
%     %\item identify: ATTACKER ROLES and COMMUNICATION SURFACE INTERACTION -- done
%     % \item abstract attack types: read, write, execute, break/remove/destroy file , this means eavesdrop, modify/inject, spoof -- counts as create, jamming counts as interrupt  -- todo
% \end{enumerate}

%The attack identification differentiates between different types of attacker stages.
%The physical attack surfaces are inside the vehicle, 


%- attacks from D2.1 history of attacks
%Attacks, Threats, Attack Agents, Attack Vectors, Attack Propagation


%% summing up literature review of deliverable D2.1

%- history of attacks: 
%references: and then summary


%- layers from deliverable go into direction of reference model

%- potential attacks on AV and AV communication networks 14


% - then 15/16
% - Denial-of-service (DoS) and distributed denial-of-service (DDoS) attacks 
% - TCP/SYN flood attack 
% - Teardrop attack 
% - Smurf attack 
% - Ping of death attack 
% - Botnets Man in the middle attack (MitM) 
% - Session hijacking 
% - IP/GPS spoofing 
% - Replay 
% - Wormhole 
% - Phishing and spear phishing attacks 
% - Drive by attack 
% - Password attack 
% - SQL injection attack 
% - Cross-site scripting (XSS) attack 
% - Eavesdropping attack 
% - Birthday attack 
% - Malware attack 

% ---- next types of attacks in IoV: arrow direction is important !!
% Attacks on authentication 
% - wormhole attack: concealing (tarnen/verbergen) of real distance between two malicious nodes from normal nodes, in order to absorb data flow and cause network conjunction(verknüfung-verUNDung) or perform other malicious interactions
% - masquerading, copy of same id 
% - gps deception: supply fake info about location speed or other gps attributes, crucial to localization system
% - sybil attack: complicated, creation of multiple equal identities, identity generation for confusion

% Routing attacks (!important because mentioned in dynamics IoV background)
% - route modification: modification of number of hops in forwarding request packets or other routing info 
% - masquerading attack (fake identity (network identity) attack to get access, masque venecia)
% - denial of service attacks 
% - eavesdropping attack 

% data authenticity attacks 
% - replay attacks (possible through secrecy attacks for ex)
% - camouflage attack: cloaking/masquerading (verhüllend) node under false ID, then legitimately authenticated= authenticity attack successful - then creation/fabrication attack of false/malicious messages
% - fabrication attack, tampering with messages, used in way to catch message and masquerade/hide sensed evidence to hide vehicle attacks 17
% - Illusion attack: other generation attack of false data from sensors that are properly authenticated and identified in network: this attack also after failing authenticity attack

% availability attacks 
% - DOS DDOS , interferance attacks exploitation of bandwidth and transmission power to collapse system

% secrecy attacks 
% - target secret and private info such as user identities + pw to (eavesdropping or interception of network)


% Attack references to read: 13 (Attacks and countermeasures in the internet of vehicles, 
% Sun2017_Article_AttacksAndCountermeasuresInThe.pdf), 17 (Kannhavong B, Nakayama H, Nemoto Y, Kato N, Jamalipour A (2007) A survey of routing attacks in mobile ad hoc networks. IEEE Wirel Commun 14(5):85–91), 14 (A review on safety failures, security attacks, and available countermeasures for autonomous vehicles, 1-s2.0-S1570870518309260-main.pdf ), 15 (A Brief Survey on Autonomous Vehicle Possible Attacks,Exploits and Vulnerabilities, 3d23100777db3f273a21208f06d74410312d985a.pdf), 16 (Andreea Bendovschi, “Cyber-Attacks – Trends, Patterns and Security Countermeasures”, 13-14 April 
% 2015;https://www.researchgate.net/publication/283967866_Cyber-Attacks_-
% _Trends_Patterns_and_Security_Countermeasures), 12 (Cybersecurity Best Practices for Modern Vehicles, 812333_cybersecurityformodernvehicles.pdf ), 11 (https://www.statista.com/statistics/194083/global-top-attack-categories-of-cyber-attacks/ ), 94 (), 95 ()



% History: 1 (https://medium.com/driving-to-the-future/how-to-avoid-cyber-attacks-to-connected-vehicles-
% 16a801ba7eb3), 2 (https://blog.appknox.com/cyber-attacks-in-connected-cars/), 3 (www.iara.biz/docs/03_05_18_IARA_CAR_2018_Presentation_FINAL_AA_FF.pdf ), 4 (https://www.cnbc.com/2017/11/21/uber-hack-exposes-data-of-57-million-users-and-drivers-
% report-says.html ), 5 (https://www.vice.com/en_us/article/3kvw8y/researchers-hack-car-infotainment-system-and-fin-sensitive-user-data-inside )



%% NARROW DOWN:: summing up literature review of GHOST project deliverable review




%% NARROW DOWN:: summing up KONFIDO D3.1 deliverable literature review 




% 2017 - driving with sharks
% 2017 - cyber threats facing autonomous and connected vehicles
% 2017 - A threat to vehicular cyber security and the urgency for correction
% Malicious firmware update, attack on vehicle network, attack on key/certificate storage, attack from rouge apps in mobile devices, attack from downloaded apps, man in the middle attack, and malware on removable media mark the in vehicle threat vectors that apply to the decomposed skeleton of system assets of use case three \cite{rizvi2017threat}.

% Take a look at my mindmap


% GROUPING AND CAEGORIZATION FROM BEGINNING ON; MAYBE USE TABLE



% The IoV stakeholder requirement analysis uncovers the most relevant system assets and functionalities  






==> sections/1.2_methodology2.tex <==

\section{\ac{iov} Security Methodology based on 4+1 View Model Analysis}
% \section{Defence Mechanism Identification \& Security Design}
\label{section5}



\subsection{Introduction of Security Methodology}
\label{proposedsolution}

With the help of the view model analysis, it is possible to gain insights about the assets that contribute to the location service application of an \ac{iov} infrastructure. 
The output of the logical, developer, process, and physical view analysis identifies all relevant asset while at the same time mapping them to the categories of data, software, networking, and hardware.
During the system decomposition, the reference architecture marks one dimension to categorize assets next to the view model perspective.
This enables to apply the view model descriptions per reference sub-architecture. 
Sub-architecture modeling identifies application relevant assets which attract attackers.
Hence, they mark the targets and from there, it is possible to analyze threat, vulnerabilities, and potential defence mechanisms.
Connections between assets will pave the way for attack vectors towards the ultimate attacking goal.
Inspection of attack vectors between low level and domain specific assets may cause high complexity which causes graph modeling challenges \cite{mjihil2017improving}.
Using abstract and quantitative verification modeling concepts, as introduced in section \ref{evalmodel}, allows security verification of security concepts along attack vectors that affect different sub-architectures.

\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.9, ->, >=stealth', node distance=2.5cm]
    
    \node (el1) at (-1,10) [rectangle, anchor=west, thick, draw=black, fill=white!95!gray, minimum width=9.6cm, minimum height=0.5cm, transform shape = true, align=left] {Definition of Scenarios};
    \node (el1) at (-1,9) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=9.6cm, minimum height=0.5cm, transform shape = true, align=left] {\ \ \ \ \ \ \ \ \ \ Reference Architecture Domains\\ (Cloud, Infra \& Edge, Vehicle \& Peripherals, ...) };
    
    
    \node (abox1) at (-1,3.85) [draw, anchor=west, thick, fill=white!95!blue, align=left, minimum height=8.8cm, minimum width=2cm, transform shape = true] {};
    \node (vuln) at (-0.6,7.5) [transform shape = true, align=left, anchor=west] {Logical \\View};
    \node (a1) at (-0.6,6.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Assets};
    
    \node (abox1) at (1.5,3.85) [draw, anchor=west, thick, fill=white!95!red, align=left, minimum height=8.8cm, minimum width=2cm, transform shape = true] {};
    \node (vuln) at (1.75,7.5) [transform shape = true, align=left, anchor=west] {Developer \\View};
    \node (a1) at (1.85,6.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Assets};
    
    \node (abox1) at (4,3.85) [draw, anchor=west, thick, fill=white!95!green, align=left, minimum height=8.8cm, minimum width=2cm, transform shape = true] {};
    \node (vuln) at (4.4,7.5) [transform shape = true, align=left, anchor=west] {Process \\View};
    \node (a1) at (4.4,6.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Assets};
    
    \node (abox1) at (6.6,3.85) [draw, anchor=west, thick, fill=white!95!yellow, align=left, minimum height=8.8cm, minimum width=2cm, transform shape = true] {};
    \node (vuln) at (6.9,7.5) [transform shape = true, align=left, anchor=west] {Physical \\View};
    \node (a1) at (7,6.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Assets};
    
    
    \node (abox1) at (-0.8,3.7) [draw, anchor=west, thick, fill=white!95!gray, align=left, minimum height=4cm, minimum width=9.2cm, transform shape = true] {};
    \node (vuln) at (0.75,5.3) [transform shape = true, align=left, anchor=west] {Attack Analysis};
    \node (vuln) at (5,5.3) [transform shape = true, align=left, anchor=west] {Security Design};
    
    \node (a1) at (0,4.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=4cm, minimum height=0.5cm, transform shape = true, align=left] {Threat \& Vuln. Analysis};
    \node (a1) at (0,3.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=4cm, minimum height=0.5cm, transform shape = true, align=left] {Risk Analysis};
    \node (a1) at (0,2.5) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=4cm, minimum height=0.5cm, transform shape = true, align=left] {Security Requirements};
    
    
    \node (a1) at (5.25,4.5) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Prevention};
    \node (a1) at (5.25,3.5) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Detection};
    \node (a1) at (5.25,2.5) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Reaction};
    
    
    \node (el1) at (-0.8,1) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=9.2cm, minimum height=0.5cm, transform shape = true, align=left] {Attack Vector Construction};
    
    \tikzstyle{every state}=[fill=white,draw=black,thick,text=black,scale=1,transform shape = true]
            \node[state]    (A)               {};
            \node[state]    (B)[right of=A]   {};
            \node[state]    (C)[right of=B]   {};
            \node[state]    (D)[right of=C]   {};
            \path
            (A) edge[bend left]     node{}     (B)
            (B) edge[bend left]    node{}           (C)
                edge[bend left, below]    node{}           (A)
            (C) edge[bend left]    node{}   (D)
                edge[bend left, below]     node{}   (B)
            (D) edge[bend left, below]    node{}    (C);
            
            
    \node (el1) at (-1,-1) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=9.6cm, minimum height=0.5cm, transform shape = true, align=left] {Quantitative Unit/System Security Verification };

    \end{tikzpicture}
  \caption{View Model Security Methodology for the \ac{iov}}
\label{fig:mainsecuritydesigntailored}
\end{figure}


Our proposed modular and flexible view model security methodology of Figure \ref{fig:mainsecuritydesigntailored} combines the introduced concepts into consecutive processing steps.
After the initial scenario selection, it depends on the security engineer to determine the amount of sub-architecture abstraction domains.
For each of the sub-architectures, there is the selection of different view perspectives which identify assets and categorize connected infrastructure components.
Class, state, activity, communication, etc. diagrams or sequence charts structure assets.
To secure identified assets of the system, the attack analysis marks the next step.
Agile threat modeling and risk assessment per domain allows to iteratively extract and weight security requirements to improve unit or system wide security design. 
The choice of framework for each of the attack analysis procedures depends on the security expert.
Attack analysis between components moreover enables attack vector construction.
Table \ref{tab:attackpropagation} illustrates inter domain attack vectors which happen for example when an attacker performs network attacks after compromising software privileges.
Attack vector propagation stages together with risk assessment scores, which incorporate attack, vulnerability, and defence mechanism assessments, form the input for the final step of our methodology where we utilize probabilistic Markov Chains to model attack vector propagation as state transitions.
Table \ref{tab:cvssscores} for example indicates such risk assessment scores. 
This procedure provides quantitative security verification of single or multiple system units.
Subsection \ref{section6} applies the methodology to the location service use case analysis of this work and outlines constrains of the presented security methodology. 

The overall security methodology for the \ac{iov} architecture follows a very high abstraction level in order to connect the relevant domains. 
The resulting quantitative security assessment outlines initial problem zones which require more detailed inspection individually.
% When applied to a real use case, it is necessary to investigate attack and defence mechanisms for the most relevant sub-modules and assets first and in detail before designing quantitative system specific model checking concepts.
Next, the methodology remains extendable towards several aspects.
First, the amount of viewpoints can be increased to represent more detailed assets, attacks, and defence mechanisms.
Second, the reference model domains can change to group cohesive system aspects for better segmentation in respect of security analysis. 
The vehicle domain, for instance, allows splitting and prioritization between \ac{ecu}s, peripherals, and gateways.
Last and apart from abstract concepts, it is possible to increase or, if possible, mix the amount of scenarios. 
For instance, a secure infotainment application benefits from our security methodology if it aligns with similar comprehensive security aspects in any analysis domain.




% Regarding the reference architecture, it is possible to map the assets to cloud, infrastructure and edge, and vehicle and peripherals.
% The two mappings are important for the following reasons. 
% Since it is possible to categorize cybersecurity attacks and defence mechanisms with regard to hardware, software, communication, and data, this categorization among assets outlines what kind of threat vectors as well as prevention mechanisms apply to each asset. Next to threat identification and prevention techniques, the attacker capability and asset susceptibility contribute to risk determination of a specific asset.
% The \ac{cvss} score allows to incorporate all vulnerability relevant properties of an asset.
% The second reason for mapping assets to different reference model domains allows to set up attack vector propagation paths with the help of the process view. 
% Again, abstraction of assets into attack surface categories reduces complexity and facilitates attack vector construction. 
% This fact is important, as detailed attack vector propagation in the cloud domain alone comes with complex attack graph modeling challenges \cite{mjihil2017improving}. 


%builds upon the categories of attack surface type and reference model type. 
% Layer 1 to 4 of the framework show the categorization of the attack surface types. At the same time, the grouping of reference model types happens in each layer as well. 
% Next, our security framework requires a scenario that needs to be secured.
% The scenario guides the selection and identification of assets in respect of the attack surface and reference model type. 
% Table \ref{tab:attacksurfevaluation} shows the result of this step for the location service scenario.
% The threat modeling and risk assessment analysis in combination with the identified assets allows the construction of the attack vector propagation of Table \ref{tab:attackpropagation}.
% The table describes the access opportunities of the attackers while indicating the propagation between the attack surface types. 
% The prevention domain with upwards arrows in the left half of Figure \ref{fig:mainsecuritydesigntailored} shows the prevention design path from data to hardware assets. 
% It is of course possible for an attacker to attack and compromise the communication layer assets only which depends on the attacker motivation.
% During the attack and at each propagation stage, the attacker faces an attack probability of the Table \ref{tab:cvssscores} while facing defence mechanism probabilities that remain open to determine more accurately. % of Table \ref{tab:defenceanalysis}. 


% After setting up all possible prevention techniques, it is further necessary to investigate the data collection procedures that allow to track back attacks and contribute to successful attack detection, risk management, and verification models.
% Every asset of the respective reference model and attack surface category serves for data collection and monitoring purposes for the system wide detection process. 
% Relevant data that is necessary for the detection procedures need to reach the \ac{siem} component which determines the reaction and response action. 
% Depending on the affected asset, the \ac{siem} component relies on single module or system design decisions that enable the realization of the response strategy.
% It is moreover important to set up anonymization measures at respective interfaces to design a privacy regulation conform incident detection process.
% The right half of Figure \ref{fig:mainsecuritydesigntailored} indicates the response mechanism that has the ability to propagate backwards to each affected asset of the system. 
% It is important to emphasize the link of the \ac{siem} module to the respective stakeholder or system administrator that is part of layer 0. 
% As a matter of fact, decisions on response actions such as isolation, forensics, recovery, shut down, re-calibration, and notifications often depend on stakeholder decisions itself.
% In our location service scenario, the major reaction pattern is to re-establish the system critically level. 
% If the amount of defect system functionality is too high and location services cannot be guaranteed anymore, the vehicle must stop safely.







% \subsection{Overall Defence Concept}




% \todo{security design in every stage of the attack path, isolated layers enable step by step security concept application and verification of signle and system parts, thats the goal, this should be described in the overall defence concept}

% Preventing the attacker from reaching its goal means closing all conditions that make up vulnerabilities that eventually allow an attacker to reach the goal. 
% From the quantitative perspective, the focus on the most vulnerable assets reduces susceptibility. Moving physical and communication access out of the attacker's reach affects the attack surface accessibility. The mitigation of the attacker capabilities requires component diversity and system detection, reaction/identification, and adaption functionality \cite{hughes2013quantitative}.
% These basic mitigation concepts drive the design decisions of the final security design.

% % attack prevention
% With the insights of the identified assets of the system, it is possible to start mitigating threats on all assets through attack prevention techniques. 
% The prioritization of defence concept should target the most likely risks of assets first.
% Following this approach puts the focus on \ac{ecu} software that determines positions estimation. 
% At the same time, data assets represents the attackers most desirable goal when attacking location services.
% The risk assessment evaluation, driven by the 4+1 view model analysis,  Table \ref{tab:attacksurfevaluation} lists the security requirements for in-vehicle and peripheral software. 
% With Table \ref{tab:attackanalysis}, it is now possible to see which attacks apply to these security requirements and design prevention mechanisms accordingly. 
% Section \ref{countermeasuresiov} provides an overview of suitable state-of-the-art mitigation techniques for the \ac{iov} infrastructure. 
% The final security framework indicates if multiple prevention techniques need application to cover one or multiple security requirements. 
% Optimized importance weighting of prevention techniques remains future nonetheless. 
% By following the attack vector propagation, it is possible to reduce attack vector accessibility step by step. 
% This approach addresses transferred risk and guides security design in respect of risk avoidance and acceptance strategies.  
% For instance, to mitigate the attack vector of attacker type unauthorized and model type cloud, defence design tackles software attacks which originate from in-vehicle communication attacks. These communication attacks depend on gateway communication attacks which in turn belong to specified cloud communication requests. 


% % everything after attack prevention: --> SIEM platform
% The prevention techniques mark the first building block of three main security blocks proposed by the \ac{etsi} standardization specification for information security \cite{etsi008gsisi}. % important to follow eu regulations in security design
% Figure \ref{fig:mainsecurityblocks} shows the building blocks together with the \ac{etsi} \ac{siem} approach.
% The \ac{siem} framework allows attack detection, reaction, and adaptation which mitigates the attacker capability condition. 


% % detection examples and process explanation
% The detection of security critical events comprise different procedures. 
% Risk evaluation as the initial incident processing step feeds the parameterization of security policies. Examples for risk evaluation are vulnerability scores such as the \ac{cvss} score \cite{schiffman2004common}, \ac{dread}, \ac{stride} \cite{cagnazzo2018threat}, or the location of the incident detection along an attack path which aggregates metrics such as the \ac{mttc} \cite{nzoukou2013unified}. % \cite{abraham2016estimating}, PASTA, CIA
% Security policies apply differently depending on the assessment of security requirements or patch feasibility of assets.
% The third part of the event detection process organizes and improves security rules of security models that are used for verification. For instance, verification procedures can rely on architectures for probabilistic model checking which allows modular and system wide security analysis \cite{mundhenk2015security}. 


% % reaction/adaptation/ examples and explanation
% An example intrusion detection in the software domain is the time interval analysis of in-vehicle network messages \cite{song2016intrusion}. % intrusion detection timing analysis of can messages
% Such an detection triggers the reaction process of a \ac{siem} framework which performs the countermeasure strategy. The transition of the driving level into safe mode is a potential neutralization of the attack that precedes the damage evaluation step of the reaction plan \cite{waszecki2017automotive}. 

%cite mundhenk vehicle verification model as design goal ! reminder
% In Vehicle: Automotive Electrical and Electronic Architecture Security via Distributed In-Vehicle Traffic Monitoring
%% https://s-steinhorst.github.io/PDF/2017-TCAD-Automotive%20Electrical%20and%20Electronic%20Architecture%20Security%20via%20Distributed%20In-Vehicle%20Traffic%20Monitoring.pdf


%The asset identification process outlines the attack surfaces from software, hardware, and communication perspective in different layers of the reference architecture. To recap, the cloud, infrastructure and edge, and vehicle and peripherals make up the main layers of the reference model. 
%Those three mitigation concepts drive the defence design. In order to implement all concepts
%Apart from the basic security 

%Build your risk treatment strategy
%\textbf{Reduce}: building controls if the form of code upgrades, confirming a specific design for the application or building a specific configuration during the deployment phase to make sure that application risk is reduced.

%\textbf{Transfer}: For a specific component in the application the risk can be transferred to an outsourced third party to develop that component and making sure that the third party is doing the right testing for the component; or during the deployment phase, outsourcing a third party to do the deployment and transferring that risk to that third party.

%\textbf{Avoid}: an example of avoiding the risk is disabling a specific function in the application that is the source for that risk.
%\textbf{Accept}: if the risk is within acceptable criteria set earlier, in that case, the designer risk owner can accept that risk
%defence mechanism is risk treatment 


% \subsection{\ac{iov} Cyber Defence State of Practice} % (existing technologies)
% \label{countermeasuresiov}

% \subsubsection{Mitigation \& Countermeasures}
% The overview of defence mechanisms groups all potential countermeasures with regard to security requirements and attack surface types. Table \ref{tab:defenceanalysis} shows the summary of all collected defence concepts of the following surveys.
% The works \cite{cui2019review}, \cite{jang2014survey}, \cite{abdulghani2019study}, and \cite{abdul2018comprehensive} bring together and categorize countermeasures against attacks that target \ac{iov} specific hardware, software, and communication, data at rest, \ac{iot} software, communication protocols, network communication, connectivity, and physical hardware.
% Next, the following works highlight the importance of the selected concepts of interoperability \cite{eu2018road}, \ac{gdpr} \cite{sfakianakis2019enisa}, dynamic and automated risk assessment \cite{rao2017probabilistic}, attack prediction and attribution \cite{patel2013classification}, threat predictive analytics, monitoring, and detection intelligence \cite{nec18itaru}, encrypted traffic analysis \cite{cheng2018encrypted} \cite{anderson2017machine}, forensic readiness \cite{valjarevic2013harmonized}, intrusion detection \cite{haas2017intrusion} \cite{alheeti2016hybrid}, intrusion prevention \cite{anwar2017intrusion} \cite{anuar2009response}, penetration testing \cite{scarfone2008technical}, and honeypots \cite{wahlisch2013design}. 
% The collection of countermeasures serves for orientation about which countermeasure to apply in what layer of the proposed multi-layer security concept.


%Image signature verification, Volume encryption, Ephemeral disk encryption, Sahara, Magnum, Octavia/LBaaS, Swift, Passwords in Config Files (https://docs.openstack.org/security-guide/secrets-management/secrets-management-use-cases.html)

% \todo{this section rather into related works/background}



%% Dont know if this table should remain or not !!
% \begin{table}[htbp] % [!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{IoV Cyber Defence Mechanism Evaluation}
% \label{tab:defenceanalysis}
% \centering
% \begin{tabular}{|p{1.25cm}|p{5.5cm}|p{0.8cm}|} % p{1cm}|
% \hline
% \textbf{Affected Requirements} & \textbf{Defence Mechanism} & \textbf{Surface Type} \\  % & \textbf{Category}   \\
% \hline
% \hline
% Access control & Detection, Anti-spoofing methods, Access control lists, Sessions  & All \\ %%  & Create, Modify  \\
% \hline
% Usability & Anti-jamming technique, Filtering data, Honeypots, Other source of data, Separate infotainment system, Intrusion detection, Anti-virus, Firewall & All \\ % & Create, Modify, Read, Remove  \\
% \hline
% Integrity & Authenticated map server, CAN security, Intrusion detection, Filtering data, Other source of data, Runtime integrity check, \ac{dlt}  & COM, SW    \\ % & Create, Modify \\
% \hline
% Privacy & Anonymization schemes, Homomorphic encryption, Encryption, Searchable encryption, Hash schemes, Obfuscation & All  \\ % & Read, \ \ \ \ Interrupt, Modify \\
% \hline
% Non-repudiation & Secure Logging, active and passive intrusion response system, Deduplication, Introspection & SW, COM  \\ % & Modify, Remove \\
% \hline
% Manage- ability & Hypervisor, Security operation center, Interoperability, Distributed data repositories, Recovery schemes & SW \\ % & Interrupt \\
% \hline
% Physical Protection & System Hardening, Process separation, Trusted computing, Secure Ethernet switching, Self-desctruction,Tamper proofing, Side channel signal analysis, Watermarking, Obfuscation  & HW   \\ %  & Interrupt, Modify  \\
% \hline
% Attack \ \ Detection & Logging, IDPS, IDS, Auditing, Signature detection, Anomaly detection, Stateful protocol analysis  & SW     \\ %   & Create, Read \\
% \hline
% Fare Exchange & Anti-spoofing methods, Key management, Endpoint verification, PKI trust management &  All  \\ %  & \\
% \hline
% Freshness & Secure diagnosis, Quality of service, Secure updates & SW    \\ % & Modify, Remove, Read, Create \\
% \hline
% Secure Information Flow & Process separation, Application sandbox, Domain separation, Network firewall, Proxy, Secure switching, Secure data migration  & COM, SW    \\ % & Read, Create, Interrupt, Remove \\
% \hline
% Confor-mance & Anti-virus, Model checking  & SW   \\ % & x \\
% \hline
% \end{tabular}
% \end{table}


% \begin{table}[ht] % [!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% % if using array.sty, it might be a good idea to tweak the value of \extrarowheight as needed to properly center the text within the cells
% \caption{Countermeasures}
% \label{table_countermeasures}
% \centering
% % Some packages, such as MDW tools, offer better commands for making tables
% % than the plain LaTeX2e tabular which is used here.
% \begin{tabular}{|c||c||c||c||c|}
% \hline
% \textbf{Name} & \textbf{Type} & \textbf{Attack} & \textbf{Layer} & \textbf{References} \\
% \hline 
% \hline 
% Data Collection & Prediction  & & &  \\
% \hline
% Access Rights/Roles & Avoidance & & &  \\
% \hline
% Encryption & Avoidance & & &  \\
% \hline
% Anomaly Detection & Prediction & & &  \\
% \hline
% Blocking & Mitigation & & &  \\
% \hline
% Isolation & Recovery & & &  \\
% \hline
% Redundancy & Recovery & & &  \\
% \hline
% \end{tabular}
% \end{table}
%% src: emanuel: **Types:** Which type of mechanism?
% Mitigation types:::
%          - Redundancy: error correction, N-Version
%          - Recovery: roll-back, reconfigure
%          - Barrier: Firewall


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SHORTCOMINGS AND GAPS
% \subsubsection{Shortcomings/Gaps in existing solutions}

% Even though the state of practice of defence mechanisms covers a very wide range of attacks, shortcomings remain. Problematic is the adaptation of security frameworks to latest security standards \cite{rasmussen2018gap}. It is therefore important to pay special attention to the following categories of security gaps of the works \cite{sun2017attacks},  \cite{barnard2014threat}, and \cite{parkinson2017cyber}.
% \begin{itemize}
%     \item Reduction of effects of existing systems
%     \item External effects
%     \item Long term studies of fast evolving security techniques
%     \item Knowledge Gaps and their potential impact
%     \item Human error and criminology
%     \item Impact of law, policy, and liability
% \end{itemize}


% Cyber Threats Facing Autonomous and Connected vehicles future challenges summarizes everything \cite{parkinson2017cyber}

% Konfido main statement that security is outdated \cite{rasmussen2018gap}

% Gaps of D2.1 [29] \cite{neghina2013managing}:
% 1. Weak software security and weak data encryption.
% 2. A lot of inter-dependencies with big and complex attack surfaces mostly due to the
% heterogeneous nature of the components of the CAV ecosystems.
% 3. Human error and insider attacks.
% 4. Cascade effects when there are interdependencies between groups of CAV devices in the context
% of smart cities.
% 5. Lack of (complete) automation in risk assessment frameworks. Periodic risk assessment
% approaches have been currently deployed utilising manual interventions to solve the identified
% issues. This is mostly due to limited knowledge of the system and lack of understanding of risk
% propagation with the inter-dependent components of the system in question.
% 6. Lack of global propagation of the information regarding threats to the involved stakeholders
% 7. Reactive as opposed to proactive threat detection and mitigation strategies.
% 8. Lack of dynamic threat detection of previously unknown attacks
% 9. Lack of (near) real time spatio-temporal parameters to measure risk levels instead of static/fixed
% attributes

% [93] \cite{sun2017attacks}:
% 1. Reducing the defects of existing Intrusion Detection Systems
% 2. Privacy protection in the package routing processing in IoV
% 3. Dealing with big data. Vehicle manufacturers are facing the challenge of handling large quantities
% of data generated by millions of vehicles while maintaining the security and privacy of customer
% information
% 4. Verification of trust-based recommendation in IoV social network is also a current challenge
% 5. Providing good delay performance under the restrictions of vehicles’speed, unstable connection,
% and quickly changing network topology
% 6. Data protection of the mobile cloud users and allowing users to decide how to expose or hide
% their information are the main targets of mobile cloud computing
% 7. Appropriate design of the cross layered transmission protocol is really important for IoVs to
% support real-time and multimedia applications
% 8. In-depth investigation of the user’s behaviour and extracting rules for this kind of attacks
% 9. Pay attention to factors such as instability of bandwidth and network topologies when designing
% the forwarding of an IoV network package from one network node to another.


%GHOST project Deliverable D3.1: Initial Gap analysis and recommendations (https://drive.google.com/file/d/1loUPkaCCpP5Wb60eiJm8Cj2JWwXR5MSR/view), \cite{barnard2014threat}: 
% - larger incident response strategy, how can a vehicle contribute (to what extend information shared securely)
% - natural disasters(not too important)
% - criminology, new behavior of criminals
% - role of vehicle in critical infrastructure
% - liability and insurance issues, especially with autonomos driving
% - impact of law and policy
% - baseline requirement standardization
% - user education for IoV 
% - training at various levels and development of best practices
% - IoV security diagnosis and forensic methods
% - Interface between vehicles and infrastructure
% - security methodologies: patching, updates, provision of information to asset owners, incident logging and report,
% - long term studies



% Iterate over components and check for shortcomings

%\subsection{Attack to Defence/Countermeasure Mechanism Mapping}

%Mapping problem methodology, static and dynamic mapping, np hard - heuristic methodologies

% \subsection{Need of a complete system}
% The IoV stakeholder requirement analysis uncovers the most relevant system assets and functionalities  

% \subsubsection{Stakeholder Requirements}
%\subsubsection{Functional Requirements}

% Security mechanisms protect against a subset of possible attacks. 

% Hence, security design concepts need to quantify which assets to protect. 
% Next, security concepts need to determine which possible attack it wants the asset to protect against.
% After provision determination, it should be possible to state the amount of time and money it takes for an attack to compromise an asset.

% paragraph about attack categorization
% external internal, local/remote, device owner, specialist, etc... not tooo important maybe, connection to stakeholders 

% paragraph about protection mechanisms, most complex one, this requires threat model which first investigates assets -> we do it by requirement analysis and stakeholders, then

% Work \cite{lu2014connected} categorizes IoV architecture into vehicle-to-sensor on-board (V2S), vehicle-to-vehicle (V2V), vehicle-to-road infrastructure (V2R), and vehicle-to-Internet (V2I) and provides characteristics and challenges.

% Components: Vehicle, Road Infrastructure, Internet, On-Board-Sensors

% Stakeholders of an IoV infrastructure are Autonomous Vehicle Manufacturers, Transportation Authorities, Customers, Governments

% \begin{table}[!ht] % [!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% % if using array.sty, it might be a good idea to tweak the value of \extrarowheight as needed to properly center the text within the cells
% \caption{Stakeholders}
% \label{table_stakeholders}
% \centering
% \begin{tabular}{|c||c||c|}
% \hline
% \textbf{Stakeholder} & \textbf{Description} \\
% \hline
% \hline
% Autonomous Vehicle Manufacturer & ... \\
% \hline
% Transport Authority & ... \\
% \hline
% Customer & ....  \\
% \hline
% Government & .... \\
% \hline
% Automotive Service/Parts Supplier & .... \\
% \hline
% \end{tabular}
% \end{table}










%% continue here....
% design components of detailed attacks and detailed design of defence components at layer intersections and sub systems is future work. also asset identification for different use cases might look differently, we suggest that this analysis of other use cases have to be compared to our work to develop major components that fulfil multiple tasks of different applications with similar units, then this contributes to the overal general security design for a total iov infrastructure. but out use case shows an extendable framework that can be changed and modified/extended based on new use case needs to eventually reach perfect design. 

% The asset identification and evaluation drives the attack prevention design of our security framework proposal that aims to secure the position estimation service within an \ac{iov} infrastructure. 
% The reason for that is the ability to set up propagation paths of attack vectors that aim to harm the location service.  
% Therefore, attacks of the categories of hardware, communication, and software apply to cloud, infrastructure and edge, and vehicle and peripheral domains of the total reference architecture. 
% The identified attacks belong to the collection of threat vectors towards the infrastructure surface and represent the first quantity of the vulnerability 


% security design aligns with nIoVe adaptive cybersecurity framework link.
% from outside to inside: identified security requirements apply to the assets on the attack surface and the defence investigation lists possible mitigation techniques and defence mechanism, where the interplay and selection needs to be further investigated. after the outest layer of assets the same attack and defence mechanisms need to secure possible attack path propagation from either of the three main attack graphs with different attacker model properties of the attacker. after all prevention techniques are in place, it is then possible to start investigating what data needs to be collected, and where collectors need to be placed to enable attack detection. the core module of the analytics siem component depends on its hardware requirements which decides whether to install several analytical components directly inside of the car or on more powerful 
% RSUs or in the cloud, important is as much data should be processed locally as possible and anonymized to respect data privacy regulations, in cases of reponse strategy that triggers forensics, more data can be logged and stored in the defence architecture, the siem detection of attacks then triggers response mechanisms that travel back to the modules and perform the mitigation/response strategy of isolation, recovery, shut down, and inform stakeholders of the system so that the car can park safely after location data cannot be guaranteed anymore.
% afterwards requires need calibration mechanisms to get back on track. collected data of the vehicle is the inspected afterwards by vehicle holder. 

% figure: \ref{fig:mainsecuritydesigntailored} summarizes the defence concept towards position determination use case 



% \begin{figure}[!ht]
%     \centering
%     \begin{tikzpicture}[scale=0.9]
    
%     % 3 major blocks in center
%     \node (el1) at (0,-4) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=9.6cm, minimum height=0.5cm, transform shape = true, align=left] {Layer 0: IoV Stakeholders and System Administrators \& \\Control, Monitoring and Notification User Interfaces};
    
%     \node (el2) at (2.25,-2) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=5cm, minimum height=0.5cm, transform shape = true, align=left] {Layer 1: Scenario Data \\Assets (Cloud, Infra, Vehicle)};
    
%     \node (el3) at (3.5,-1) [transform shape = true, anchor=west , align=left] {Data Collection};
    
%     \node (el122) at (2.25,0) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=5cm, minimum height=0.5cm, transform shape = true, align=left] {Layer 2: Scenario Software \\Assets (Cloud, Infra, Vehicle)};
    
%     \node (el3) at (3.5,1) [transform shape = true, anchor=west , align=left] {Data Collection};
    
%     \node (el4) at (2.25,2) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=5cm, minimum height=0.5cm, transform shape = true, align=left] {Layer 3: Scenario Networking \\Assets (Cloud, Infra, Vehicle)};
    
%     \node (el5) at (3.5,3) [transform shape = true, anchor=west , align=left] {Data Collection};
    
%     \node (el6) at (2.25,4) [rectangle, anchor=west, thick, draw=black, fill=white!90!gray, minimum width=5cm, minimum height=0.5cm, transform shape = true, align=left] {Layer 4: Scenario Hardware \\Assets (Cloud, Infra, Vehicle)};
    
%     \node (el17) at (3.5,5) [transform shape = true, anchor=west , align=left] {Data Collection};
    
%     \node (el18) at (2.25,6) [rectangle, anchor=west, thick, draw=black, fill=white!70!gray, minimum width=5cm, minimum height=0.5cm, transform shape = true, align=left] {Layer 5: Software SIEM Frame-\\work (Detection, Reaction)};
    
%     \node (el70) at (0,-2) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ DATA};
%     \node (el7) at (0,0) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ \ SW};
%     \node (el8) at (0,2) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ NET};
%     \node (el9) at (0,4) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ \ HW};
    
%     \node (el10) at (7.55,4) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ \ HW};
%     \node (el11) at (7.55,2) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ NET};
%     \node (el12) at (7.55,0) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ \ SW};
%     \node (el13) at (7.55,-2) [rectangle, anchor=west, dashed, draw=black, fill=white, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Scenario 2 \\ \ \ \ DATA};

%     \draw [<-, dashed] (el70.south) --  ++(0,-1.025);
%     \draw [->, dashed] (el70.north) --  (el7.south);
%     \draw [->, dashed] (el7.north) --  (el8.south);
%     \draw [->, dashed] (el8.north) -- (el9.south);
%     \draw [->, dashed] (el9.north) -- ++(0,1.55) -- (el18.west);
%     \draw [->, dashed] (el18.east) -- ++(1.25,0) -- (el10.north);
%     \draw [->, dashed] (el10.south) -- (el11.north);
%     \draw [->, dashed] (el11.south) -- (el12.north);
%     \draw [->, dashed] (el12.south) -- (el13.north);
%     \draw [->, dashed] (el13.south) -- ++(0,-1.025);
    
    
%     \draw [->, line width=0.05mm] (el1.north) -- ++(2, 0) -- ++(-4,0) -- ++(0, 1);
%     \draw [->, line width=0.05mm] (el122.south) -- ++(-2, 0) -- ++(4,0) -- ++(0, -1);
    
%     \draw [->, line width=0.05mm] (el122.north) -- ++(2, 0) -- ++(-4,0) -- ++(0, 1);
%     \draw [->, line width=0.05mm] (el2.south) -- ++(-2, 0) -- ++(4,0) -- ++(0, -1);
    
%     \draw [->, line width=0.05mm] (el2.north) -- ++(2, 0) -- ++(-4,0) -- ++(0, 1);
%     \draw [->, line width=0.05mm] (el4.south) -- ++(-2, 0) -- ++(4,0) -- ++(0, -1);
    
%     \draw [->, line width=0.05mm] (el4.north) -- ++(2, 0) -- ++(-4,0) -- ++(0, 1);
%     \draw [->, line width=0.05mm] (el6.south) -- ++(-2, 0) -- ++(4,0) -- ++(0, -1);
    
%     \draw [->, line width=0.05mm] (el6.north) -- ++(2, 0) -- ++(-4,0) -- ++(0, 1);
%     \draw [->, line width=0.05mm] (el18.south) -- ++(-2, 0) -- ++(4,0) -- ++(0, -1);
    
    
%     \node (el20) at (0,7) [rectangle, anchor=west, thick, draw=black, fill=yellow, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Prevention};
    
%     \node (el21) at (3.75,7) [rectangle, anchor=west, thick, draw=black, fill=yellow, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Detection};
    
%     \node (el22) at (7.55,7) [rectangle, anchor=west, thick, draw=black, fill=yellow, minimum width=2cm, minimum height=0.5cm, transform shape = true, align=left] {Reaction};
    
%     % \draw [-] (el3.south) -- ++(0,-0.69);
%     % \draw [-] (el2.north) -- ++(0,0.78);

%     % top blocks for detection block
%     % \node (netw1) at (3.25,2) [draw, align=left, minimum height=1.5cm,minimum width=7.75cm, transform shape = true] {};
%     % \node (el4) at (1.3,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Risk \\Evaluation};
%     % \node (el5) at (3.1,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Security \\Policy};
%     % \node (el6) at (4.7,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Master \\Plan};
%     % \node (el7) at (7,2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Verification};

%     % \draw [->] (el4.east) -- (el5.west);
%     % \draw [->] (el5.east) -- (el6.west);
%     % \draw [->] (el6.east) -- (el7.west);

%     % % lower blocks for reaction block
%     % \node (netw2) at (3.25,-2) [draw, align=left, minimum height=1.7cm,minimum width=9.5cm, transform shape = true] {};
%     % \node (el8) at (0.4,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Identify \& \\Confirm \\Event};
%     % \node (el9) at (2.4,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Neutralise \\Attack};
%     % \node (el10) at (4.25,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Evaluate \\Damages};
%     % \node (el11) at (6.25,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Restore \\Normal \\Operation};
%     % \node (el12) at (7.85,-2) [rectangle, anchor=east, thick, draw=black, fill=white!70!gray, minimum width=1cm, minimum height=0.5cm, transform shape = true, align=left] {Learn \\Lesson};

%     % \draw [->] (el8.east) -- (el9.west);
%     % \draw [->] (el9.east) -- (el10.west);
%     % \draw [->] (el10.east) -- (el11.west);
%     % \draw [->] (el11.east) -- (el12.west);

%     \end{tikzpicture}
%   \caption{Extendable Holistic Multi-Layer \ac{iov} Security Methodology}
% \label{fig:mainsecuritydesigntailored}
% \end{figure}




% layer 0 has identified assets and communication paths that position data travels
% layer 1 has secure communication and software modules that collect data and send around
% layer 2 is the  siem analytics framework, that analyses data of ecus, if possible in vehicle, such that no interval data is wrong and no big anomalies and outliners during position data mathcing and maneuver calculations exist, in any case the vehicle needs to be stopped
% attacks should be tracked back if possible to determine the damage causing unit and develop response strategy, if the component that was compromised has important funcitonality mechanisms such as decentralized designs with majority and redundancy should create more reliable solutions where system can rely on majority that is harder to attack.
% layer 3 is connection of analytics software to user interfaces of iov stakeholders and system administrators and also vehicle operators, such that they can take action (reduce, transfer, avoid, accept critically level determined by location service sources, and depending on avaliable input) if necessary and correct location manually/last case
% problem is that model should not be layered in best case, but have a U form, left side up, then down to feedback and response back to components.


% cite [1]  Angeliki Zacharaki, Ioannis Paliokas, Konstantinos Votis, Christos Alexakos, Dimitrios Serpanos and Dimitrios Tzovaras, “Complex Engineering Systems as an enabler for security in Internet of Vehicles: The nIoVe approach”, IEEE Societal Automation 2019 (SA2019), (in press).
% (https://niove.eu/index.php/dissemination/publications)







% refer to 4 layer (cloud, infra \& edge, vehicle, peripherals) reference architecture 

% aligns with logical view 7 layers architecture


\subsection{Framework Application \& Evaluation}
\label{section6}

The application of our proposed 4+1 security methodology with regard to the \ac{iov} location service scenario produces risk assessment data in Table \ref{tab:cvssscores}. 
The data of identified assets makes up quantitative input to the a Markov Model.
The Markov Model can be used to verify individual reference model domains/layers and respective domains of the view model analysis.
Our evaluation approach verifies data, software, networking, and hardware security in different reference model domains.
Unfortunately and up to this point, the reference model characteristics do not influence the \ac{cvss} scores.
The result of missing incorporation of reference model characteristics to the risk assessment per attack propagation stage causes the attack vectors of row one and two as well as row four and five of Table \ref{tab:cvssscores} to have equal security verification values.
Apart from this constrain, several other constrains apply which we address in the next subsection.
Nonetheless, the sample application and resulting security verification results evaluate the proposed 4+1 view security methodology and point out constrains that need to be considered in order to receive a unbiased quantitative security verification results.

% \begin{table}[htbp] % [!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Amount of Security Requirements per Asset}
% \label{tab:amountrequirementsonassets}
% \centering
% \begin{tabular}{|p{1.25cm}|p{1.75cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}|} % p{1cm}|
% \hline
% \textbf{Total} & \textbf{Surface Type} & \textbf{Cloud} & \textbf{Infra} & \textbf{Vehicle}  \\  % & \textbf{Category}   \\
% \hline
% \hline
% 7 & \textbf{HW} & 2 &  2  & 3  \\ 
% \hline
% 16 & \textbf{COM} & 8 &  4  & 4  \\ 
% \hline
% 18 & \textbf{SW} & 6 &  2  & 10  \\ 
% \hline
% \hline
% \textbf{Total} & & \textbf{16} & \textbf{8} & \textbf{17} \\ 
% \hline
% \end{tabular}
% \end{table}

% corresponding atatck graph created with the application of the security framework
% In order to evaluate the individual security design which aligns with the categorizations of the proposed security framework, 

\subsubsection{Evaluation Constrains} % Assumptions
\label{evalassumptions}

%In the same way as the probabilities depend on the surface and model categories, each state of the attacker in the attack network graph of Table \ref{tab:attackpropagation} maps to surface and model type.  


% \todo{align the values to related work (Security Analysis of Automotive Architectures using
% Probabilistic Model Checking -- done)}

% 
%                 A
%            (.9)/
%           A    
%    (.2)/  (./1)\ 
%     /           A'
% S_0  
%     \           A
%    (.8)\  (.7)/
%         A'
%           (.3)\
%                 A'
% 
% Here, S_0 = [.2, .8] is initial state, then after one week for ex S_1 = [.2 .8][.9 .1] = [.74 .26]
%                                                                                [.7 .3]    
% Total path W^n (S_0 to A) = (.2)*(.9) + (.8)*(.7) = .18+.56 = .74
% our case is more simple as it only considers one path and multiplies the transition probabilities together

The values for the calculation of the state transition matrix depend on the probabilities of attacks and patches. 
Table \ref{tab:cvssscores} shows the vulnerability scores per asset for each domain of the view model analysis. 
Higher values determine a higher likelihood in successfully attacking an asset. 
% The amount of attacks and preventive defence mechanism play a minor role because it is almost always possible to find a defence mechanism per attack. 
% The data variance of the distribution of security requirements is more expressive.
As a matter of fact, the risk assessment \ac{cvss} score over the maximum possible score determines the attacking probability $a$ of an attack in a specific time window.
% the table entry of the amount of security requirements per assets over the amount of all security requirements serves as the probability $a$ that an attack occurs in a specific time window.
Based on the Formula \ref{formula0}, the attack probability for a networking attack is shown in Formula \ref{formula1}.
% \begin{equation}
% \label{formula1}
% a = \frac{8}{12} \hspace{5mm} (1-a)=\frac{4}{12} \hspace{5mm} d=\frac{1}{2} \hspace{5mm} (1-d)=\frac{1}{2}
% \end{equation}
As already indicated, it would be possible to determine the \ac{cvss} scores with respect to the reference model domains of cloud, infrastructure and edge, and vehicle and peripherals to create three different \ac{cvss} scores per view model domain.
To achieve this improvement, the vulnerability scoring system would needs to incorporate the reference model characteristics into the environment score.
To proceed without the consideration of reference model types during security verification and to simplify, we expect the probability of an occurrence of a countermeasure over a specific time window to be constant with the value of $d=\frac{1}{10}$ for this evaluation.
\begin{equation}
\label{formula1}
\resizebox{.9\hsize}{!}{$
a=\frac{15}{42.5}=0.35; \hspace{1mm} (1-a)=\frac{27.5}{42.5}; \hspace{1mm} d=\frac{1}{10}; \hspace{1mm} (1-d)=\frac{9}{10}
$}
\end{equation}
The reason for the value is that attack detection and effective response mechanism miss long term studies and steady integration into all systems where cost typically prevents the implementation of advanced security for every asset.
As a general disclaimer, we need to state that all numbers of the evaluation align with related work assumptions but require further investigation. 
It is moreover assumed that the attacks on the location scenario face defence concepts at every stage. % where they do not have explicit access.


% disclaimer that this overall value assumption needs further investigation, but it suffices to evaluate the framework

It is now possible to apply the risk assessment values of Table \ref{tab:cvssscores} as a measure for attacking probability and apply them to one of the attack vectors of Table \ref{tab:attackpropagation}. 
To demonstrate the evaluation process we take the short attack vector propagation of row three of Table \ref{tab:attackpropagation}.
The attack path starts with hardware access of the attacker to vehicle peripherals and interfaces at stage $i=1$. 
The next attack is of type communication and targets a model type of vehicle and peripherals at stage $i=2$.
By taking the attack probability formula \ref{formula02}, the attack and complementary attack probability are $a = 1-e^{-2*(\frac{15}{42.5})} = 0.506$ and $(1-a) = 0.504$ respectively. The defence and complementary defence probability remain as stated in Formula \ref{formula1}.
% is $a=\frac{4}{12}$ and $(1-a)=\frac{8}{12}$ respectively. 
These values make up the first row entries the transition probability matrix \ref{probtransitionmatrix} when the values are applied to the transition formulas seen in Figure \ref{fig:transitionprobgraph}.
In this case with an authorized attacker, we can neglect the transition probabilities of the initial state $S_1$ which reduces the matrix dimensions by 1.

\begin{equation}
    \label{probtransitionmatrix}
    P = \begin{bmatrix}
       0.5 & 0.5 & 0  & 0 \\[0.3em]
       0.05 & 0.55  & 0.40 & 0 \\[0.3em]
       0 & 0.01 &  0.21  & 0.78 \\[0.3em]
       0  & 0  & 0.1 & 0.9
     \end{bmatrix}
\end{equation}
% \begin{equation}
%     \label{probtransitionmatrix}
%     P = \begin{bmatrix}
%       \frac{8}{12} & \frac{4}{12} & 0           \\[0.3em]
%       \frac{1}{12} & \frac{6}{12}           & \frac{5}{12} \\[0.3em]
%       0           & \frac{6}{12} & \frac{6}{12}
%      \end{bmatrix}
% \end{equation}
% \todo{its possible to express this matrix with regard to state surface and model type}

The second attack on the attack path is of type software and harms a component of the vehicle model type.
As a result and for stage $i=3$, $a = 1-e^{-3*(\frac{8.1}{42.5})} = 0.435$ and the transition equations of state $i=3$ of Figure \ref{fig:transitionprobgraph} produce the entries of the second row of matrix \ref{probtransitionmatrix} which represents the state transitions of $S_3$ to $S_2$, $S_3$ to $S_3$, and $S_3$ to $S_4$ respectively. 
For instance, transition probability between $S_3$ and $S_3$ at stage $i=3$ is $0.435*0.1+0.565*0.9=0.55$.
The last transition probabilities depend on the countermeasure only.
Last, the formula $W^{3}(S_0) = 0.5*0.4*0.78 = 0.156 = 15.6\%$ aggregates all state transition probabilities where we leave out any possible detours. % $W^{3}(S_0) = \frac{4}{12}*\frac{5}{12} = \frac{5}{36}$
In contrast, if we take the formula \ref{formula0} to calculate the attack probability $a$ and the same attack path as just indicated, we receive a total probability of $2.8\%$.
This final calculation completes the process of calculating the total attack realization probability from an initial state $S_1$ to the target state $S_5$ of the scenario.
The total attack probability value of our example is the top right entry of Table \ref{tab:results}.
Likewise, other values of Table \ref{tab:results} correspond to all other initial to target state attack realization probabilities of our attack vector graph.
\begin{table}[htbp] % [!t]
\renewcommand{\arraystretch}{1.3}
\caption{Attack Realization Probabilities of All Initial Attack States}
\label{tab:results}
\centering
\begin{tabular}{|p{2cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}|} % p{1cm}|
\hline
\textbf{Attacker Type} & \textbf{Cloud} & \textbf{Infra} & \textbf{Vehicle}  \\  % & \textbf{Category}   \\
\hline
\hline
% Authorized & 0.0231 & 0.0231 &  0.1389   \\ 
% \hline
% Unauthorized & 0.0077 & 0.0039 &  0.0405   \\ 
% \hline
% Authorized & 2.3\% & 2.3\% &  13.8\%   \\ 
% \hline
% Unauthorized & 0.7\% & 0.3\% &  4\%   \\ 
% \hline
Authorized & 11.2\% & 11.2\% &  15.6\%   \\ 
\hline
Unauthorized & 2.8\% & 2.8\% &  5.9\%   \\ 
\hline
\end{tabular}
\end{table}

% idea, say attack successfull if higher probability than 75 percent, compare with modeling of mundhenk


\subsubsection{Results}
\label{results}

The attack realization probabilities of the initial states align with the expected behavior of lower probable attacks for longer attack paths.
The results moreover show the variance of the security evaluation metrics with regard to changes of the proposed methodology. 
The decomposition of multiple view model layers into more detailed categories lowers the attack probabilities drastically due to the multiplicative aggregation. 
Hence, the level of detail should remain similar among the different categories.
An extension of the number of scenarios first of all would not affect results of already calculated attacking probabilities when they are looked at independently. 
Nevertheless, the extendable methodology allows to take over states of already evaluated scenarios to support the evaluation of additional scenarios.
The surface abstraction of data, software, networking, and hardware provides another dimension to fine tune the security design. 
Generally, high level defence mechanisms exist for high level attack categories. 
However, the methodology allows a more detailed analysis of asset vulnerability categorizations and attack to vulnerability mappings which we did not included into our simplified evaluation concept.
Another remaining point to investigate is the affect of the view mode security methodology on the reaction and countermeasure probabilities. 
Since attack response mechanisms face similar network propagation transitions such as attack occurrences, they are expected to behave similar to the attack realization events.


In total, the evaluation shows that our methodology contributes to an early estimation of system vulnerability propagation and distribution within the system. 
The methodology considers all security relevant connections, and allows repetitive adaptation of design parameters for an structured approach to security design. 
The evaluation shows that the high level categorization already connects the relevant security design requirements and, thereby, proves to be valuable. 


% \todo{only top right is correct, need to update rest}

% (and how vulnerabilities traverse the infrastructure depending on the scenario, framework considers all security relevant connections, and allows repetitive adaptation of design for an structured approach to security design that considers the parameters set initially) which can be addressed by taking a more detailed look into the respective domains. But the evaluation shows that the high level categorization already affects the design with regard to security and connects the relevant security design requirements and thereby proves to be valuable. 

% change the parameters of the security framework: \# of scenarios, \# of layers, \# of reference model 
% and create respective transition probability matrices that allow to calculate the security evaluation of the design that aligns with our framework. 

% \subsection{Risk Assessment Types}

% \begin{itemize}
%     \item Time-to-Compromise \& Const-to-Compromise (Probabilistic)
%     \item Time Between Vulnerability Disclosure
%     \item Automating the Attack Graph
%     \item Threat Coupling to Database Known Vulnerabilities
% \end{itemize}


% \subsection{Risk Before Application of Holistic Security Framework}


% \begin{figure}[!t]
% \centering
% \includegraphics[width=3.25in]{time-to-compromise1}
% \caption{Time to Compromise  \cite{xiong2019threat}.}
% \label{fig:time-to-compromise-without-protection}
% \end{figure}


% \subsection{Risk After Application of Holistic Security Framework}






==> sections/1.5_conclusion.tex <==
\section{Conclusion}
\label{section7}


\subsection{Summary}

The application of the well established 4+1 view model in the security context allows to apply agile threat modeling and risk assessment strategies on \ac{iov} infrastructure assets in a structured way.
The view model analysis separates data, software, networking, and hardware perspectives and enables attack vector construction between these layers. 
Moreover, the fine grained asset identification contributes to flaw detection and security requirements definition per asset.
Resulting vulnerability analysis on identified assets enable comprehensive risk assessment per attacking stage.
Risk parameters serve as quantitative input to probabilistic Markov Chain models which evaluate attack trees on security metrics.
The proposed security methodology of this work combines the 4+1 view model perspectives with security objectives and enables quantitative security assessment of holistic \ac{iov} architectures.

\subsection{Future Work}
\begin{itemize}
    \item To support the quantitative security verification results of the 4+1 view security model, hacker teams need to conduct comprehensive and multidisciplinary methodologies such as QuERIES. 
    Contrasting \ac{ttc} times of security assessment of the 4+1 view security model and QuERIES \ac{ttc} results indicates the offset with regard to real security performance metrics.
    \item The extendibility of the proposed security framework requires evaluation with regard to the application of additional metrics such as attacker cost, defence detection and reaction times, and other scenarios.
    Next to the security \ac{ttc} metric, the 4+1 view analysis may focus or incorporate metrics such as \ac{ctc}, time between vulnerability disclosure, time to detect, and threat coupling to known vulnerabilities or utilize other risk assessment models.
    \item No research has been conducted with regard to automation of the security analysis approach. 
    To cope with complex systems of the \ac{iov}, automation of analysis concepts is mandatory for system wide security coverage \cite{rao2017probabilistic}.
    Here, it is possible to utilize existing automated threat modeling and risk assessment tools on separated perspectives. 
    
    
    
    % Our work modelled a security strategy as well as the attacks for the \ac{iov} location service scenarios. Next, the QuERIES methodology could optimize the security framework by quantification of both models by measuring the cost for the implementation of all security requirements per asset. Quantification of the attacking cost of the attacker models is typically conducted through hired hacker teams. With the quantification information, it is possible to propose an efficient investment strategy for the cybersecurity framework to promote its establishment \cite{carin2008cybersecurity}.
    % \item Our work investigates security of technical aspects of localization scenarios as they are most important for a vehicle to move. When vehicles move securely, it is necessary to ensure security for remaining scenarios such as traffic light recognition, obstacle detection, secure and verifiable compliance with road traffic law, and secure course determination, deployment and maintenance. 
    % \item Risk Assessment Types

    % \begin{itemize}
    %     \item Time-to-Compromise \& Const-to-Compromise (Probabilistic)
    %     \item Time Between Vulnerability Disclosure
    %     \item Automating the Attack Graph
    %     \item Threat Coupling to Database Known Vulnerabilities
    %     \item Time To Detect
    % \end{itemize}
    
    % \item Details of each layer and details of every asset and the software role and purpose of every component in multi sensor fusion scenario and location scenario
\end{itemize}





% \todo{this table to appendix??}

% \begin{table}[htbp] % [!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Flaws of Vulnerability Taxonomies \cite{igure2008taxonomies}}
% \label{tab:appendixtable1}
% \centering
% \begin{tabular}{|p{1.25cm}|p{6.5cm}|}
% \hline
% \textbf{Attack Surface Type} & \textbf{Vulnerabilities} \\ 
% \hline
% \hline
% Software Data  & Incomplete parameter validation, Inconsistent parameter validation, Implicit sharing of privileged/confidential data, Inadequate identification, Authentication or authorization, Asynchronous validation or inadequate serialization, Violable prohibition or limiting and exploitable logic error \\ 
% \hline
% Software Implementation &  \\ 
% \hline
% Commun- ication/ Networking & The transfer strategy (circuit-switched or packet-switched), The network transfer control method, The transfer link structure, Link access method or protocol, System topology architecture, Topology, Physical layer, Data link layer, Network layer, Management and control, Traffic analysis, Passive eavesdropping, Active eavesdropping, Unauthorized access, Man-in-the-middle, Session highjacking and replay attacks, Clear text communication, Non-robust protocol message parsing, Insecure protocol state handling, Inability to handle abnormal packet rates, Replay and reuse, Protocol field authentication, Entropy problems \\ 
% \hline
% Hardware &   \\ 
% \hline
% \end{tabular}
% \end{table}


% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{eearch}
% \caption{Physical View of In-Vehicle E/E-Architecture \cite{brunner2017automotive}.}
% \label{fig:physicalautomotivearchorginal}
% \end{figure}
% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{tileshop}
% \caption{Logical View of Vehicle Localization Components \cite{vetrella2016differential}.}
% \label{fig:logviewlocationoriginal}
% \end{figure}
% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{logicalview-gps-reception}
% \caption{Logical Views of GPS Receiver Tracking System \cite{navstar1996user}.}
% \label{fig:logicalviewgpsreceive}
% \end{figure}
% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{sensor-analysis}
% \caption{Logical View of Sensor data processing \cite{chen2017multi}.}
% \label{fig:sensorlogical}
% \end{figure}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{autosarclassic}
% \caption{Developer View Software Autosar Classic without libraries, rather high level \cite{warschofsky2009autosar}.}
% \label{fig:sensorlogical}
% \end{figure}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{autosaradaptive}
% \caption{Developer View Software Adaptive AUTOSAR software architecture without libraries, rather high level \cite{furst2016autosar}.}
% \label{fig:sensorlogical}
% \end{figure}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{attack-path1}
% \caption{attack graph 1 \cite{xiong2019threat}}
% \label{fig:attackgraph1}
% \end{figure}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{attack-path2}
% \caption{attack graph 2 \cite{xiong2019threat}}
% \label{fig:attackgraph1}
% \end{figure}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=3.25in]{attack-vec1}
% \caption{attack to communication and vulnerable assets 2 \cite{rizvi2017threat}}
% \label{fig:attackvec1}
% \end{figure}

